Adversarial Satisfiability Problem

We study the adversarial satisfiability problem, where the adversary can choose whether variables are negated in clauses or not in order to make the resulting formula unsatisfiable. This is one case of a general class of adversarial optimization problems that often arise in practice and are algorithmically much harder than the standard optimization problems. We use the cavity method to compute large deviations of the entropy in the random satisfiability problem with respect to the negation-configurations. We conclude that in the thermodynamic limit the best strategy the adversary can adopt is extremely close to simply balancing the number of times every variable is and is not negated. We also conduct a numerical study of the problem, and find that there are very strong pre-asymptotic effects that are due to the fact that for small sizes exponential and factorial growth is hardly distinguishable.

==> figures/fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,3298){\makebox(0,0)[r]{\strut{}$(s_{B},\mathcal{L}_{B}), \alpha=1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,2852){\makebox(0,0)[r]{\strut{}$(s_{B},\mathcal{L}_{B}), \alpha=2$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,2407){\makebox(0,0)[r]{\strut{}$(s_{B},\mathcal{L}_{B}), \alpha=3$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,1961){\makebox(0,0)[r]{\strut{}$(s_{R},\mathcal{L}_{R}), \alpha=1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,1515){\makebox(0,0)[r]{\strut{}$(s_{R},\mathcal{L}_{R}), \alpha=2$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2591,1069){\makebox(0,0)[r]{\strut{}$(s_{R},\mathcal{L}_{R}), \alpha=3$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1179){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1774){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,2368){\makebox(0,0)[r]{\strut{} 3}}%
      \put(946,2962){\makebox(0,0)[r]{\strut{} 4}}%
      \put(946,3557){\makebox(0,0)[r]{\strut{} 5}}%
      \put(946,4151){\makebox(0,0)[r]{\strut{} 6}}%
      \put(946,4745){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1078,484){\makebox(0,0){\strut{} 0.1}}%
      \put(2262,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3446,484){\makebox(0,0){\strut{} 0.3}}%
      \put(4630,484){\makebox(0,0){\strut{} 0.4}}%
      \put(5814,484){\makebox(0,0){\strut{} 0.5}}%
      \put(6998,484){\makebox(0,0){\strut{} 0.6}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4334,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6498,4932){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s),\,\alpha=1$}}%
      \csname LTb\endcsname%
      \put(6498,4712){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s),\,\alpha=2$}}%
      \csname LTb\endcsname%
      \put(6498,4492){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s),\,\alpha=3$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig10.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{} 8.93}}%
      \put(1342,1156){\makebox(0,0)[r]{\strut{} 8.94}}%
      \put(1342,1609){\makebox(0,0)[r]{\strut{} 8.95}}%
      \put(1342,2061){\makebox(0,0)[r]{\strut{} 8.96}}%
      \put(1342,2514){\makebox(0,0)[r]{\strut{} 8.97}}%
      \put(1342,2966){\makebox(0,0)[r]{\strut{} 8.98}}%
      \put(1342,3419){\makebox(0,0)[r]{\strut{} 8.99}}%
      \put(1342,3871){\makebox(0,0)[r]{\strut{} 9}}%
      \put(1342,4324){\makebox(0,0)[r]{\strut{} 9.01}}%
      \put(1342,4776){\makebox(0,0)[r]{\strut{} 9.02}}%
      \put(1663,484){\makebox(0,0){\strut{}-2.5}}%
      \put(2610,484){\makebox(0,0){\strut{}-2}}%
      \put(3557,484){\makebox(0,0){\strut{}-1.5}}%
      \put(4503,484){\makebox(0,0){\strut{}-1}}%
      \put(5450,484){\makebox(0,0){\strut{}-0.5}}%
      \put(6397,484){\makebox(0,0){\strut{} 0}}%
      \put(440,2740){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}_{SP}(\Sigma)$}}}%
      \put(4172,154){\makebox(0,0){\strut{}$\Sigma$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5038,4603){\makebox(0,0)[r]{\strut{}$\mathcal{L}_{SP}(\Sigma)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig10}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig11.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,1043){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1210,1722){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1210,2401){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1210,3079){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1210,3758){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1210,4437){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1342,484){\makebox(0,0){\strut{} 4}}%
      \put(2263,484){\makebox(0,0){\strut{} 5}}%
      \put(3185,484){\makebox(0,0){\strut{} 6}}%
      \put(4106,484){\makebox(0,0){\strut{} 7}}%
      \put(5027,484){\makebox(0,0){\strut{} 8}}%
      \put(5949,484){\makebox(0,0){\strut{} 9}}%
      \put(6870,484){\makebox(0,0){\strut{} 10}}%
      \put(440,2740){\rotatebox{90}{\makebox(0,0){\strut{}$p_{s}$}}}%
      \put(4106,154){\makebox(0,0){\strut{}$L$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5852,4603){\makebox(0,0)[r]{\strut{}$N=9$}}%
      \csname LTb\endcsname%
      \put(5852,4383){\makebox(0,0)[r]{\strut{}$N=18$}}%
      \csname LTb\endcsname%
      \put(5852,4163){\makebox(0,0)[r]{\strut{}$N=27$}}%
      \csname LTb\endcsname%
      \put(5852,3943){\makebox(0,0)[r]{\strut{}$N=36$}}%
      \csname LTb\endcsname%
      \put(5852,3723){\makebox(0,0)[r]{\strut{}$N=45$}}%
      \csname LTb\endcsname%
      \put(5852,3503){\makebox(0,0)[r]{\strut{}$N=54$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig11}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(1342,1156){\makebox(0,0)[r]{\strut{}-0.35}}%
      \put(1342,1609){\makebox(0,0)[r]{\strut{}-0.3}}%
      \put(1342,2061){\makebox(0,0)[r]{\strut{}-0.25}}%
      \put(1342,2514){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(1342,2966){\makebox(0,0)[r]{\strut{}-0.15}}%
      \put(1342,3419){\makebox(0,0)[r]{\strut{}-0.1}}%
      \put(1342,3871){\makebox(0,0)[r]{\strut{}-0.05}}%
      \put(1342,4324){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1342,4776){\makebox(0,0)[r]{\strut{} 0.05}}%
      \put(1474,484){\makebox(0,0){\strut{} 0}}%
      \put(2373,484){\makebox(0,0){\strut{} 0.05}}%
      \put(3273,484){\makebox(0,0){\strut{} 0.1}}%
      \put(4172,484){\makebox(0,0){\strut{} 0.15}}%
      \put(5071,484){\makebox(0,0){\strut{} 0.2}}%
      \put(5971,484){\makebox(0,0){\strut{} 0.25}}%
      \put(6870,484){\makebox(0,0){\strut{} 0.3}}%
      \put(440,2740){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s) $}}}%
      \put(4172,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2540,4448){\makebox(0,0)[r]{\strut{}$N=21$}}%
      \csname LTb\endcsname%
      \put(2540,4228){\makebox(0,0)[r]{\strut{}$N=27$}}%
      \csname LTb\endcsname%
      \put(2540,4008){\makebox(0,0)[r]{\strut{}$N=39$}}%
      \csname LTb\endcsname%
      \put(2540,3788){\makebox(0,0)[r]{\strut{}$N=60$}}%
      \csname LTb\endcsname%
      \put(2540,3568){\makebox(0,0)[r]{\strut{}$N=75$}}%
      \csname LTb\endcsname%
      \put(2540,3348){\makebox(0,0)[r]{\strut{}$(s_L,0)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1210,1619){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,2534){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1210,3450){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1210,4365){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1210,5280){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1342,484){\makebox(0,0){\strut{} 0.44}}%
      \put(2175,484){\makebox(0,0){\strut{} 0.46}}%
      \put(3008,484){\makebox(0,0){\strut{} 0.48}}%
      \put(3841,484){\makebox(0,0){\strut{} 0.5}}%
      \put(4674,484){\makebox(0,0){\strut{} 0.52}}%
      \put(5507,484){\makebox(0,0){\strut{} 0.54}}%
      \put(6340,484){\makebox(0,0){\strut{} 0.56}}%
      \put(7173,484){\makebox(0,0){\strut{} 0.58}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4466,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4652,4346){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1210,1619){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,2534){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1210,3450){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1210,4365){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1210,5280){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1342,484){\makebox(0,0){\strut{} 0.44}}%
      \put(2175,484){\makebox(0,0){\strut{} 0.46}}%
      \put(3008,484){\makebox(0,0){\strut{} 0.48}}%
      \put(3841,484){\makebox(0,0){\strut{} 0.5}}%
      \put(4674,484){\makebox(0,0){\strut{} 0.52}}%
      \put(5507,484){\makebox(0,0){\strut{} 0.54}}%
      \put(6340,484){\makebox(0,0){\strut{} 0.56}}%
      \put(7173,484){\makebox(0,0){\strut{} 0.58}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4466,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4400,4169){\makebox(0,0)[r]{\strut{}$(s_{L},\mathcal{L}_{L})$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1210,1619){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,2534){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1210,3450){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1210,4365){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1210,5280){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1342,484){\makebox(0,0){\strut{} 0.44}}%
      \put(2175,484){\makebox(0,0){\strut{} 0.46}}%
      \put(3008,484){\makebox(0,0){\strut{} 0.48}}%
      \put(3841,484){\makebox(0,0){\strut{} 0.5}}%
      \put(4674,484){\makebox(0,0){\strut{} 0.52}}%
      \put(5507,484){\makebox(0,0){\strut{} 0.54}}%
      \put(6340,484){\makebox(0,0){\strut{} 0.56}}%
      \put(7173,484){\makebox(0,0){\strut{} 0.58}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4466,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4400,3848){\makebox(0,0)[r]{\strut{}$(s_{R},\mathcal{L}_R)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1210,1619){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,2534){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1210,3450){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1210,4365){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1210,5280){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1342,484){\makebox(0,0){\strut{} 0.44}}%
      \put(2175,484){\makebox(0,0){\strut{} 0.46}}%
      \put(3008,484){\makebox(0,0){\strut{} 0.48}}%
      \put(3841,484){\makebox(0,0){\strut{} 0.5}}%
      \put(4674,484){\makebox(0,0){\strut{} 0.52}}%
      \put(5507,484){\makebox(0,0){\strut{} 0.54}}%
      \put(6340,484){\makebox(0,0){\strut{} 0.56}}%
      \put(7173,484){\makebox(0,0){\strut{} 0.58}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4466,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4400,3574){\makebox(0,0)[r]{\strut{}$(s_{\rm{ran}}, L  \log 2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2782,1460){\makebox(0,0)[r]{\strut{} 0.44}}%
      \put(2782,1874){\makebox(0,0)[r]{\strut{} 0.48}}%
      \put(2782,2288){\makebox(0,0)[r]{\strut{} 0.52}}%
      \put(2782,2702){\makebox(0,0)[r]{\strut{} 0.56}}%
      \put(2914,1240){\makebox(0,0){\strut{}-300}}%
      \put(3453,1240){\makebox(0,0){\strut{}-200}}%
      \put(3993,1240){\makebox(0,0){\strut{}-100}}%
      \put(4532,1240){\makebox(0,0){\strut{} 0}}%
      \put(5071,1240){\makebox(0,0){\strut{} 100}}%
      \put(5611,1240){\makebox(0,0){\strut{} 200}}%
      \put(6150,1240){\makebox(0,0){\strut{} 300}}%
      \put(1880,2236){\rotatebox{90}{\makebox(0,0){\strut{}$s(x)$}}}%
      \put(4532,910){\makebox(0,0){\strut{}$x$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5295,2488){\makebox(0,0)[r]{\strut{}$s(x)$}}%
      \csname LTb\endcsname%
      \put(5295,2268){\makebox(0,0)[r]{\strut{}$s_{L}$}}%
      \csname LTb\endcsname%
      \put(5295,2048){\makebox(0,0)[r]{\strut{}$s_{R}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplbacktext
    \put(0,0){\includegraphics{fig6}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig7.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,829){\makebox(0,0)[r]{\strut{} 8.84}}%
      \put(1342,1167){\makebox(0,0)[r]{\strut{} 8.88}}%
      \put(1342,1505){\makebox(0,0)[r]{\strut{} 8.92}}%
      \put(1342,1843){\makebox(0,0)[r]{\strut{} 8.96}}%
      \put(1342,2181){\makebox(0,0)[r]{\strut{} 9}}%
      \put(1342,2519){\makebox(0,0)[r]{\strut{} 9.04}}%
      \put(2056,440){\makebox(0,0){\strut{}-0.08}}%
      \put(3221,440){\makebox(0,0){\strut{}-0.06}}%
      \put(4386,440){\makebox(0,0){\strut{}-0.04}}%
      \put(5551,440){\makebox(0,0){\strut{}-0.02}}%
      \put(6716,440){\makebox(0,0){\strut{} 0}}%
      \put(440,1589){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(\Sigma)$}}}%
      \put(4532,110){\makebox(0,0){\strut{}$\Sigma$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6603,833){\makebox(0,0)[r]{\strut{}$\mathcal{L}(\Sigma), L=13$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,3522){\makebox(0,0)[r]{\strut{} 8.2}}%
      \put(1342,4015){\makebox(0,0)[r]{\strut{} 8.22}}%
      \put(1342,4508){\makebox(0,0)[r]{\strut{} 8.24}}%
      \put(1342,5001){\makebox(0,0)[r]{\strut{} 8.26}}%
      \put(2118,3056){\makebox(0,0){\strut{}-0.016}}%
      \put(3405,3056){\makebox(0,0){\strut{}-0.012}}%
      \put(4693,3056){\makebox(0,0){\strut{}-0.008}}%
      \put(5981,3056){\makebox(0,0){\strut{}-0.004}}%
      \put(7268,3056){\makebox(0,0){\strut{} 0}}%
      \put(440,4261){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(\Sigma)$}}}%
      \put(4532,2726){\makebox(0,0){\strut{}$\Sigma$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6603,3449){\makebox(0,0)[r]{\strut{}$\mathcal{L}(\Sigma), L=12$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig7}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/fig9.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,1023){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1342,1555){\makebox(0,0)[r]{\strut{} 1.55}}%
      \put(1342,2087){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(1342,2620){\makebox(0,0)[r]{\strut{} 1.65}}%
      \put(1342,3152){\makebox(0,0)[r]{\strut{} 1.7}}%
      \put(1342,3684){\makebox(0,0)[r]{\strut{} 1.75}}%
      \put(1342,4216){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(1342,4748){\makebox(0,0)[r]{\strut{} 1.85}}%
      \put(1342,5280){\makebox(0,0)[r]{\strut{} 1.9}}%
      \put(1944,484){\makebox(0,0){\strut{} 0.52}}%
      \put(2885,484){\makebox(0,0){\strut{} 0.522}}%
      \put(3826,484){\makebox(0,0){\strut{} 0.524}}%
      \put(4767,484){\makebox(0,0){\strut{} 0.526}}%
      \put(5708,484){\makebox(0,0){\strut{} 0.528}}%
      \put(6649,484){\makebox(0,0){\strut{} 0.53}}%
      \put(7590,484){\makebox(0,0){\strut{} 0.532}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4532,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6735,1931){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s),\, \,N=10^2,\,P=10^3 $,}}%
      \put(6735,1711){\makebox(0,0)[r]{\strut{} balanced negations}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,1023){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1342,1555){\makebox(0,0)[r]{\strut{} 1.55}}%
      \put(1342,2087){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(1342,2620){\makebox(0,0)[r]{\strut{} 1.65}}%
      \put(1342,3152){\makebox(0,0)[r]{\strut{} 1.7}}%
      \put(1342,3684){\makebox(0,0)[r]{\strut{} 1.75}}%
      \put(1342,4216){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(1342,4748){\makebox(0,0)[r]{\strut{} 1.85}}%
      \put(1342,5280){\makebox(0,0)[r]{\strut{} 1.9}}%
      \put(1944,484){\makebox(0,0){\strut{} 0.52}}%
      \put(2885,484){\makebox(0,0){\strut{} 0.522}}%
      \put(3826,484){\makebox(0,0){\strut{} 0.524}}%
      \put(4767,484){\makebox(0,0){\strut{} 0.526}}%
      \put(5708,484){\makebox(0,0){\strut{} 0.528}}%
      \put(6649,484){\makebox(0,0){\strut{} 0.53}}%
      \put(7590,484){\makebox(0,0){\strut{} 0.532}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4532,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6735,1399){\makebox(0,0)[r]{\strut{}$\mathcal{L}(s),\, N=P=500$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,1023){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1342,1555){\makebox(0,0)[r]{\strut{} 1.55}}%
      \put(1342,2087){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(1342,2620){\makebox(0,0)[r]{\strut{} 1.65}}%
      \put(1342,3152){\makebox(0,0)[r]{\strut{} 1.7}}%
      \put(1342,3684){\makebox(0,0)[r]{\strut{} 1.75}}%
      \put(1342,4216){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(1342,4748){\makebox(0,0)[r]{\strut{} 1.85}}%
      \put(1342,5280){\makebox(0,0)[r]{\strut{} 1.9}}%
      \put(1944,484){\makebox(0,0){\strut{} 0.52}}%
      \put(2885,484){\makebox(0,0){\strut{} 0.522}}%
      \put(3826,484){\makebox(0,0){\strut{} 0.524}}%
      \put(4767,484){\makebox(0,0){\strut{} 0.526}}%
      \put(5708,484){\makebox(0,0){\strut{} 0.528}}%
      \put(6649,484){\makebox(0,0){\strut{} 0.53}}%
      \put(7590,484){\makebox(0,0){\strut{} 0.532}}%
      \put(440,2992){\rotatebox{90}{\makebox(0,0){\strut{}$\mathcal{L}(s)$}}}%
      \put(4532,154){\makebox(0,0){\strut{}$s$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6735,1133){\makebox(0,0)[r]{\strut{}$(s_{B },\mathcal{L}_{B})$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig9}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/figures.tex <==
%figures.tex - all figure data

\newcommand{\figureoneB}{


}

\newcommand{\figurezero}{%
%
\begin{tikzpicture}[line width=.9pt,scale=3]  
%[inner sep=10mm,  place/.style={circle,draw=blue!50,fill=blue!20,thick},  transition/.style={rectangle,draw=black!50,fill=black!20,thick}]  
\path (0,0)  node[draw,shape=rectangle, minimum size=.7cm] (a){$a$}; 
\path (-.45,.25)  node[draw,shape=circle,minimum size=.8cm,] (j) {$j$}; 
\path (-.45,-.25)  node[draw,shape=circle,minimum size=.8cm,] (k) {$k$}; 
\path (.5,0)  node[draw,shape=circle,minimum size=.8cm,] (i) {$i$}; 
\path (.95,.25)  node[draw,shape=rectangle,minimum size=.7cm] (b){$b$}; 
\path (.95,-.25)  node[draw,shape=rectangle,minimum size=.7cm] (c){$c$}; 
%\path (.5,.5)  node[draw,shape=rectangle,minimum size=.7cm,] (h)  {$ia$}; 
%\path (.5,0)  node[draw,shape=circle,minimum size=.7cm,style={draw,double}] (J)  {$\omega_{ia}$}; 
%\path (0,0) node[draw,shape=rectangle,minimum size=.5cm]  {};
%\path (1,0) node[draw,shape=rectangle,minimum size=.5cm]  {};
\draw 
(a) -- (j)
(a) -- (i)
(-.85,.45) -- (j)
(a) -- (k)
(i) -- (b);
\draw[dashed]
(-.85,-.45) -- (k)
(-.05,-.45) -- (k)
(1.35,-.45) -- (c)
(1.35,.45) -- (b)
(i) -- (c);
\end{tikzpicture} 
%
}






\newcommand{\figureone}{%
%
%tikz picture content goes here
\begin{tikzpicture}[line width=.2pt,scale=10](2.5,.4)
[inner sep=10mm,  place/.style={circle,draw=blue!50,fill=blue!20,thick},  transition/.style={rectangle,draw=black!50,fill=black!20,thick}]  
\path (0,0)  node[draw,shape=rectangle,minimum size=.5cm] (v0)  {$a$}; 
\path (.5,0)  node[draw,shape=circle,minimum size=.85cm] (x)  {$i$}; 
\path (1,0)  node[draw,shape=rectangle,minimum size=.5cm] (psi)  {$b$}; 
\path (-.25,-.25) node[draw,shape=circle,minimum size=.5cm] (y)  {$i_a^2$}; 
\path (-.25,.25) node[draw,shape=circle,minimum size=.5cm] (z)  {$i_a^3$}; 
\path (1.25,.25) node[draw,shape=circle,minimum size=.5cm] (u)  {$i_b^2$}; 
\path (1.25,-.25) node[draw,shape=circle,minimum size=.5cm] (v)  {$i_b^1$}; 
\draw 
(-.5,-.5) -- (y)
(-.5,.5) -- (z)
(v0) -- (x)  	 
(0,.5) -- (z)	
(v0) -- (y) 	
(psi) -- (v); 
\draw[dashed]
(x) -- (psi) 
(psi) -- (u) 	 
(v0) -- (z) 
(1,-.5) -- (v)
(1.5,.5) -- (u);
%\draw[arrows=->](0.5,.25)--(1.,.25); 
%\draw[arrows=<-](0.5,.2)--(1.,.2); 	 
%\draw[arrows=->](0.,.225)--(.5,.225); 	 
%\draw[arrows=<-](0.,.175)--(.5,.175);
\end{tikzpicture} 
%
}






\newcommand{\figuretwo}{%
%
\begin{tikzpicture}[line width=.9pt,scale=3]  
\path (0,0)  node[draw,shape=rectangle,minimum size=.7cm,label=below:$a$] (a){}; 
\path (0,0) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};
\path (1,0)  node[draw,shape=circle,minimum size=.8cm,label=below:$i$] (i) {}; 
\path (1,0) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};
\path (.5,.5)  node[draw,shape=rectangle,minimum size=.7cm, fill=black, label=above:$ia$ ] (h)  {}; 
\path (.5,0)  node[draw,shape=circle,minimum size=.7cm,fill=black, label=below:$\omega_{ia}$] (J)  {}; 
\path (-.6,-.6)  node[draw,shape=circle,minimum size=.8cm,] (j){}; 
\path (-.6,-.6) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};
\path (-.6,.6)  node[draw,shape=circle,minimum size=.8cm,] (k){}; 
\path (-.6,.6) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};
\path (1.6,.6)  node[draw,shape=rectangle,minimum size=.7cm] (b){}; 
\path (1.6,.6) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};
\path (1.6,-.6)  node[draw,shape=rectangle,minimum size=.7cm] (c){}; 
\path (1.6,-.6) node[draw,shape=rectangle,minimum size=.5cm, fill=black]  {};

\path (-.3,-.3)  node[draw,shape=circle,minimum size=.7cm,fill=black] (J2)  {}; 
\path (-.3,.3)  node[draw,shape=circle,minimum size=.7cm,fill=black] (J1)  {}; 
\path (1.3,-.3)  node[draw,shape=circle,minimum size=.7cm,fill=black] (J3)  {}; 
\path (1.3,.3)  node[draw,shape=circle,minimum size=.7cm,fill=black] (J4)  {}; 

\path (-.6,0)  node[draw,shape=rectangle,minimum size=.7cm, fill=black] (h1)  {}; 
\path (0,-0.6)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (h2)  {}; 
\path (1,-0.6)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (h3)  {}; 
\path (1.6,-0.)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (h4)  {}; 



%\path (1.9,-.4)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp1)  {}; 
%\path (1.9,-.8)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (hp1)  {}; 

%\path (-.9,-.4)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp2)  {}; 
%\path (-.9,-.8)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (hp2)  {}; 

%\path (-.9,.4)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp3)  {}; 
%\path (-.9,.8)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (hp3)  {}; 

%\path (1.9,.4)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp4)  {}; 
%\path (1.9,.8)  node[draw,shape=rectangle,minimum size=.7cm, fill=black ] (hp4)  {}; 

%\path (1.4,-.9)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp5)  {}; 
%\path (-.4,.9)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp6)  {}; 
%\path (1.4,.9)  node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp7)  {}; 
%\path  (-.4,-.9)   node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp8)  {}; 
%\path   (0.1,-.4)   node[draw,shape=circle,minimum size=.7cm,fill=black] (Jp9)  {}; 


\draw 
(i) -- (J)
(J) -- (a)
(h) -- (J)
(j) -- (a)
(k) -- (a)
(c) -- (i)
(b) -- (i)
(J1) -- (h1)
(J2) -- (h2)
(J3) -- (h3)
(J4) -- (h4)


%(c) -- (Jp1)
%(k) -- (Jp3)
%(b) -- (Jp4)
%(j) -- (Jp2);
%(Jp1) -- (hp1)
%(Jp2) -- (hp2)
%(Jp3) -- (hp3)
%(Jp4) -- (hp4)
%(Jp1) -- (2.3,-.4)
%(Jp2) -- (-1.3,-.4)
%(Jp3) -- (-1.3,.4)
%(Jp4) -- (2.3,.4)
%(c) -- (Jp5)
%(k) -- (Jp6)
%(b) -- (Jp7)
%(j) -- (Jp8) 
%(j) -- (Jp9) 
;
\end{tikzpicture} 
%
}

\newcommand{\figurethree}{
%
\begin{tikzpicture}[line width=.9pt,scale=3]  
\path (0,0)  node[draw,shape=rectangle,minimum size=.7cm] (i){$a$}; 
\path (1,0)  node[draw,shape=circle,minimum size=.8cm,] (a) {$i$}; 
\path (.5,.5)  node[draw,shape=rectangle,minimum size=.7cm,] (h)  {$ia$}; 
\path (.5,0)  node[draw,shape=circle,minimum size=.7cm,style={draw,double}] (J)  {$\zeta_{ia}$}; 
\path (0,0) node[draw,shape=rectangle,minimum size=.5cm]  {};
\path (1,0) node[draw,shape=rectangle,minimum size=.5cm]  {};
\draw 
(a) -- (J)
(J) -- (i)
(h) -- (J)
(-.25,-.25) -- (i)
(-.25,.25) -- (i)
(1.25,-.25) -- (a)
(1.25,.25) -- (a);
\end{tikzpicture} 
%
}

==> myentries.tex <==
@book{Balian83,
	author="Roger Balian",
	title="Du Microscopique au Macroscopique,
	Cours de physique statistique de l'Ecole polytechnique"	,
	publisher="Ellipses",
	year="1983"
}

@BOOK{DiuGutman89,
  AUTHOR =       "B. Diu and C. Guthmann and D. Lederer and B. Roulet",
  TITLE =        "Physique Statistique",
  PUBLISHER =    "Hermann",
  YEAR =         "1989",
  series =       "Collection Enseignement des Sciences",
  address =      "Paris"
}

@book{AartsLenstra97,
        editor = "E. H. L. Aarts and J. K. Lenstra",
        title = "Local Search in Combinatorial Optimization",
        publisher = "J. Wiley \& and Sons",
        year = 1997,
        address = "New York"}

@book{Pearl88,
 author = {Judea Pearl},
 title = {Probabilistic reasoning in intelligent systems: networks of plausible inference},
 year = {1988},
 isbn = {0-934613-73-7},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
 }


@article{CrawfordAuton96,
 author = {James M. Crawford and Larry D. Auton},
 title = {Experimental results on the crossover point in random 3-SAT},
 journal = {Artif. Intell.},
 volume = {81},
 number = {1-2},
 year = {1996},
 issn = {0004-3702},
 pages = {31--57},
 doi = {http://dx.doi.org/10.1016/0004-3702(95)00046-1},
 publisher = {Elsevier Science Publishers Ltd.},
 address = {Essex, UK},
 }

@misc{EFFprize,
   note="http://w2.eff.org/awards/coop-prime-rules.php"
}

@article{AjtaiKomlos84,
    author = "M. Ajtai and J. Komlos and G. Tusnady",
    title = "On Optimal Matchings",
    journal = "Combinatorica",
    year = 1984,
    volume = 4,
    pages = "259--264"}

@article{AgrawalKayal04,
    author = "Manindra Agrawal and Neeraj Kayal and Nitin Saxena",
    title = "PRIMES is in P",
    journal = "Annals of Mathematics",
    year = 2004,
    number = 2,
    volume = 160,
    pages = "781--793"}


@incollection{AlavaDuxbury01,
       author = "M.J. Alava and P.M. Duxbury and C. Moukarzel and H.
Rieger",
       title = "Exact combinatorial algorithms: Ground states
                of disordered systems",
       editor = "J. Lebowitz and C. Domb",
       booktitle = "Phase Transitions and Critical Phenomena",
       year = 2001,
       publisher = "Academic press"}

@article{AlberichDoussineau97,
      author = "F. Alberich and P. Doussineau and A. Levelut",
      title = "",
      journal = "J. Phys. I (France)",
      volume = 7,
      pages = "329",
      year = 1997}

@article{Aldous01,
  author = "D. J. Aldous",
  title = "The $\zeta(2)$ limit in the random assignment problem",
  journal = "Rand. Struct. Algo.",
    year = 2001,
    volume = 18,
    pages = "381--418"}

@article{Aldous90,
  author = "D. J. Aldous",
  title = "A random tree model associated with random graphs",
  journal = "Rand. Struct. Algo.",
    year = 1990,
    volume = 1,
    pages = "383--402"}

@article{AldousBandyopadhyay05,
  author = "D. J. Aldous and A. Bandyopadhyay",
  title = "A survey of max-type recursive distributional equations",
  journal = "Annals of Applied Probability",
  volume =15,
  year = 2005,
  pages = "1047--1110"
}

@article{AldousPercus03,
      author = "D. Aldous and A. Percus",
      title = "Scaling and Universality in Continuous length Combinatorial Optimization",
      journal = "Proc. Natl. Acad. Sci. USA",
      volume = 100,
      pages = "11211--11215",
      year = 2003
}

@article{AldousPercus03,
  author = "D. J. Aldous and A. G. Percus",
  title = "Scaling and universality in continuous length combinatorial optimization",
  journal = "PNAS",
    year = 2003,
  volume = 100,
    pages = "11211--11215"}

@InProceedings{AldousSteele03,
    author = "D. Aldous and M. Steele",
    title ="The objective method: Probabilistic combinatorial optimization and local weak convergence",
    booktitle ="Encyclopedia of Mathematical Sciences",
  editor="H. Kesten",
  volume=110,
  pages = "1--72",
  publisher = "Springer",
  year = 2003}

@article{AlmeidaThouless78,
    author = "J. R. L. de Almeida and D. J. Thouless",
    title = "Stability of the {S}herrington-{K}irkpatrick Solution of a Spin-Glass Model",
    journal = "J. Phys. A",
    year = 1978,
    volume = 11,
    pages = "983--990"}


@article{Anderson72,
    author = "P.~W. Anderson",
  title = "More is different",
    journal = "Science",
    year = 1972,
    volume = 177,
    pages = "392"}

@article{AndreanovBarbieri04,
      author = " A. Andreanov and F. Barbieri and O. C. Martin",
      title = "Large deviations in spin-glass ground-state energies",
      journal = "Eur. Phys. J. B.",
      volume = 41,
      pages = "365",
      year = 2004
}

@article{Angell00,
    author = "C. A Angell",
    journal = "J. Phys. C.",
    year = 2000,
    volume = 29,
    pages = "6463"}

@article{Angell95,
    author = "C.~A. Angell",
    title = "Formation of Glasses from Liquids and Biopolymers",
    journal = "Science",
    year = 1995,
    volume = 267,
    number = "5206",
    pages = "1924-1935"}

@article{AnglesSourlas97,
    author = "J.-C. {Angles d'Auriac} and N. Sourlas",
    title = "The 3{D} Random-Field {I}sing Model at Zero Temperature",
    journal = "Europhys. Lett.",
    year = 1997,
    volume = 39,
    pages = "473--478"}

@article{ArdeliusAurell06,
    author = "John Ardelius and Erik Aurell",
    title = "Behavior of heuristics on large and hard satisfiability problems",
    journal = "Phys. Rev. E",
    year = 2006,
    volume = 74,
    pages = "037702"}

@article{ArdeliusZdeborova08,
    author = "John Ardelius and Lenka Zdeborov\'a",
    title = "Exhaustive enumeration unveils clustering and freezing in random 3-SAT",
    journal = "Phys. Rev. E (Rapid Com.)",
    year = 2008,
    page = "040101(R)"}

@unpublished{AlavaArdelius07,
    author = "Mikko Alava and John Ardelius and Erik Aurell and Petteri Kaski and Supriya Krishnamurthy and Pekka Orponen and Sakari Seitz",
    title = "Circumspect descent prevails in solving random constraint satisfaction problems",
    year = 2007,
    note = "arXiv:0711.4902v1 [cs.DS]",    
}

@article{SeitzAlava05,
    author = "Sakari Seitz and Mikko Alava and Pekka Orponen",
    title = "Focused Local Search for Random 3-Satisfiability",
    journal = "J. Stat. Mech.",
    year = "2005",
    pages = "P06006"}

@article{AspelmeierBray02,
    author = "T. Aspelmeier and A.J. Bray and M.A. Moore",
    title = "Why temperature chaos in spin glasses is hard to observe",
    journal = "Phys. Rev. Lett.",
    year = "2002",
    volume = "89",
    pages = "197202"}

@article{AspelmeierMoore02,
    author = "T. Aspelmeier and M.A. Moore",
    title = "Free energy fluctuations in {I}sing spin glasses",
    journal = " ",
    year = 2002,
    volume = " ",
    pages = " ",
  note = "cond-mat/0211707"}
%   note = "cond-mat/0009418"


@book{AthreyaNey72,
    author = "K. B. Athreya and P. E. Ney",
    title = "Branching processes",
    publisher = "Springer",
    address = "New York",
    year = 1972}

@article{AvramBertsimas92,
       author = "F. Avram and D. J. Bertsimas",
       title = "The Minimum Spanning Tree Constant in Geometrical
               Probability and under the Independant Model: A Unified
               Approach",
       journal = "Ann. Appl. Probab.",
       year = 1992,
       volume = 2,
       pages = "113--130"}

@article{Azuma67,
        author  = "X. Azuma",
        title   = "Weighted sums of certain dependent random
variables",
        journal = "Tohuku Math. Journal",
        year = 1967,
        volume = 19,
        pages = "357--367"}

@article{BaldiBaum86,
    author = "P. Baldi and E. B. Baum",
    title = "Bounds on the Size of Ultrametric Structures",
    journal = "Phys. Rev. Lett.",
    year = 1986,
    volume = 56,
    pages = "1598--1600"}

@article{BallDerigs83,
    author = "M. O. Ball and U. Derigs",
    title = "An Analysis of Alternative Strategies for Implementing
        Matching Algorithms",
    journal = "Networks",
    year = 1983,
    volume = 13,
    pages = "517--549"}

@article{BanavarBray87,
    author = "J. R. Banavar and A. J. Bray",
    title = "Chaos in spin glasses: A renormalization-group study",
    journal = "Phys. Rev. B",
    year = 1987,
    volume = 35,
    pages = "8888--8890"}

@article{BanavarSherrington87,
    author = "J. R. Banavar and D. Sherrington and N. Sourlas",
    title = "Graph Bipartitioning and Statistical Mechanics",
    journal = "J. Phys. A Lett.",
    year = 1987,
    volume = 20,
    pages = "L1--L8"}

@article{Bandyopadhyay04,
      author = "A. Bandyopadhyay",
      title = "Bivariate Uniqueness in the Logistic Recursive Distributional Equation",
     note = "math.PR/0401389",
      year = 2004}

@article{BargForney02,
      author = "A. Barg and G. D. Forney Jr",
      title = "Random codes : minimum distances and error exponents",
     journal = "IEEE Trans. Inform. Theory",
      volume = 48,
      pages = "2568--2573",
      year = 2002}

@article{Barrat97,
    author = "A. Barrat",
    title = "The p-spin spherical spin glass model",
    year = 1997,
  note = "Cond-mat/9701031"}
    %note = "cond-mat/0210144"

@article{BarratBerthier01,
    author = "A. Barrat and L. Berthier",
    title = "Real space application of the mean-field description of spin
glass dynamics",
  journal = "Phys. Rev. Lett",
    year = 2001,
    volume = 87,
    pages = "087204"}

@article{BarratFranz97,
    author = "A. Barrat and S. Franz and G. Parisi",
    title = "Temperature evolution and bifurcation of metastables states
in mean-field spin glasses, with connections with structural
glasses",
  journal = "J. Phys. A",
    year = 1997,
    volume = 30,
    pages = "5593-5612"}
    %note = "cond-mat/0210382"

@article{BarreBishop05a,
      author = " J. Barr\'e and A. R. Bishop and T. Lookman and A. Saxena",
      title = "The cavity method for the rigidity transition",
      journal = "J. Stat. Phys.",
      volume = "118",
      pages = "1057",
      year = 2005}

@article{BarreBishop05b,
      author = " J. Barr\'e and A. R. Bishop and T. Lookman and A. Saxena",
      title = "On adaptability and intermediate phase in randomly connected networks",
      journal = "Phys. Rev. Lett.",
      volume = "94",
      pages = "208701",
      year = 2005}

@ARTICLE{BattagliaBraunstein05,
   author = {{Battaglia}, D. and {Braunstein}, A. and {Chavas}, J. and {Zecchina}, R.
	},
    title = "{Source coding by efficient selection of ground-state clusters}",
  journal = {Phys. Rev. E},
   eprint = {arXiv:cond-mat/0412652},
     year = 2005,
    month = jul,
   volume = 72,
   number = 1,
    pages = {015103},
      doi = {10.1103/PhysRevE.72.015103},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvE..72a5103B},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{BauerGolinelli01,
      author = "M. Bauer and O. Golinelli",
      title = "Core percolation in random graphs: a critical phenomena analysis",
     journal = "Eur. Phys. J. B",
      volume = "24",
      pages = "339--352",
      year = 2001}

@book{Baxter82,
    author = "R. J. Baxter",
    title = "Exactly solved models in statistical mechanics",
  publisher = "Academic Press",
    year = 1982}

@article{Baxter99,
  author = "R. J. Baxter",
  title = "Planar lattice gases with nearest-neighbour exclusion",
  journal = "Annals of Combin.",
  year = 1999,
  volume = 3,
  pages = "191--203"}

@article{BeardwoodHalton59,
    author = "J. Beardwood and J. H. Halton and J. M. Hammersley",
    title = "The Shortest Path through Many Points",
    journal = "Proc. Camb. Phil. Soc.",
    year = 1959,
    volume = 55,
    pages = "299--327"}

@article{BellonCiliberto00,
      author = "L. Bellon and S. Ciliberto and C. Laroche",
      title = "Memory in the aging of a polymer glass",
      journal = "Europhys. Lett.",
      volume = "51",
      pages = "551--556",
      year = 2000}

@article{BellonCiliberto01,
      author = "L. Bellon and S. Ciliberto and C. Laroche",
      title = "Violation of the fluctuation-dissipation relation during the formation of a colloidal glass",
      journal = "Europhys.Lett.",
      volume = "53",
      pages = "511--517",
      year = 2001}

@article{BellonCiliberto02,
      author = "L. Bellon and S. Ciliberto",
      title = "Experimental study of the fluctuation-dissipation
relation
               during an aging process",
      journal = " Physica D",
      volume = "168-69",
      pages = "325--335",
      year = 2002}

@article{BellonCiliberto02b,
    author = "L. Bellon and S. Ciliberto and Laroche C.",
    title = "Advanced memory effects in the aging of a polymer glass",
    journal = "Eur. Phys. Jour. B.",
    year = 2002,
    volume = 25,
    pages = "223--231"}

@article{BellonCiliberto99,
      author = "L. Bellon and S. Ciliberto and C. Laroche",
      title = "Temperature cycling during the aging of a polymer
glass",
      journal = " ",
      volume = " ",
      pages = " ",
      year = 1999,
      note = "cond-mat/9905160"}

@article{Bendisch97,
    author = "J. Bendisch",
    title = "Ground State Threshold in Triangular Anisotropic +/- {J}
        {I}sing Model",
    journal = "Physica A",
    year = 1997,
    volume = 245,
    pages = "560--574"}

@article{BernadetPazmandi00,
    author = "K. Berardet and F. P\'azm\'andi and G. G. Batrouni",
    title = "Disorder Averaging and Finite-Size Scaling",
    journal = "Phys. Rev. Lett.",
    year = 2000,
    volume =  84,
    pages = "4477"}

@article{BernardiLemke98,
    author = "L. Bernardi and N. Lemke and P. Mari and I. Campbell",
    title = "The Spin Glass Transition: Exponents and Dynamics",
    year = 1998,
    note = "cond-mat/9804244"}

@article{BernardiLemke98,
    author = "L. Bernardi and N. Lemke and P.O. Mari and I.A. Campbell
            and A. Alegria and J. Colmenero",
    title = "The spin glass transition : exponents and dynamics",
    journal = "Physica A,",
    volume = "257",
    pages = "",
    year = "1998"}


@article{BernardiPrakash96,
    author = "L. Bernardi and S Parkash and I. Campbell",
    title = "Ordering Temperatures and Critical Exponents in Ising Spin
        Glasses",
    journal = "Phys. Rev. lett.",
    volume = 77,
    pages = "2798--2801",
    year = 1996}

@article{Berthier00,
    author = "L. Berthier",
    title = "Sub-ageing in a domain growth model",
    year = 2000,
  journal ="Eur. Phys. J. B ",
  volume = "17",
  pages = "689"}

@article{BerthierBarrat01,
    author = "L. Berthier and J.-L Barrat and J. Kurchan",
    title = "Dynamic ultrametricity in spin glasses",
    year = 2001,
  journal ="Phys. Rev. E",
  volume = "63",
  pages = "016105"}

@article{BerthierBouchaud02,
    author = "L. Berthier and J.-P. Bouchaud",
    title = "Geometrical Aspects of Aging and Rejuvenation in the Ising
Spin Glass: A Numerical Study",
        year = "2002",
        journal= "Phys. Rev. B",
        volume = "66",
        pages= "054404"}

@article{BerthierHoldsworth01,
    author = "L. Berthier and P.~C.~W. Holdsworth and M. Sellitto",
    title = "Non equilibrium critical dynamics of the 2D XY model",
    year = 2001,
  journal ="J. Phys. A",
  volume = "34",
  pages = "1805"}

@article{BerthierHoldsworth02,
    author = "L. Berthier and P.~C.~W. Holdsworth",
    title = "Surfing on a critical line: Rejuvenation without chaos,
Memory without a hierarchical phase space",
    year = 2002,
  journal ="Europhys. Lett. ",
  volume = "58",
  pages = "35",
  note = "cond-mat/0109169"}

@InProceedings{BerthierViasnoff02,
    author = {L. Berthier and V. Viasnoff and O. White and V. Orlyantchik
and F. Krzakala},
    title =              {Hiking through glassy phase : physics beyond aging},
    booktitle =      {Procedings of the Les Houches 2002 LXXVII summer
school},
    note = "To be publish",
  year = "2002"
}

@article{BertsimasRyzin90,
    author = "D. J. Bertsimas and G. {van Ryzin}",
    title = "An Asymptotic Determination of the Minimum Spanning Tree and Minimum Matching Constants in Geometrical Probability",
    journal = "Oper. Res. Lett.",
    year = 1990,
    volume = 9,
    pages = "223--231"}

@article{Bethe35,
      author = "H. A. Bethe",
      title = "Statistical physics of superlattices",
     journal = "Proc. Roy. Soc. London A",
      volume = 150,
      pages = "552--575",
      year = 1935}

@book{BevingtonRobinson94,
    author = "P. R. Bevington and D. K. Robinson",
    title = "Data Reduction and Error Analysis for the Physical Sciences",
    publisher = "McGraw-Hill",
    year = 1994,
    address = "New York"}

@book{LesHouches02,
    author = "J.-L. Barrat and M.V. Feigelman and J. Kurchan and J. Dalibard",
    title = "Slow Relaxations and Nonequilibrium Dynamics in Condensed Matter Les Houches Session LXXVII, 1-26 July, 2002",
    publisher = "Springer",
    year = 2003,
    address = "Berlin"}

@article{BhattYoung86,
    author = "R. Bhatt and A. P. Young",
    journal = "J. Magn. Magn. Mater.",
    year = 1986,
    volume = "54--57",
    pages = 191}

@article{BiecheMaynard80,
    author = "I. Bieche and R. Maynard and R. Rammal and J. P. Uhry",
    title = "On the Ground States of the Frustration Model of a Spin Glass by a Matching Method of Graph Theory",
    journal = "J. Phys. A",
    year = 1980,
    volume = 13,
    pages = "2553--2576"}

@article{Biggins77,
      author = "J. D. Biggins",
      title = "Chernoff theorem in the branching random walk",
     journal = "J. Appl. Probab.",
      volume = 14,
      pages = "630--636",
      year = 1977}

@article{BilloireMarinari00,
  author= "A. Billoire and E. Marinari",
  title= "Evidences Against Temperature Chaos in Mean Field and
Realistic Spin Glasses",
  journal = "J. Phys. A",
  year = 2000,
    volume = 33,
    pages = "L265"}

@article{BilloireMarinari02,
  author= "A. Billoire and E. Marinari",
  title= "Overlap Among States at Different Temperatures in the SK Model",
  journal = "Europhys. Lett.",
  year = 2002,
  volume = 60,
  pages  = 775}

@article{BinderYoung86,
    author = "K. Binder and A. P. Young",
    title = "Spin-Glasses: Experimental Facts, Theoretical Concepts and Open Questions",
    journal = "Rev. Mod. Phys.",
    year = 1986,
    volume = 58,
    pages = "801--976"}

@article{BiroliMezard02,
  author = "G. Biroli and M. M\'ezard",
  title = "Lattice Glass Models",
  journal = "Phys. Rev. Lett.",
  year = 2002,
  volume = 88,
  pages = "025501"}

@article{BiroliMonasson00,
  author = "G. Biroli and R. Monasson and M. Weigt",
  title = "A variational description of the ground state structure in random satisfiability problems",
  journal = "Eur. Phys. J. B",
  year = 2000,
  volume = 14,
  pages = "551"}

@article{Boettcher03a,
  author = "S. Boettcher",
  title = "Numerical Results for Ground States of Spin Glasses on
         {B}ethe Lattices",
  year="2003",
  journal = "Eur. Phys. J. B",
  volume = "31",
  pages = "29--39",
  note="cond-mat/0208196"}

@article{Boettcher03b,
  author = "S. Boettcher",
  title = "Numerical Results for Ground States of Mean-Field
           Spin Glasses at low Connectivities",
  journal = "Phys. Rev. B",
  volume = "67",
  pages = "060403",
  year="2003",
  note="cond-mat/0208444"}

@article{Boettcher03c,
  author = "S. Boettcher",
  title = "Reduction of Spin Glasses applied to the {M}igdal-{K}adanoff

           Hierarchical Lattice",
  journal = "",
  volume = "",
  pages = "",
  year="",
  note="cond-mat/0302424"}

@article{Boettcher03d,
  author = "S. Boettcher",
  title = "Determining Stiffness Exponents from the Reduction of
           Dilute Lattice Spin Glasses",
  journal = "",
  volume = "",
  pages = "",
  year="",
  note="cond-mat/0303431"}

@book{Bollobas01,
    author = "B. Bollob{\'a}s",
    title = "Random graphs",
  publisher = "Cambridge University Press",
  edition="Second",
    year = 2001}

@article{BollobasThomason86,
      author = "B. Bollob\'as and A. Thomason",
      title = "Threshold functions",
     journal = "Combinatorica",
      volume = 7,
      pages = "35--38",
      year = 1986}

@incollection{Bouchaud00,
      author = "J.-P. Bouchaud",
      title = "Aging in glassy systems: new experiments, simple models,
and open questions",
      editor = "M.E. Cates and M.R. Evans",
      booktitle = "Soft and Fragile Matter: Nonequilibrium Dynamics,
Metastability and Flow",
      year = 2000,
      address = "Bristol and Philadelphia",
      publisher = "IOP Publishing"}

@article{Bouchaud00b,
  author = "J.-P. Bouchaud",
  title = "Power-laws in economy and finance: some ideas from
physics",
  journal = "Journal of
Quantitative Finance", year=2000}

@article{BouchaudBiroli04,
      author = "J. P. Bouchaud and G. Biroli",
      title = "On the {A}dam-{G}ibbs-{K}irkpatrick-{T}hirumalai-{W}olynes scenario for the viscosity increase of classes",
     journal = "J. Chem. Phys.",
      volume = 121,
      pages = "7347--7354",
      year = 2004}

@incollection{BouchaudCugliandolo98,
      author = "J.-P. Bouchaud and L. Cugliandolo and J. Kurchan and M
          M{\'e}zard",
      title = "Out of Equilibrium Dynamics in Spin Glasses and Other
Glassy
          Systems",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@article{BouchaudDean95,
    author = "J.-P. Bouchaud and D. Dean",
    title = "Aging on Parisi's Tree",
    journal = "J. Phys. I, France",
    year = 1995,
    volume = 5,
    pages = "265--286"}

@article{BouchaudDupuis01,
    author = "J.-P. Bouchaud and V. Dupuis and J. Hammann and E.
Vincent",
    title = "",
    journal = "Phys. Rev. B.",
    year = 2001,
    volume = 65,
    pages = "024439"}

@article{BouchaudGeorges90,
    author = "J.-P. Bouchaud and A. Georges",
    title = "Anomalous Diffusion in Disordered Media: Statistical
        Mechanisms, Models and Physical Applications",
    journal = "Phys. Rep.",
    year = 1990,
    volume = 195,
    pages = "127--293"}

@article{BouchaudKrzakala03,
    author = "J.-P. Bouchaud and F. Krzakala and O. C. Martin",
    title = "Energy exponents and corrections to scaling
           in {I}sing spin glasses",
    journal = "",
    year = 2003,
    volume = " ",
    pages = " ",
  note = "cond-mat/0212070"
}

@article{BouchaudMezard00,
    author = "J.-P. Bouchaud and M. M{\'e}zard",
    title = "Wealth condensation in a simple model of economy",
    journal = "Physica A",
    year = 2000,
    volume = 282,
    pages = "536"}

@article{BouchaudMezard97,
    author = "J.-P. Bouchaud and M. M{\'e}zard",
    title = "Universality Classes for Extreme Value Statistics",
    journal = "J. Phys. A",
    year = 1997,
    volume = 30,
    pages = "7997--8015"}

@phdthesis{Boutet96,
    author = "J. H. {Boutet de Monvel}",
    title = "Physique Statistique et Mod\`eles \`a Liens Al\'eatoires",
    school = "Universit\'e {P}aris {XI}",
    year = 1996,
    address = "Orsay, France"}

@article{BoutetMartin97,
    author = "J. H. {Boutet de Monvel} and O. C. Martin",
    title = "Mean-Field and Corrections for the {E}uclidean Minimum
        Matching Problem",
    journal = "Phys. Rev. Lett.",
    year = 1997,
    volume = 79,
    pages = "167--170"}


@article{BornFock28,
    author = "M. Born and V. A. Fock",
    title = "Beweis des Adiabatensatzes",
    journal = "Zeitschrift fur Physik a Hadrons and Nuclei",
    year = 1928,
    volume = 51,
    pages = "165--180"}

@article{BovierFrohlichXX}

@article{BraunsteinMulet03,
    author = "A. Braunstein and R. Mulet and A. Pagnani and M. Weigt and
R. Zecchina",
    title = " Polynomial iterative algorithms for coloring and analyzing
random graphs",
  journal = "Phys. Rev. E",
   year = 2003,
   volume = "68",
   pages = "036702"}

@article{Bulatov02,
author = {Andrei A. Bulatov},
title = {A Dichotomy Theorem for Constraints on a Three-Element Set},
journal = {Proc. of FOCS 2002},
year = {2002},
issn = {0272-5428},
pages = {649},
doi = {http://doi.ieeecomputersociety.org/10.1109/SFCS.2002.1181990},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@Article{GabayToulouse81,
  title = {Coexistence of Spin-Glass and Ferromagnetic Orderings},
  author = {Gabay, Marc  and Toulouse, G\'erard },
  journal = {Phys. Rev. Lett.},
  volume = {47},
  number = {3},
  pages = {201--204},
  numpages = {3},
  year = {1981},
  month = {Jul},
  doi = {10.1103/PhysRevLett.47.201},
  publisher = {American Physical Society}
}



@article{Gasarch02,
    author = "William I. Gasarch",
    title = "The P=?NP poll",
  journal = "SIGACT News",
   year = 2002,
   volume = "33(2)",
   pages = "34-47"}

@article{GillinSherrington01,
    author = " P. Gillin, H. Nishimori and D.  Sherrington",
    title = "Multispin Ising spin glasses with ferromagnetic interactions",
  journal = " J. Phys. A: Math. Gen.",
   year = 2001,
   volume = "34",
   pages = "2949"}



@article{BraunsteinZecchina04,
   author = {{Braunstein}, A. and {Zecchina}, R.},
    title = "{Survey propagation as local equilibrium equations}",
  journal = {Journal of Statistical Mechanics: Theory and Experiment},
     year = 2004,
    pages = {P06007},
      doi = {10.1088/1742-5468/2004/06/P06007},
   adsurl = {http://adsabs.harvard.edu/abs/2004JSMTE..06..007B},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{Bray94,
    author = "A. J. Bray",
    title = "Theory of phase ordering kinetics",
    journal = "Adv. Phys.",
    year = 1994,
    volume = 43,
    pages = "357"}

@article{BrayFeng87,
    author = "A. J. Bray and S. Feng",
    title = "Percolation Of Order In Frustrated Systems: The
           Dilute +-{J} Spin Glass",
    journal = "Phys. Rev. B",
    year = 1987,
    volume = 36,
    pages = "8456"}

@article{BrayMoore80,
    author = "A. J. Bray and M. A. Moore",
    title = "Metastable States in Spin-Glasses",
    journal = "J. Phys. C Lett.",
    year = 1980,
    volume = 13,
    pages = "L469--L476"}

@article{BrayMoore84,
    author = "A. J. Bray and M. A. Moore",
    title = "Lower Critical Dimension of {I}sing Spin-Glasses: A
        Numerical Study",
    journal = "J. Phys. C Lett.",
    year = 1984,
    volume = 17,
    pages = "L463--L468"}

@article{BrayMoore85,
    author = "A. J. Bray and M. A. Moore",
    title = "Critical Behaviour of the Three-Dimensional {I}sing
        Spin-Glass",
    journal = "Phys. Rev. B",
    year = 1985,
    volume = 31,
    pages = "631--633"}

@inproceedings{BrayMoore86,
    author = "A. J. Bray and M. A. Moore",
    title = "Scaling Theory of the Ordered Phase of Spin-Glasses",
    booktitle = "Heidelberg Colloquium on Glassy Dynamics",
    editor = "J. L. van Hemmen and I. Morgenstern",
    year = 1986,
    volume = 275,
    series = "Lecture Notes in Physics",
    pages = "121--153",
    address = "{B}erlin",
    publisher = "{S}pringer"}

@article{BrayMoore87,
    author = "A. J. Bray and M. A. Moore",
    title = "Chaotic Nature of the Spin-Glass Phase",
    journal = "Phys. Rev. Lett.",
    year = 1987,
    volume = 58,
    pages = "57--60"}

@article{BraySompolinsky86,
    author = "A. J. Bray and H. Sompolinsky and C. Yu",
    title = "On the naive mean-field equations for spin glasses",
    journal = "J. Phys. C.",
    year = 1986,
    volume = 19,
    pages = "6389--6406"}

@article{Brout59,
    author = "R. Brout",
    journal = "Phys. Rev.",
    year = 1959,
    volume = 115,
    pages = 824}

@article{BrunetDerrida00,
      author = "E. Brunet and B. Derrida",
      title = "Probability distribution of the free energy of a directed polymer in a random medium",
      journal = "Phys. Rev. E",
      volume=61,
      pages = "6789--6801",
      year = 2000}

@article{BrunettiKrauth91,
    author = "R. Brunetti and W. Krauth and M. M{\'e}zard and G. Parisi",
    title = "Extensive Numerical Simulations of Weighted Matchings:
        Total Length and Distribution of Links in the Optimal
        Solution",
    journal = "Europhys. Lett.",
    year = 1991,
    volume = 14,
    pages = "295--301"}

@article{BundschuhHwa01a,
    author = "R. Bundschuh and T. Hwa",
  title = " Glass transition in secondary structures formed by random
RNA sequences ",
  note = "cond-mat/0106029"
}

@article{BundschuhHwa01b,
    author = "R. Bundschuh and T. Hwa",
  title = "Statistical mechanics of secondary structures formed by
random RNA sequences",
  note = "cond-mat/0107210"
}

@article{Burkard02,
  author = "R. E. Burkard",
  title = "Selected topics in assignment problems",
  journal = "Discrete Applied Mathematics",
    year = 2002,
    volume = 123,
    pages = "257--302"}

@article{CabasinoMarinari88,
    author = "S. Cabasino and E. Marinari and P. Paolucci and G.
Parisi",
    title = "Eigenstates and limit cycles in the SK model",
    journal = "J. Phys. A",
    year = 1988,
    volume = 21,
    pages = "4201--4210"}

@article{CacciutoMarinari97,
    author = "A. Cacciuto and E. Marinari and G. Parisi",
    title = "A Numerical Study of Ultrametricity in Finite-Dimensional
        Spin Glasses",
    journal = "J. Phys. A",
    year = 1997,
    volume = 30,
    pages = "L263--L269"}

@techreport{CalegariCoray97,
         Author = "P. Calegari and G. Coray and A. Hertz and D. Kobler
and
     P. Kuonen",
         Title = "A Taxonomy of Evolutionary Algorithms in
Combinatorial
     Optimisation",
         institution = "Swiss Federal Institute of Technology",
         year = 1997,
         note = "submitted"}

@article{CaraccioloParisi90a,
    author = "S. Caracciolo and G. Parisi and S. Paternallo and N.
                Sourlas",
    title = "3-d {I}sing spin glasses in a
               magnetic field and mean field theory",
    journal = "Europhys. Lett.",
    year = 1990,
    volume = 11,
    pages = "783"}


@article{CaraccioloParisi90b,
    author = "S. Caracciolo and G. Parisi and S. Paternallo and N.
        Sourlas",
    title = "Low Temperature Behaviour of {3-D} Spin Glasses in a
        Magnetic Field",
    journal = "J. Phys. France",
    year = 1990,
    volume = 51,
    pages = "1877--1895"}

@article{CarpentierLedoussal01,
  author = "D. Carpentier and P. Le Doussal",
  title = "",
  journal = "Phys. Rev. E",
  year = 2001,
  volume = 63,
  pages = "026110"}

@article{CarterBray02,
        author = "A. C. Carter and A. J. Bray and M. A. Moore",
        title = "Aspect-Ratio Scaling and The Stiffness Exponent for
Ising Spin Glasses",
        journal = "Phys. Rev. Lett",
        year = 2002,
        volume = "88",
        pages = "077201"}

@article{Cates90,
        author = "M. E. Cates",
        title = "Microemulsions and the L3 Phase",
        journal = "Colloque de Physique",
        year = 1990,
        volume = "23(51), C7",
        pages = "73-82"}

@article{CavagnaGiardina05,
      author = "A. Cavagna and I. Giardina and G. Parisi",
      title = "Cavity Method for Supersymmetry Breaking Spin Glasses",
     journal = "Phys. Rev. B",
      volume = 71,
      pages = "024422",
      year = 2005}

@article{CerfBoutet97,
    author = "N. J. Cerf and J. H. {Boutet de Monvel} and O. Bohigas and
    O. C. Martin and A. G. Percus",
    title = "The Random Link Approximation for the {E}uclidean Traveling
        Salesman Problem",
    journal = "J. Physique I France",
    year = 1997,
    volume = 7,
    pages = "117--136"}

@article{ChavasFurtlehner05,
      author = "Joel Chavas and Cyril Furtlehner and Marc M\'ezard and Riccardo Zecchina",
      title = "Survey-propagation decimation through distributed local computations",
     journal = "J. Stat. Mech.",
     pages = "P11016",
      year = 2005}


@article{CieplakBanavar90,
    author = "M. Cieplak and J.R. Banavar",
    title = "Scaling of stiffness in {I}sing spin glasses",
    journal = "J. Phys. A.",
    year = 1990,
    volume = 23,
    pages = "4385--4398"}



@ARTICLE{CilibertiMezard05,
   author = {{Ciliberti}, S. and {M{\'e}zard}, M. and {Zecchina}, R.},
    title = "{Lossy Data Compression with Random Gates}",
  journal = {Physical Review Letters},
   eprint = {cond-mat/0504509},
     year = 2005,
    month = jul,
   volume = 95,
   number = 3,
    pages = {038701},
      doi = {10.1103/PhysRevLett.95.038701},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005PhRvL..95c8701C&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{CilibertiMezard05c,
   author = {{Ciliberti}, S. and {M\'ezard}, M. and {Zecchina}, R.},
    title = "{Message passing algorithms for non-linear nodes and data compression}",
  journal = {ArXiv Condensed Matter e-prints},
   eprint = {cond-mat/0508723},
     year = 2005,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005cond.mat..8723C&db_key=PRE},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}


@ARTICLE{CilibertiMezard05b,
   author = {{Ciliberti}, S. and {M{\'e}zard}, M.},
    title = "{The theoretical capacity of the Parity Source Coder}",
  journal = {Journal of Statistical Mechanics: Theory and Experiment},
   eprint = {cond-mat/0506652},
     year = 2005,
    month = oct,
   volume = 10,
    pages = {P10003},
      doi = {10.1088/1742-5468/2005/10/P10003},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005JSMTE..10..003C&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}


@article{CiriaParisi93,
    author = "J.C. Ciria and G. Parisi and F. Ritort and J.J.
        {Ruiz-Lorenzo}",
    title = "The de {A}lmeida-{T}houless line in the Four Dimensional
        {I}sing Spin Glass",
    journal = "J. Physique I France",
    year = 1993,
    volume = 3,
    pages = "2207--2227"}

@article{CoccoDubois03,
      author = "S. Cocco and O. Dubois and J. Mandler and R. Monasson",
      title = "Rigorous decimation-based construction of ground pure states for spin glass models on random lattices",
     journal = "Phys. Rev. Lett.",
      volume = 90,
      pages = "047205",
      year = 2003}

@incollection{CoccoMonasson04,
      author = "S. Cocco and R. Monasson and A. Montanari and G. Semerjian",
      title = "Approximate analysis of search algorithms with ``physical'' methods",
      editor = "G. Istrate, C. Moore, A. Percus",
      booktitle = "Phase transitions and Algorithmic complexity",
      year = 2004}

@article{CookDerrida89,
   author = "J. Cook and B. Derrida",
   title = "Directed polymers in a random medium: 1/d expansion",
   journal = "Europhys. Lett",
   year = 1989,
   volume = "10 (3)",
   pages = "195--199"}

@article{CorrealeLeone06,
   author = {{Correale}, L. and {Leone}, M. and {Pagnani}, A. and {Weigt}, M. and 
	{Zecchina}, R.},
    title = "{Core Percolation and Onset of Complexity in Boolean Networks}",
  journal = {Physical Review Letters},
   eprint = {arXiv:cond-mat/0412443},
     year = 2006,
    month = jan,
   volume = 96,
   number = 1,
    pages = {018101},
      doi = {10.1103/PhysRevLett.96.018101},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvL..96a8101C},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}


@proceedings{Coudert97,
      author = "0. Coudert",
      title = "Exact Coloring Of Real-life Graphs Is Easy",
      editor = "G. Istrate, C. Moore, A. Percus",
      booktitle = "Design Automation Conference, 34th Conference on (DAC'97)",
      pages = "121--126",
      year = 1997}

@book{CoverThomas91,
    author = "T. M. Cover and J. A. Thomas",
    title = "Elements of information theory",
  publisher = "Wiley",
  address = "New-York",
    year = 1991}

@article{CrisantiLeuzzi04,
      author = "A. Crisanti and L. Leuzzi and T. Rizzo",
      title = "Complexity in mean-field spin-glass models: {I}sing $p$-spin",
      journal = "Phys. Rev. B",
      volume = 71,
      pages = "0942024",
      year = 2005}

@article{CrisantiPaladin92,
    author = "A. Crisanti and G. Paladin and J.-J. Sommers and
             A. Vulpiani",
    title = "Replica trick and fluctuations in disordered systems",
    journal = "J. Physique I France",
    year = 1992,
    volume = 2,
    pages = "1325--1332"}

@article{CrisantiSommers95,
    author = "A.~Crisanti and H.-J. Sommers",
    title = "On the TAP approach to the spherical p-spin SG model",
    journal = "J. Phys. I (France)",
    year = 1995,
    volume = 5,
    pages = "805"}

@article{CruzFernandez02,
    author = "A. Cruz and L. A. Fernandez and S. Jimenez and J. J.
Ruiz-Lorenzo and A. Tarancon",
 title = "Off-equilibrium fluctuation-dissipation relations in the 3d
Ising Spin Glass in a magnetic field", year=2002,
note="cond-mat/0209350"}

@article{Cugliandolo02,
    author = "L.~F Cugliandolo",
    title = "Slow non-equilibrium dynamics: analytical methods",
    journal = "Procedings of the Les Houches 2002 LXXVII summer school",
    year = 2002,
  note ="\`A paraitre"}

@article{CugliandoloDean97,
    author = "L. F. Cugliandolo and D. S. Dean and J. Kurchan",
    title = "Fluctuation-Dissipation Theorems and Entropy Production in
        Relaxational Systems",
    journal = "Phys. Rev. Lett.",
    year = 1997,
    volume = 79,
    pages = "2168--2171"}

@article{CugliandoloKurchan93,
    author = "L. F. Cugliandolo and J. Kurchan",
    title = "Analytical solution of the off-equilibrium dynamics of a
long-range spin glass model",
    journal = "Phys. Rev. Lett.",
    year = 1993,
    volume = 71,
    pages = "173"}

@article{CugliandoloKurchan94,
    author = "L. F. Cugliandolo and J. Kurchan",
    title = "On the out of equilibrium dynamics of the long-range
Sherrington-Kirkpatrick model",
    journal = "J. Phys. A",
    year = 1994,
    volume = 27,
    pages = "5749"}

@article{CugliandoloKurchan95,
    author = "L. F.  Cugliandolo and J. Kurchan",
    title = "Weak ergodicity breaking in mean-field spin glass models",
    journal = "Philos. Mag. B",
    year = 1995,
    volume = 71,
    pages = "501"}

@article{CugliandoloKurchan97,
    author = "L. F Cugliandolo and J. Kurchan and L. Peliti",
    title = "Energy flow, partial equilibrium and effective temp\'eratures
in systems with slow dynamics",
    journal = "Phys. Rev. E",
    year = 1997,
    volume = 55,
    pages = "3898"}

@article{CuradoMeunier88,
    author = "E. M. F. Curado and J.-L. Meunier",
    title = "Spin-glass in low dimensions and the {M}igdal-{K}adanoff
           approximation",
    journal = "Physica A",
    year = 1988,
    volume = 149,
    pages = "164--181"}

@article{DeanMajumdar01,
  author ="D.S. Dean and S.N. Majumdar",
  title  ="Extreme Value Statistics of Hierarchically Correlated
Variables:
           Deviation from Gumbel Statistics and Anomalous
Persistence",
  journal="Phys. Rev. E",
  year   ="2001",
  volume =64,
  pages  ="046121--"}





@book{DemboZeitouni93,
    author = "A. Dembo and O. Zeitouni",
    title = "Large Deviations Techniques and Applications",
  publisher = "Jones and Bartlett",
  address = "Boston",
    year = 1993}

@article{Derrida80,
    author = "B. Derrida",
    title = "Random-energy model: Limit of a family of disordered models",
    journal = "Phys. Rev. Lett",
    year = 1980,
    volume = 45,
    pages = "79--82"}

@article{Derrida81,
    author = "B. Derrida",
    title = "Random-Energy Model: An Exactly Solvable Model of Disordered Systems",
    journal = "Phys. Rev. B",
    year = 1981,
    volume = 24,
    pages = "2613--2626"}

@article{Derrida90,
      author = "B. Derrida",
      title = "Directed polymers in a random medium",
     journal = "Physica A",
      volume = 163,
      pages = "71--84",
      year = 1990}

@incollection{Derrida94,
    author = "B. Derrida",
    title = "Non-Self-Averaging Effects in Sums of Random Variables, Spin-Glasses, Random Maps and Random-Walks",
    booktitle = "On Three Levels",
    publisher = "Plenum Press",
    year = 1994,
    editor = "M. Fannes and others"}

@article{DerridaGardner86,
   author = "B. Derrida and E. Gardner",
   title = "Solution of the generalised random energy model",
   journal = "J. Phys. C.",
   year = 1986,
   volume = 19,
   pages = "2253--2274"}

@article{DerridaGardner86b,
   author = "B. Derrida and E. Gardner",
   title = "Magnetic properties and function q(x) of the
            generalised random energy model",
   journal = "J. Phys. C.",
   year = 1986,
   volume = 19,
   pages = "5783--5798"}

@article{DomanyHed01,
  author = "E. Domany and G. Hed and M. Palassini and A.~P. Young",
    title = " State Hierarchy Induced by Correlated Spin Domains in short
range spin glasses",
    journal = "Phys. Rev. B",
    year = 2001,
    volume = 64,
    pages = "224406",
  note="cond-mat/0104264"}

@article{Dominicis78,
        author  = "C. de Dominicis",
        title   = "Dynamics as a substitue for replicas in systems with quenched random impurities",
        journal = "Phys. Rev. B",
        volume = 18,
        pages = "4913",
        year = 1978}

@article{DominicisGoldschmidt89,
        author  = "C. de Dominicis and Y. Goldschmidt",
        title   = "Replica Symmetry Breaking in Finite Connectivity Systems: a Large Connectivity Expansion at Finite and Zero Temperature",
        journal = "J. Phys. A Lett.",
        volume = 22,
        pages = "L775--L781",
        year = 1989}

@article{DominicisHilhorst85,
        author = "C. de Dominicis and H. J. Hilhorst",
        title = "Random (Free) Energies in Spin Glasses",
        journal = "J. Physique Lett.",
        year = 1985,
        volume = 46,
        pages = "L909--L914"}

@article{DominicisKondor83,
    author = "C. de Dominicis and I. Kondor and T. Temesvari",
    title = "Eigenvaues of the Stability Matrix for Parisi Solution of
the Long-range Spin-Glass",
    journal = "Phys. Rev. B",
    year = 1983,
    volume = 27,
    pages = "606-608"}

@article{DominicisKondor91,
    author = "C. de Dominicis and I. Kondor and T. Temesvari",
    title = "Short-Range Corrections to the Order Parameter of the {I}sing Spin-Glass above the Upper Critical Dimension",
    journal = "J. Phys. A Lett.",
    year = 1991,
    volume = 24,
    pages = "L301--L308"}

@incollection{DominicisKondor97,
  author = "C. de Dominicis and I. Kondor and T. Temesvari",
    title = "Beyond the Sherrington-Kirkpatrick Model",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@article{DominicisMottishaw87,
        author  = "C. de Dominicis and P. Mottishaw",
        title   = "Replica Symmetric Solutions in the {I}sing Spin-Glass: the Tree Approximation.",
        journal = "Europhys. Lett.",
        year = 1987,
        volume = 3,
        pages = "87--94"}

@article{DorigoGambardella97,
        author  = "M. Dorigo and L. M. Gambardella",
        title = "Ant Colony System: A Cooperative Learning Approach to the Traveling Salesman Problem",
        journal = "IEEE Transactions on Evolutionary Computation",
        volume = 1,
        pages = "53--66",
        year = 1997}

@article{DotsenkoFranz94,
        author  = "Vik Dotsenko and Silvio Franz and Marc Mezarda",
        title = "Partial annealing and overfrustration in disordered systems",
        journal = "J. Phys. A: Math. Gen.",
        volume = 27,
        pages = "2351",
        year = 1994}

@Book{Dotsenko97,
    author =     {Vic. Dotsenko},
    title =    {Introduction to the Replica Theory of Disordered Statistical Systems},
    publisher =      {Cambridge},
    year =               {2000}
}

@Book{Sinclair93,
    author =     {A. Sinclair},
    title =    {Algorithms for Random Generation and Counting: A Markov Chain Approach},
    publisher =      {Birkhaüser},
    year =               {1993},
    address = " Boston-Basel-Berlin"
}



@article{DrosselBokil00,
        author = "H. Bokil and  B. Drossel and M.~A. Moore",
        title = "The influence of critical behavior on the spin glass phase",
       journal = "Phys. Rev. B",
       volume = 62,
       year=2000,
       page=946}

@article{DrosselBokil00b,
        author = "H. Bokil and  B. Drossel and M.~A. Moore",
        title = "Spin glasses without time-reversal symmetry and the absence of a genuine structural glass",
       journal = "Phys. Rev. E",
       volume = 62,
       year=2000,
       page="7690--7699"}

@Article{DrosselBokil99,
        author = "B. Drossel and H. Bokil and  M.~A. Moore and A.~J. Bray",
        title = "The Link Overlap and Finite Size Effects for the 3D Ising Spin Glass",
       journal = "Eur. Phys. J. B",
       volume = 22,
       year=2000,
       page=369}

@article{DrosselMoore01,
    author = "B. Drossel and M.A. Moore",
    title = "The $\pm{J}$ spin glass in {M}igdal-{K}adanoff approximation",
    journal = "Eur. Phys. J. B",
    year = 2001,
    volume = 22,
    pages = "589--894"}

@article{Dupuis02,
    author = "V. Dupuis",
    title = "Dynamique Lente Des Syst\`emes Magn\'etiques D\'esordonn\'es",
  journal = "",
    year = "2002",
  volume = "",
  pages = "",
  note = "{P}h.D. Thesis, University Paris XI"}

@article{DupuisVincent01,
  author = "V. Dupuis and E. Vincent and J.-P. Bouchaud J. Hammann and A. Ito and H. Aruga Katori",
  title = "Aging, rejuvenation and memory effects in {I}sing and {H}eisenberg spin glasses",
  journal = "Phys. Rev. B",
  year = 2001,
  volume = "64",
  pages = "174204"}

@article{DupuisVincent02,
  author = "V. Dupuis and E. Vincent and M. Alba and J. Hammann",
  title = "Aging, rejuvanation and memory in re-entrant ferromagnet",
  journal = " ",
  year = 2002,
  volume = " ",
  pages = " ",
  note = "cond-mat/0203132"
}

@article{Duxbury03,
      author = "P.M. Duxbury",
      title = "Percolation of frozen order in glassy combinatorial problems",
      note ="cond-mat/0308211",
      year = 2003}

@article{DuxburyJacobs99,
      author = "P.M. Duxbury and D.J. Jacobs and M.F. Thorpe and C. Moukarzel",
      title = "Floppy Modes and the Free Energy: Rigidity and Connectivity Percolation on {B}ethe Lattices",
     journal = "Phys. Rev. E",
      volume = 59,
      pages = "2084--2092",
      year = 1999}

@article{MonthusGarel10,
      author = "C. Monthus and T. Garel",
      title = "Matching between typical fluctuations and large deviations in disordered systems : application to the statistics of the ground state energy in the SK spin-glass model",
     journal = "J. Stat. Mech.",
      volume = "P02023",
      year = 2010}

@article{Wood93,
      author = "R. K. Wood",
      title = "Deterministic Network Interdiction",
     journal = "Mathematical and Computer Modeling",
      volume = 17,
      pages = "1-18",
      year = 1993}

@article{ChenInterian05,
      author = "H. Chen and Y. Interian",
      title = "A model for generating random quantified boolean formulas",
     journal = "In Proceedings of the 19th International joint Conference on Artificial Intelligence (IJCAI 2005)",
      pages = "66-71",
      year = 2005}

@article{McMastersMustin70,
      author = "Alan W. McMasters and Thomas M. Mustin",
      title = "Optimal interdiction of a supply network",
     journal = "Naval Research Logistics Quarterly",
      volume = 17,
      pages = "261–268",
      year = 1970}


@incollection{EenSorensson04,
      author = "Niklas E\'en and Niklas Sorensson",
      title = "An Extensible SAT-solver",
      booktitle = "Theory and Applications of Satisfiability Testing",
      publisher = "Springer Berlin",
      address= "Heidelberg",
      pages = "502--518",
      year = "2004",
}

@incollection{GarelOrland98,
      author = "T. Garel and H. Orland and E. Pitard",
      title = "Protein folding and heteropolymers",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}



@InProceedings{Edwards70,
    author =  {S. F. Edwards},
    booktitle =  {Proceding of the Third International Conference on Amorphous Materials},
  page=279,
  year=1970,
  editor = {R. W. Douglas and B. Ellis, New-york}
}

@article{EdwardsAnderson75,
    author = "S. F. Edwards and P. W. Anderson",
    title = "Theory of Spin-Glasses",
    journal = "J. Phys. F",
    year = 1975,
    volume = 5,
    pages = "965--974"}

@unpublished{BravyiMoore09,
    author = "Sergey Bravyi, Cristopher Moore, Alexander Russell",
    title = "Bounds on the quantum satisfibility threshold",
    year = 2009,
    note = "arXiv:0907.1297v2"}

@unpublished{Scardicchio_com,
    author = "A. Scardicchio",
    year = 2010,
    note = "in preparation"}

@article{LaumannMoessner09,
    author = "C. R. Laumann and R. Moessner and A. Scardicchio and S. L. Sondhi",
    title = "Phase transitions and random quantum satisfiability",
    journal = "Quant. Inf. and Comp.",
    year = 2010,
    volume = 10,
    pages = "1-15"}

@article{LaumannLauchli10,
    author = "C. R. Laumann and A. M. Lauchli and R. Moessner and A. Scardicchio and S. L. Sondhi",
    title = "Product, generic, and random generic quantum satisfiability",
    journal = "Phys. Rev. A",
    year = 2010,
    volume = 81,
    pages = "062345"}

@book{Ellis85,
    author = "R. S. Ellis",
    title = "Entropy, Large Deviations, and Statistical Mechanics",
  publisher = "Springer-Verlag",
  address = "New-York",
    year = 1985}

@article{Ellis95,
      author = "R. S. Ellis",
      title = "An overview of the theory of large deviations and applications to statistical physics",
     journal = "Scand. Acturial J.",
      volume = 1,
      pages = "97--142",
      year = 1995}

@article{EngelMonasson04,
      author = "A. Engel and R. Monasson and A. K. Hartmann",
      title = "On large deviation properties of {E}rd{\H{o}}s-{R}\'enyi random graphs",
     journal = "J. Stat. Phys.",
      volume = 117,
      pages = "387",
      year = 2004}

@article{ErdosRenyi60,
      author = "P. Erd{\H{o}}s and A. R{\'e}nyi",
      title = "On the evolution of random graphs",
      journal = "Publ. Math. Inst. Hungar. Acad. Sci.",
      volume = 5,
      pages = "17--61",
      year = 1960}

@article{ErdosRenyi59,
	author="P. Erd{\H{o}}s and A. R{\'e}nyi",
	title="On random graphs",
	journal="Publ. Math. Debrecen",
	volume="6",
	pages="290--297",
	year=1959
}


@unpublished{FarhiGoldstone00,
    author = {{Farhi}, E. and {Goldstone}, J. and {Gutmann}, S. and {Sipser}, M.
	},
    title = "{Quantum Computation by Adiabatic Evolution}",
    note = "arXiv:quant-ph/0001106v1",
    year = 2000,
}



@article{Fisher86,
    author = "D. S. Fisher",
    title = "Scaling and Critical Slowing Down in Random-Field
        {I}sing Systems",
    journal = "Phys. Rev. Lett.",
    year = 1986,
    volume = 56,
    pages = "416--419"}


@book{FischerHertz91,
    author = "K. H. Fischer and J. A. Hertz",
    title = "Spin-Glasses",
    publisher = "Cambridge University Press",
    year = 1991,
    address = "Cambridge",
    volume = 1,
    series = "Cambridge Studies in Magnetism"}

@article{Fisher86,
    author = "D. S. Fisher",
    title = "Scaling and Critical Slowing Down in Random-Field
        {I}sing Systems",
    journal = "Phys. Rev. Lett.",
    year = 1986,
    volume = 56,
    pages = "416--419"}

@article{FisherHuse86,
    author = "D. S. Fisher and D. A. Huse",
    title = "Ordered Phase of Short-Range {I}sing Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1986,
    volume = 56,
    pages = "1601--1604"}

@article{FisherHuse87,
    author = "D. S. Fisher and D. A. Huse",
    title = "Absence of Many States in Realistic Spin-Glasses",
    journal = "J. Phys. A Lett.",
    year = 1987,
    volume = 20,
    pages = "L1005--L1010"}

@article{FisherHuse88,
    author = "D. S. Fisher and D. A. Huse",
    title = "Equilibrium Behavior of the Spin-Glass Ordered Phase",
    journal = "Phys. Rev. B",
    year = 1988,
    volume = 38,
    pages = "386--411"}

@article{FisherHuse91,
    author = "D. S. Fisher and D. A. Huse",
    title = "Directed path in a random potential",
    journal = "Phys. Rev. B",
    year = 1991,
    volume = 43,
    pages = "10728--10742"}

@article{FisherSompolinsky85,
    author = "D. S. Fisher and H. Sompolinski",
    title = "Scaling in Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1985,
    volume = 54,
    pages = "1063--1066"}

@Article{FranzLeone01,
  title = {Exact Solutions for Diluted Spin Glasses and Optimization Problems},
  author = {Franz, Silvio  and Leone, Michele  and Ricci-Tersenghi, Federico  and Zecchina, Riccardo },
  journal = {Phys. Rev. Lett.},
  volume = {87},
  number = {12},
  pages = {127209},
  numpages = {4},
  year = {2001},
  month = {Aug},
  doi = {10.1103/PhysRevLett.87.127209},
  publisher = {American Physical Society}
}

@article{FranzLeone02,
        author = "S. Franz and M. Leone and A. Montanari and F. Ricci-Tersenghi",
        title = "The dynamic phase transition for decoding algorithms",
        year = 2002,
        journal = "Phys. Rev. E",
        volume = "66",
        pages = "046120"}

@article{FranzLeone03,
        author = "S. Franz and M. Leone",
        title = "Replica bounds for optimization problems
                 and diluted spin systems",
        year = 2003,
        journal = "J. Stat. Phys.",
        volume = "3-4",
        pages = "535--564"}

@article{FranzLeone03b,
        author = "Silvio Franz and Michele Leone and Fabio Lucio Toninelli",
        title = "Replica bounds for diluted non-Poissonian spin systems",
        year = 2003,
        journal = "J. Phys. A: Math. Gen.",
        volume = "36",
        pages = "10967-10985"}

@article{FranzMezard01,
        author = "S. Franz and M. M{\'e}zard and
        F. Ricci-Tersenghi and M. Weigt and R. Zecchina",
        title = "A ferromagnet with a glass transition",
        journal = "Europhys. Lett.",
        volume = 55,
        pages = "465",
        year = 2001}

@article{FranzMezard94a,
        author = "S. Franz and M. M{\'e}zard",
        title = "Off equilibrium glassy dynamics : A simple case",
        journal = "Europhys. Lett.",
        volume = 26,
        pages = "209",
        year = 1994}

@article{FranzMezard94b,
        author = "S. Franz and M. M{\'e}zard",
        title = "On mean field glassy dynamics out of equilibrium",
        journal = "Physica A",
        volume = 210,
        pages = "48",
        year = 1994}

@article{FranzMezard98,
        author = "S. Franz and M. M{\'e}zard and G. Parisi and L. Peliti",
        title = "Measuring Equilibrium Properties in Aging Systems",
        journal = "Phys. Rev. Lett.",
        volume = 81,
        pages = "1758--1761",
        year = 1998}

@article{FranzNifle95,
        author = "S. Franz and M. Ney-Nifle",
        title="On chaos in mean-field spin glasses",
        journal="J. Phys. A",
        volume=28,
        year=1995,
        pages="2499"}


@article{FranzParisi92,
        author = "S. Franz and G. Parisi and M. A. Virasoro",
        title = "The replica method on and off equilibrium",
        year = 1992,
        journal = "J. Phys. I France",
        volume = "2",
        page="1869-1880"}

@article{FranzParisi94,
        author = "S. Franz and G. Parisi and M. A. Virasoro",
        title = "Interfaces and lower critical dimension in a spin
                 glass model.",
        year = 1994,
        journal = "Jour. de Phys.",
        volume = "4",
        page="1657"}

@ARTICLE{FranzParisi95,
   author = {{Franz}, S. and {Parisi}, G.},
    title = "{Recipes for Metastable States in Spin Glasses}",
  journal = {Journal de Physique I},
     year = 1995,
    month = nov,
   volume = 5,
    pages = {1401-1415},
   adsurl = {http://adsabs.harvard.edu/abs/1995JPhy1...5.1401F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{FranzParisi97,
  title = {Phase Diagram of Coupled Glassy Systems: A Mean-Field Study},
  author = {Franz, Silvio  and Parisi, Giorgio },
  journal = {Phys. Rev. Lett.},
  volume = {79},
  number = {13},
  pages = {2486--2489},
  numpages = {3},
  year = {1997},
  month = {Sep},
  doi = {10.1103/PhysRevLett.79.2486},
  publisher = {American Physical Society}
}


@Article{FranzParisi98,
  title = {EFFECTIVE POTENTIAL IN GLASSY SYSTEMS : THEORY AND SIMULATIONS},
  author = {Franz, Silvio  and Parisi, Giorgio },
  journal = {Physica A},
  volume = {261},
  number = {3-4},
  pages = {317-339},
  year = {1998},
}



@article{FranzRicci99,
        author = "S. Franz and F. Ricci-Tersenghi",
        title = "Ultrametricity in {3D} {E}dwards-{A}nderson Spin Glasses",
        year = 1999,
    note = "cond-mat/9903130"}

@article{Friedberg85,
        author = "R. Friedberg",
        title = "The $1/d$ Expansion of the {E}den Model",
        journal = "Phys. Lett. A",
        volume = 112,
        pages = "129--132",
        year = 1985}

@article{FriedgutKalai96,
      author = "E. Friedgut and G. Kalai",
      title = "Every monotone property has a sharp threshold",
      journal = "Proc. Amer. Math. Soc.",
      volume = 124,
      pages = "2993--3002",
      year = 1996}

@article{FuAnderson86,
    author = "Y. Fu and P. W. Anderson",
    title = "Application of Statistical Mechanics to {NP}-Complete
        Problems in Combinatorial Optimization",
    journal = "J. Phys. A",
    year = 1986,
    volume = 19,
    pages = "1605--1620"}

@book{Galambos87,
  author = "J. Galambos",
  title = "The asymptotic Theory of Extreme Order Statistics",
  publisher = "R.E. Krieger Publishing Co.",
  year = "1987",
  address = "Malabar, Florida"}

@article{Gallager62,
   author = "Robert G. Gallager",
   title = "Low-density parity check codes",
   journal = "IEEE Trans. Inform. Theory",
   year = 1962,
   volume = "8",
   pages = "21--28"}

@book{Gallager68,
  author = "R. G. Gallager",
  title = "Information theory and reliable communication",
  publisher = "John Wiley and Sons",
  year = "1968",
  address = "New York"}

@article{GamarnikNowiski03,
      author = "D. Gamarnik and T. Nowicki and G. Swirscsz",
      title = "Maximum Weight Independent Sets and Matchings in Sparse Random Graphs. Exact Results using the Local Weak Convergence Method",
      note = "math.PR/0309441",
      year = 2003}

@article{Gardner88,
      author = "E. Gardner",
      title = "The space of interactions in neural network models",
      journal = "J. Phys. A: Math. Gen.",
      volume = 21,
      pages = "257--270",
      year = 1988}

@article{Gardner85,
      author = "E. Gardner",
      title = "Spin glasses with p-spin interactions",
      journal = "Nuclear Physics B",
      volume = 257,
      pages = "747--765",
      year = 1985}

@article{GardnerDerrida89,
    author = "E. Gardner and B. Derrida",
    title = "The Probability Distribution of the Partition Function of the Random Energy Model",
    journal = "J. Phys. A",
    year = 1989,
    volume = 22,
    pages = "1975--1981"}

@incollection{GarelOrland98,
      author = "T. Garel and H. Orland and E. Pitard",
      title = "Protein folding and heteropolymers",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@book{GareyJohnson79,
    author = "M.R. Garey and D.S. Johnson",
    title = "Computers and intractability: A guide to the theory of NP-completeness",
    publisher = "Freeman",
    address = "San Francisco",
    year = 1979}

@book{Georgii88,
    author = "H.-O. Georgii",
    title = "Gibbs Measures and Phase Transitions",
    publisher = "De Gruyter",
    address = "Berlin",
    year = 1988}


@article{GeorgesMezard90,
        author  = "A. Georges and M. M{\'e}zard and J. S. Yedidia",
        title   = "Low-Temperature Phase of the {I}sing Spin-Glass on a Hypercubic Lattice",
        journal = "Phys. Rev. Lett.",
          year = 1990,
        volume = 64,
        pages = "2937--2940"}



@book{GestelandAtkins93,
    author = "R.F. Gesteland and J.F. Atkins",
    title = "The RNA world: the nature of modern RNA suggests a prebiotic RNA world",
    publisher = "Cold Spring Harbor Laboratory Press",
    year = 1993,
    address = "NewYork"}

@book{GloverLaguna97,
        Author = "F. Glover and M. Laguna",
        Title = "Tabu Search",
        Year = 1997,
        address = "Boston, MA",
        Publisher = "Kluwer Academic Publishers",
        annotate = "Second printing"}

@book{Goldberg89,
        Author = "D. E. Goldberg",
        Title = "Genetic Algorithms in Search, Optimization, and Machine Learning",
        Year = 1989,
        address = "Reading MA",
        Publisher = "Addison--Wesley",
        keyword = "algorithm, optimization",
        annotate = "This textbook is an easy to read introduction to Genetic algorithms, which can be used as heuristics for combinatorial optimization problems."}


@article{GrannanHetzel91,
        author  = "E. R. Grannan and R. E. Hetzel",
        title   = "Susceptibility of Two-, Three-, and Four-Dimensional Spin Glasses in a Magnetic Field",
        journal = "Phys. Rev. Lett.",
        year = 1991,
        volume = 67,
        pages = "907--910"}

@article{GrassbergerFreund90,
        author  = "P. Grassberger and H. Freund",
        title   = "An efficient heuristic algorithm for Minimum Matching",
        journal = "Z. Oper. Res.",
        year = 1990,
        volume = 34,
        pages = "239--253"}

@article{GrinsteinJayaprakash79,
        author="J. Grinstein and J. Jayaprakash and M. Wortis",
        title="Ising magnets with frustration: {Z}ero-temperature properties from series expansions",
        journal="Phys. Rev. B",
        year=1979,
        volume = 19,
        pages="260--264"}

@article{GrossMezard84,
        author  = "D.J. Gross and M. M\'ezard",
        title   = "The simplest spin glass",
        journal = "Nucl. Phys. B",
        year = 1984,
        volume = 240,
        pages = "431"}

@article{GrundelOliveira04,
  author = "D. A. Grundel and C. A. S. Oliveira and P. M. Pardalos",
  title = "On the asymptotic properties of random multidimensional assignment problems",
  journal = "Journal of Optimization Theory and Applications",
    year = 2004,
    volume = 122,
    pages = ""}

@article{Guerra02,
        author  = "F. Guerra",
        title = "Broken Replica Symmetry Bounds in the Mean Field Spin
Glass Model",
         year=2002,
        note="cond-mat/0205123"}

@article{Guerra96,
        author  = "F Guerra",
        journal = "Int. J. Mod. Phys. B",
        year = 1996,
        volume = 10}

@article{GuerraToninelli02,
        author  = "F. Guerra and F. L. Toninelli ",
        title = "The Thermodynamic Limit in Mean Field Spin Glass Models",
        year = 2002,
 note="cond-mat/0204280"}

@book{Gumbel58,
        author  = "E. J. Gumbel",
        title = "Statistics of Extremes",
        year = "1958",
        publisher = {Columbia University Press},
}

@article{Hales98,
        author  = "T. C. Hales",
        title = "An overview of the {K}epler conjecture",
        year = 1998,
        note = "available at
http://www.math.pitt.edu/$\sim$thales/PUBLICATIONS/"}

@Article{HasenbuschPelissetto08,
  title = {Critical behavior of three-dimensional Ising spin glass models},
  author = {Hasenbusch, Martin  and Pelissetto, Andrea  and Vicari, Ettore },
  journal = {Phys. Rev. B},
  volume = {78},
  number = {21},
  pages = {214205},
  numpages = {23},
  year = {2008},
  month = {Dec},
  doi = {10.1103/PhysRevB.78.214205},
  publisher = {American Physical Society}
}



@article{AppelHaken77,
   author = "K. Appel and W. Haken",
   title = "Every planar map is four colorable. Part I. Discharging",
   journal =  "Illinois J. Math.",
   volume = "21", 
   page = "421",
   year = "1977" 
}

@article{AppelHaken77b,
   author = "K. Appel and W. Haken",
   title = "Every planar map is four colorable. II. Reducibility",
   journal =  "Illinois J. Math.",
   volume = "21", 
   page = "491",
   year = "1977" 
}


@article{Halpin-HealyZhang86, 
author  = "T. Halpin-Healy and Y.C. Zhang", 
journal = "Physics Reports",
 year = 1995,
volume = 254,
 pages = 215,
}

@article{HammannVincent00, 
author  = "J.Hammann and E.Vincent and V.Dupuis and M.Alba and M.Ocio and J.-P.Bouchaud", 
title = "Comparative review of aging properties in spin glasses and other
disordered materials", 
journal = "J. Phys. Soc. Jpn",
 year =  2000,
volume = "69 Suppl.A",
 pages = "206--211",
}

@article{Hartmann00,
 author  = "A. K. Hartmann",
 title = "How to evaluate ground-state landscapes of spin glasses thermodynamical correctly",
 journal = "Eur. Phys. Jour. B",
 year = 2000,
 volume = 13,
 pages = "539--545",
 note="cond-mat/9906270"}


@article{Hartmann01,
 author  = "A. K. Hartmann",
 title = "Ferromagnetic-spin glass transition in four-dimensional random-bond {I}sing model",
 year = 2001,
 journal = "Phys. Rev. B",
 volume = 64,
 pages = "224430",
 note="cond-mat/0107583"}

@article{Hartmann01Comment,
 author  = "A. K. Hartmann",
 title = "Comment on 'Glassy transition in a disordered model for the RNA secondary structure'",
 journal = "Phys. Rev. Lett.",
 year = 2001,
 volume = 86,
 pages = "1382"}

@article{Hartmann01b,
 author  = "A. K. Hartmann",
 title = "Ground-state clusters of two-, three- and four-dimensional $\pm {J}$ {I}sing spin glasses",
 year = 2001,
 journal = "Phys. Rev. E",
 volume = 63,
 pages = "016106",
 note="cond-mat/9902120"}

@article{Hartmann96,
          author ="A. K. Hartmann",
          title = "Cluster-Exact Approximation of Spin Glass Groundstates",
           year = 1996,
           journal = "Physica A",
           volume = 224,
           pages = "480",
           note = "cond-mat/9504065",
}

@article{Hartmann97,
         author ="A. K. Hartmann",
         title = "Evidence for existence of many pure ground states in 3d $\pm {J}$ Spin Glasses",
          year = 1997,
          journal = "Europhys. Lett.",
          volume = 40,
          pages = "429-434",
          note = "cond-mat/9704187"}

@article{DebenedettiStillinger01,
         author ="Debenedetti and Stillinger ",
         title = "Supercooled liquids and the glass transition",
          year = 2001,
          journal = "Nature",
          volume = 410,
          number = "6825",
          pages = "259-267",
         }



@article{Hartmann98,
        author  = "A. K. Hartmann",
        title = "Are Ground States of 3d $\pm {J}$ Spin Glasses Ultrametric?",
        journal = "Europhys. Lett",
        year = 1999,
          volume = 44,
          pages = "249",
        note = " cond-mat/9804325"}

@article{Hartmann99,
        author  = "A. K. Hartmann",
        title = "Scaling of Stiffness Energy for 3d $\pm {J}$ {I}sing Spin Glasses",
        journal = "Phys. Rev. E",
        year = 1999,
    volume = 59,
    pages = "84--87"}

@article{Hartmann99b,
    author = "A. K. Hartmann",
    title = "Ground-state landscape of 2d $\pm {J}$ {I}sing spin glasses",
    journal = "Eur. Phys. J. B",
  volume = "8",
  pages = "619",
    year =  "1999"}

@article{Hartmann99c,
    author = "A. K. Hartmann",
    title = "Ground-state behavior of the 3d $\pm {J}$ random-bond {I}sing model",
    journal = "Phys. Rev. B "    ,
  volume = "59",
  pages = "3617--3625",
    year =  "1999"}

@article{Hartmann99d, 
author  = "A. K. Hartmann", 
title = "Calculation of ground states of four-dimensional + or - {J} {I}sing spin glasses",
 journal = "Phys. Rev. E",
 year = 1999,
 volume = 60,
 pages = "5135",
 note="cond-mat/9904296"}

@article{HartmannRicci01,
 author  = "A. K. Hartmann and F. Ricci-Tersenghi",
 title = "Equilibrium sampling of complex landscapes at low temperatures: the three-dimensional $\pm {J}$ Ising spin glass",
 year = 2001,
 note = "cond-mat/0108307, unpublished"
}

@article{HartmannRicci02,
 author  = "A. K. Hartmann and F. Ricci-Tersenghi",
 title = "Direct sampling of complex landscapes at low temperatures: the three-dimensional $\pm {J}$ {I}sing spin glass",
 year = 2002,
 journal = "Phys. Rev. B",
 volume = 66,
 pages = "224419",
 note = "cond-mat/0108307"
}

@Book{HartmannRieger02,
  Editor = "A. K. Hartmann and H. Rieger",
    title =    "Optimization Algorithms in Physics",
    publisher =      {Wiley-VCH},
    year =               {2002},
}
   

@article{HartmannYoung01,
 author  = "A. K. Hartmann and A.P. Young",
 title = "Lower Critical Dimension of Ising Spin Glasses",
 year = 2001,
 journal = "Phys. Rev. B",
 volume = 64,
 pages = "180404",
 note="cond-mat/0107308"}

@article{HartmannYoung02,
 author  = "A. K. Hartmann and A.P. Young",
 title = "Large-Scale, Low-Energy Excitations in the Two-Dimensional
Ising Spin Glass",
 year = 2002,
 note = "cond-mat/0205659"}

@article{HatanoGubernatis00,
 author  = "N. Hatano and J.E. Gubernatis",
 title = "Evidence for the droplet picture in the 3D $\pm {J}$ spin
glass",
 note = "cond-mat/0008115 "}

@article{Hayes97,
 author  = "B. Hayes",
 title = "Can't get no satisfaction",
 year = 1997,
 journal = "American scientist",
 volume = 85,
 pages = "108--112"}

@article{HedHartmann00a,
 author  = "G. Hed and A.K. Hartmann and D. Stauffer and E. Domany",
 title = "Spin domains generate hierarchical ground state structure in ${J}=\pm {1}$ spin glasses",
 journal = "Phys. Rev. Lett.",
 year = 2001,
 volume = 86,
 pages = "3148--3151",
 note="cond-mat/0007356"}

@article{HedHartmann01,
 author  = "G. Hed and A.K. Hartmann and E. Domany",
 title = "Correct extrapolation of overlap distribution in spin glasses",
 note = "cond-mat/0012451",
 journal = "Europhys. Lett.",
 year = 2001,
 volume = 55,
 pages = "112",
 note="cond-mat/0012451"}

@article{HerissonOcio01,
 author  = "D. Herisson and M. Ocio",
 title = "Fluctuation-dissipation ratio of a spin glass in the aging regime",
 journal = "Phys. Rev. Lett.",
 year = 2001,
 volume = 88,
 pages = "257202"}

@inproceedings{HertzKobler98,
    author = "A. Hertz and D. Kobler",
    title = "A Framework for the description of population based methods",
    booktitle = "Proceedings of Euro XVI",
    year = 1998}

@book{HertzKrogh91,
        author  = "J. Hertz and A. Krogh R.~G. Palmer",
        title   = "Introduction to the theory of Neural Computation",
        year = 1991,
        publisher = "Addison-Wesley",
        address = "Redwood city, CA"}

@article{Higgs96,
 author  = "P. G. Higgs",
 journal = "Phys. Rev. Lett.",
  year = 1996,
  volume = 76,
  pages = "704--708"
}

@article{HoggWilliams94,
      author = "T. Hogg and C. Williams",
      title = "The hardest constraint problems : a double phase transition",
      journal = "Artificial Intelligence",
      volume = 69,
      pages = "359--377",
      year = 1994}



@book{Holland75,
        author  = "J. H. Holland",
        title   = "Adaptation in Natural and Artificial Systems",
        year = 1975,
        publisher = "University of Michigan Press",
        address = "Ann Arbor",}

@article{Hopfield82,
 author  = "J. J. Hopfield",
 title = "Neural networks and physical systems with emergent collective computational properties",
 journal = "Proc. Nat. Acad. Sci. USA",
  year = 1982,
  volume = 79,
  pages = "2554--2558"
}

@article{Hopfield84,
 author  = "J. Hopfield",
 journal = "Proc. Nat. Acad. Sci. USA",
  year = 1984,
  volume = 81,
  pages = "3088--9092"
}

@article{Houdayer01,
  author = "J. Houdayer",
    title = "A Cluster Monte Carlo Algorithm for 2-Dimensional Spin Glasses",
    journal = "Eur. Phys. Jour. B",
    year = 2001,
    volume = 22,
    pages = "479"}

@article{Houdayer02,
  author = "J. Houdayer",
    title = "The wormhole move: A new algorithm for polymer simulations",
    journal = "",
    year = 2002,
    volume = "",
    pages = ""}

@article{HoudayerBoutet98,
  author = "J. Houdayer, J. H. Boutet de Monvel and O.C. Martin",
  title = "Comparing Mean Field and Euclidean Matching Problems",
  journal = "Eur. Phys. J. B",
    year = 1998,
    volume = 6,
    pages = "383--393"}

@article{HoudayerBoutet98,
    author = "J. Houdayer and J. H. {Boutet de Monvel} and O. C. Martin",
    title = "Comparing Mean Field and {E}uclidean Matching Problems",
    journal = "Eur. Phys. Jour. B",
    year = 1998,
    volume = 6,
    pages = "383--393"}

@article{HoudayerKrzakala00,
    author = "J. Houdayer and F. Krzakala and O. C. Martin",
    title = "Large-Scale Low-Energy excitations in 3-d Spin Glasses",
    year = 2000,
    journal = "Eur. Phys. J. B.",
  volume = 18,
  pages = "467--477",
    note = "cond-mat/0009382"}

@article{HoudayerMartin00a,
    author = "J. Houdayer and O. C. Martin",
    title = "Reply to Comment on ``Ising Spin Glasses in a Magnetic Field''",
    year = 2000,
  journal = "Phys. Rev. Lett.",
  volume = 84,
  pages = "1057",
  note = "cond-mat/9910333"}

@article{HoudayerMartin00b,
    author = "J. Houdayer and O. C. Martin",
    title = "A geometrical picture for finite dimensional spin glasses",
    year = 2000,
  journal = "Europhys. Lett.",
  volume = 49,
  pages = "794-800",
  note = "cond-mat/9909203"}

@article{HoudayerMartin01, 
author = "J. Houdayer and O. C. Martin",
        title = "A hierarchical approach for computing spin glass ground states", year = "2001", 
journal = "Phys. Rev. E",
        volume = "64", 
pages = "056704", 
note = "cond-mat/0105617"}

@article{HoudayerMartin98,
    author = "J. Houdayer and O. C. Martin",
    title = "Droplet Phenomenology and Mean Field in a Frustrated Disordered System",
    journal = "Phys. Rev. Lett.",
    year = 1998,
    volume = 81,
    pages = "2554--2557"}

@article{HoudayerMartin99a,
    author = "J. Houdayer and O. C. Martin",
    title = "{I}sing Spin Glasses in a Magnetic Field",
    journal = "Phys. Rev. Lett.",
    year = 1999,
    volume = 82,
    pages = "4934--4937",
  note = "cond-mat/9811419"}

@article{HoudayerMartin99b,
    author = "J. Houdayer and O. C. Martin",
    title = "Renormalization for Discrete Optimization",
    year = 1999,
    journal = "Phys. Rev. Lett.",
  volume = 83,
  pages = "1030--1033",
    note = "cond-mat/9901276"}

@PhdThesis{HoudayerThesis,
    author =             {J. Houdayer},
    title =              {Verres de Spins et Optimisation Combinatoire},
    school =             {Universit\'e Paris XI},
    year =               {1999}
}

@article{HukushimaNemoto96,
    author = "K. Hukushima and K. Nemoto",
    title = "Exchange Monte Carlo Method and Application to Spin Glass
        Simulations",
    year = 1996,
  journal = "J. Phys. Soc. Jpn.",
  volume = 65,
  pages = "1604",
    note = "cond-mat/9512035"}

@article{HuseFisher87,
    author = "D. A. Huse and D. S. Fisher",
    title = "Pure States in Spin-Glasses",
    journal = "J. Phys. A Lett.",
    year = 1987,
    volume = 20,
    pages = "L997--L1003"}

@article{HuseFisher91, 
author = "D. A. Huse and D. S. Fisher",
    title = "On the behavior of {I}sing spin glasses in a uniform magnetic field",
    journal = "J. Phys. I. France",
    year = 1991,
    volume = 1,
    pages = "621"}

@article{IbaHukushima00,
    author = "Y. Iba and K. Hukushima",
    title = "Identification of Metastable States in Finite Temperature
             Simulations: A Self-Organization Approach",
    journal = "Prog. Theo. Phys. Supp.",
    volume = 138,
    year = 2000,
    pages = "462--463"}

@article{ImryMa75,
    author = "Y. Imry and S.K. Ma",
    title ="Random-Field Instability of the Ordered State of Continuous Symmetry",
    year = "1975",
    journal = "Phys. Rev. Lett.",
    volume = "35",
    pages = "1399-1401"}

@article{ItoArugakatori94,
    author = "A. Ito and H. Aruga Katori",
    title ="",
    year = "1994",
    journal = "J. Soc. Japan",
    volume = "63",
    pages = "3122"}

@article{Luczak91,
    author = "T. Luczak",
    title ="The chromatic number of random graphs",
    year = "1991",
    journal = "Combinatorica ",
    volume = "11",
    pages = "45"}


@article{Janis05,
    author = "V. Jani\v{s}",
    title =" Stability of solutions of the Sherrington-Kirkpatrick model with respect to replications of the phase space",
    year = "2005",
    journal = "Phys. Rev. B",
    volume = "71",
    pages = "214403"}


@book{JansonLuczak00,
    author = "S. Janson and  T. Luczak and  A. Rucinski",
    title = "Random graphs",
    publisher = "Wiley",
    address = "New-York",
    year = 2000}


@incollection{JohnsonMcGeoch97,
        author  = "D. S. Johnson and L. A. McGeoch",
        title   = "The Traveling Salesman Problem: A Case Study in Local Optimization",
        booktitle = "Local Search in Combinatorial Optimization",
        publisher = "J. Wiley \& and Sons",
        year = 1997,
        editor = "E. H. L. Aarts and J. K. Lenstra",
        address = "New York",
pages = "215-310"}


@article{JonasonNordblad99,
    author = "K. Jonason and P. Nordblad and E. Vincent and J. Hammann and J.-P. Bouchaud",
    title = "Memory Interference effects in Spin Glasses",
    year = 1999,
    note = "cond-mat/9904410"}

@article{Jonasson02,
    author = "J. Jonasson",
    title = "Uniqueness of uniform random colorings of regular trees",
    journal = "Statistics and Probability Letters",
    volume = "57",
    year = 2002,
    pages = "243--248"}


@article{JonasonVincent98,
    author = "K. Jonason and E. Vincent and J. Hammann and J.P. Bouchaud and P. Nordblad",
    title = "Memory and Chaos Effects in Spin Glasses",
    year = 1998,
  journal = "Phys. Rev. Lett.",
  volume = "81",
  pages = "3243",
    note = "cond-mat/9904410"}

 @article{Derrida85,
   author = "B. Derrida",
   title = "A generalization of the random energy model which includes correlations between energies",
   journal = "J. Phys. Lett. (France)",
   year = 1985,
   volume = "46",
   pages = "401"}

@article{JonssonJonason99,
    author = "T. Jonsson and K. Jonason and P. J{\"o}nsson and P. Nordblad",
    title = "Nonequilibrium Dynamics in a Three-Dimensional Spin Glass",
    year = 1999,
        journal = "Phys. Rev. B",
        volume = 59,
        pages = "8770--8777"}

@article{JonssonYoshino02,
    author = "P.E. J{\"o}nsson and H. Yoshino and P. Nordblad",
    title = "Symmetrical temperature-chaos effect with positive and negative temperature shifts in a spin glass",
    year = 2002,
  journal = "Phys. Rev. Lett.",
  volume = 89,
  pages = "097201"}

 @article{DerridaSpohn88,
    author = "B. Derrida and H. Spohn",
    title = "Polymers on disordered trees, spin glasses, and traveling waves",
    journal = "J. Stat. Phys.",
    year = 1988,
    volume = 51,
    pages = "817--840"}

 @article{DerridaToulouse85,
    author = "B. Derrida and G. Toulouse",
    title = "Sample to sample fluctuations in the random energy model",
    journal = "J. Phys. Lett.",
    year = 1985,
    volume = 46,
    pages = "L223--L228"}

@Article{GrossKanter85,
title = {Mean-field theory of the Potts glass},
author = {Gross, D. J. and Kanter, I.  and Sompolinsky, H. },  
journal = {Phys. Rev. Lett.},
volume = {55},  
number = {3},
pages = {304--307},
numpages = {3}, 
year = {1985},
month = {Jul},
doi = {10.1103/PhysRevLett.55.304}, 
publisher = {American Physical Society}}


@ARTICLE{KadowakiNishimori98,
   author = {{Kadowaki}, T. and {Nishimori}, H.},
    title = "{Quantum annealing in the transverse Ising model}",
  journal = {\pre},
 keywords = {Quantum statistical mechanics, Spin-glass and other random models, Information theory and communication theory},
     year = 1998,
    month = nov,
   volume = 58,
    pages = {5355-5363},
      doi = {10.1103/PhysRevE.58.5355},
   adsurl = {http://adsabs.harvard.edu/abs/1998PhRvE..58.5355K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{KanterSompolinsky87,
title = {Graph optimisation problems and the Potts glass},
author = {Kanter, I.  and Sompolinsky, H. },  
journal = {J. Phys. A: Math. Gen},
volume = {20},  
pages = {L673--L679},
year = {1987},
}

@article{KabashimaSaad04,
        author = "Y. Kabashima and D. Saad",
        title = "Statistical mechanics of low-density parity-check codes",
        journal = "J. Phys. A: Math. Gen",
        year = 2004,
        volume = "37",
        pages = "R1--R43"}

@unpublished{Kac68,
 author  = "M. Kac",
 title   = "Trondheim Theoretical Physics Seminar",
 note = "Nordita Publ. No. 286" ,
 year = 1968}

@PhDthesis{Mora07,
 author  = "T. Mora",
 title   = "G\'eom\'etrie et inf\'erence dans l'optimisation et en th\'eorie de l'information",
 school = "Universit\'e Paris-Sud",
 note = "http://tel.archives-ouvertes.fr/tel-00175221/en/" ,
 year = 2007}

@article{Zdeborova08,
 author  = "L. Zdeborov\'a",
 title   = "Statistical Physics of Hard Optimization Problems",
 journal = "Acta Physica Slovaca",
 volume = "59",
 number = "3",
 pages = "169-303",
 year = 2009}

@PhDthesis{RivoireThese,
 author  = "Olivier Rivoire",
 title   = "Phases vitreuses, optimisation et grandes déviations",
 school = "Universit\'e Paris-Sud",
 note = "http://tel.archives-ouvertes.fr/tel-00009956/en/" ,
 year = 2005}

@article{Kac70,
        author  = "M. Kac and T. F. Lin",
        journal = "J. Math. Phys",
        year = 1970,
        volume = 11,
        page= 1584
}

@article{Kadanoff76,
        author  = "L.P. Kadanoff",
        journal = "Ann. Phys.",
        year = 1976,
        volume = 100,
        page= 359
}

@Book{Kadanoff99,
    author =     "L. P. Kadanoff",
    title =   "Statistical physics : statics, Dynamics and
Renormalization",
  publisher =    "World Scientific",
    year =               "1999"}

@incollection{Karp72,
       author = "R. Karp",
       title = "Reducibility among combinatorial problems",
       editor = "R. Miller and J. Thatcher",
       booktitle = "Complexity of Computer Computations",
       pages = "85--103",
       year = 1972,
       publisher = "Plenum Press, New-York"}

@article{Karp79,
        author  = "R. M. Karp",
        title   = "A Patching Algorithm for the Nonsymmetric Travelling Salesman Problem",
        journal = "SIAM J. Comput.",
        year = 1979,
        volume = 8}

@incollection{KarpSteele85,
        author  = "R. M. Karp and J. M. Steele",
        title   = "Probabilistic Analysis of Heuristics",
        booktitle = "The Traveling Salesman Problem",
        publisher = "John Wiley and Sons",
        address = "New York",
        year = 1985,
        editor = "E. L. Lawler and J. K. Lenstra and A. H. G. {Rinnooy Kan} and D. B. Shmoys",
pages = "561--573"}

@article{Katzgraber02,
    author = "H. G. Katzgraber",
    title = "Monte Carlo simulation of vector Spin Glasses at Low Temperatures",
        note = "cond-mat/0204305",
  year = "2002",
 journal = " "}

@Article{KatzgraberKrzakala07,
  title = {Temperature and Disorder Chaos in Three-Dimensional Ising Spin Glasses},
  author = {Katzgraber, Helmut G. and Krza\ifmmode \mbox{\c{}}\else \c{}\fi{}ka\l{}a, Florent },
  journal = {Phys. Rev. Lett.},
  volume = {98},
  number = {1},
  pages = {017201},
  numpages = {4},
  year = {2007},
  month = {Jan},
  doi = {10.1103/PhysRevLett.98.017201},
  publisher = {American Physical Society}
}



@article{KatzgraberPalassini00,
    author = "H. G. Katzgraber and M. Palassini and A. P. Young",
    title = "Spin Glasses at Low Temperatures",
  year = "2001",
  journal = "Phys. Rev. B",
  volume = "63",
  pages = "184422",
    note = "cond-mat/0007113"}

@article{KatzgraberYoung02,
    author = "H.~G. Katzgraber and P. Young",
    title = "Monte Carlo simulations of the four-dimensional XY spin glass at low temperatures",
  year = "2002",
 journal = "Phys. Rev. B",
 pages = 214401,
 volume = 65}


@article{Kauzmann48,
    author = "W. Kauzmann",
    title = "The Nature of the Glassy State and the Behavior of Liquids at Low Temperatures",
  year = "1948",
 journal = "Chem. Rev.",
 pages = 219,
 volume = 43}

@article{Kawashima00,
         author  = "N. Kawashima",
         title = "Fractal Droplets in Two Dimensional Spin Glasses",
         journal = "Jour. Phys. Soc. of J.",
         volume = "69",
         pages = "987",
         year = "2000"}

@article{KawashimaHatano92,
         author  = "N. Kawashima and H. Hatano and M. Suzuki",
         title = "Critical behaviour of the two-dimensional EA model with a Gaussian bond distribution",
         journal = "J. Phys. A",
         volume = 25,
         pages = "4985",
         year = 1992}

@article{KawashimaIto92,
         author  = "N. Kawashima and N. Ito and M. Suzuki",
         title = "Monte {C}arlo Study of the Three-Dimensional {+-J} {I}sing Spin-Glass Model in a Magnetic Field",
         journal = "Jour. Phys. Soc. of J.",
         volume = 61,
         pages = "1777-1786",
         year = 1992}

@article{KawashimaIto93,
         author  = "N. Kawashima and N. Ito",
         title = "Critical Behavior of the {T}hree-{D}imensional
                  {+-J} {M}odel in a {M}agnetic {F}ield",
         journal = "Jour. Phys. Soc. of J.",
         volume = 62,
         pages = "435-438",
         year = 1993}

@article{KawashimaRieger97,
        author  = "N. Kawashima and H. Rieger",
        title = "Finite Size Scaling Analysis of Exact Ground
                 States for {+/-J} Spin Glass Models in Two
Dimensions",
        journal = "Europhys. Lett.",
        volume = 39,
        pages = "85-91",
        year = 1997}

@article{KawashimaSuzuki92,
        author  = "N. Kawashima and M. Suzuki",
        title = "Replica Optimization Method for Ground-State Search
                 of Random Spin Systems",
        journal = "J. Phys. A",
        volume = 25,
        pages = "1055--1070",
        year = 1992}

@article{KawashimaYoung96,
        author  = "N. Kawashima and A. P. Young",
        title = "Phase Transition in the Three-Dimensional {+/-J}
{I}sing
                 Spin Glass",
        journal = "Phys. Rev. B",
        volume = 53,
        pages = "R484",
        year = 1996}

@article{KernighanLin70,
        author  = "B. Kernighan and S. Lin",
        title   = "An Efficient Heuristic Procedure for Partitioning
Graphs",
        journal = "Bell System Technical Journal",
        year = 1970,
        volume = 49,
        pages = "291 - 307"}

@article{Kikuchi51,
      author = "R. Kikuchi",
      title = "A theory of cooperative phenomena",
     journal = "Phys. Rev.",
      volume = 81,
      pages = "988--1003",
      year = 1951}

@article{KinzelBinder83,
    author = "W. Kinzel and K. Binder",
    title = "Static and Dynamic Critical Magnetic Fields in
        {I}sing Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1983,
    volume = 50,
    pages = "1509--1511"}

@article{Kirkpatrick77,
  author = "S. Kirkpatrick",
  title="Frustration and ground-state degeneracy in spin glasses",
  journal="Phys. Rev. B",
  year=1977,
  volume=16,
  pages="4630--4641"}

@inproceedings{SelmanLevesque92,
    author = "Bart Selman and Hector J. Levesque and D. Mitchell",
    title = "A New Method for Solving Hard Satisfiability Problems",
    booktitle = "Proceedings of the Tenth National Conference on Artificial Intelligence",
    publisher = "AAAI Press",
    address = "Menlo Park, California",
    editor = "Paul Rosenbloom and Peter Szolovits",
    pages = "440--446",
    year = "1992",
    }

@article{KirkpatrickGelatt83,
    author = "S. Kirkpatrick and C. D. {Gelatt Jr.} and M. P. Vecchi",
    title = "Optimization by Simulated Annealing",
    journal = "Science",
    year = 1983,
    volume = 220,
    pages = "671--680"}

@article{KirkpatrickSelman94,
    author = "S. Kirkpatrick and B. Selman",
    title = "Critical Behavior in the Satisfiability of Random Boolean
Expression",
    journal = "Science",
    year = 1994,
    volume = 264,
    pages = "1297--1301"}

@article{KirkpatrickThirumalai87a,
    author = "T.R. Kirkpatrick and D. Thirumalai",
    title = "Dynamics of the Structural Glass Transition and the $p$-Spin-Interaction Spin-Glass Model",
    journal = "Phys. Rev. Lett.",
    year = 1987,
    volume = 58,
    pages = "2091"}

@article{KirkpatrickThirumalai87b,
    author = "T.R. Kirkpatrick and D. Thirumalai",
    title = "$p$-spin-interaction spin-glass models: Connections with the
structural glass problem",
    journal = "Phys. Rev. B",
    year = 1987,
    volume = 36,
    pages = "5388"}

@article{KirkpatrickThirumalai89,
    author = "T.R. Kirkpatrick and D. Thirumalai and P.G. Wolynes",
    title = "Scaling concepts for the dynamics of viscous liquids near an ideal glassy state",
    journal = "Phys. Rev. A",
    year = 1989,
    volume = 40,
    pages = "1045"}

@article{KirkpatrickWolynes87,
    author = "T.R. Kirkpatrick and P.G. Wolynes",
    title = "Connections between some kinetic and equilibrium theories of
the glass transition",
    journal = "Phys. Rev. A",
    year = 1987,
    volume = 35,
    pages = "3072"}

@article{KirkpatrickWolynes87b,
    author = "T.R. Kirkpatrick and P.G. Wolynes",
    title = "Stable and metastable states in mean-field {P}otts and structural glasses",
    journal = "Phys. Rev. B",
    year = 1987,
    volume = 36,
    pages = "8852--8564"}

@article{KlotzKobe94,
   author = "T. Klotz and S. Kobe",
   title = "Valley structures in the phase space of a finite 3D {I}sing

            spin glass with +-{I} interactions",
   journal = "J. Phys. A",
   year = "1994",
   volume = "27",
   pages = "L95"}

@article{KobAndersen93,
    author = "W. Kob and H. A. Andersen",
    title = "Kinetic lattice-gas model of cage in high-density liquids and
a test of mode-coupling theory of the ideal-glass transition",
  journal = "Phys. Rev. E",
    year = "1993",
  volume = "48",
  pages = "4364--4377"}

@article{KomoriYoshino00,
      author = "T. Komori and H. Yoshino and H. Takayama",
      title = "Numerical Study on Aging Dynamics in Ising Spin-Glass
Models:
               Temperature-Change Protocols",
      journal = "J. Phys. Soc. Jpn. Suppl A",
      volume = "",
      pages = "228",
      year = "2000"}


@article{ShakhnovichGutin89,
      author = "E. Shakhnovich and A. M Gutin",
      title = "Frozen states of a disordered globular heteropolymer",
      journal = "J. Phys. A: Math. Gen",
      volume = "22",
      pages = "1647-1659",
      year = "1989"}
 

@article{Kondor83,
   author = "I. Kondor",
   title = "Parisi's mean-field solution for spin glasses
            as an analytic continuation in the replica number",
   journal = "J. Phys. A",
   year = "1983",
   volume = "16",
   pages = "L127-L131"}

@article{Kondor89,
    author = "I. Kondor",
    title = "On chaos in spin glasses",
    journal = "J. Phys. A",
    year = "1989",
    volume = "22",
    pages = "L163-L168"}

@article{KondorVegso93,
   author = "I. Kondor and A. V{\'e}gu{\"o}",
   journal = "J. Phys. A",
   year = "1993",
   volume = "26",
   pages = "L641"}

@incollection{Krauth98,
        author  = "W. Krauth",
        title = "Introduction to Monte Carlo Algorithms",
        booktitle = "Advances in Computer Simulation",
        year = 1998,
        publisher = "Springer Verlag",
        editot = "J. Kertesz and I. Kondor",
        note = "Lecture Notes in Physics"}

@article{KrauthMezard89,
  author = "W. Krauth and M. M\'ezard",
  title = "The cavity method and the travelling salesman problem",
  journal = "Europhys. Lett.",
    year = 1989,
    volume = 8,
    pages = "213--218"}

@article{KrauthMezard89b,
  author = "W. Krauth and M. M\'ezard",
  title = "Storage capacity of memory networks with binary couplings",
  journal = "J. Phys. France",
    year = 1989,
    volume = 50,
    pages = "3057--3066"}



@article{KrzakalaHoudayer01,
    author = "F. Krzakala and J. Houdayer and E. Marinari and O.~C. Martin
and G. Parisi",
    title = "Zero-temperature responses of a 3D spin glass in a field",
  journal = "Phys. Rev. Lett.",
    year = "2001",
  volume = "87",
  pages = "197204",
  note = "cond-mat/0107366"
}

@article{KrzakalaHoudayer01,
    author = "F. Krzakala and J. Houdayer and E. Marinari and O.~C. Martin
and G. Parisi",
    title = "Zero-temperature responses of a 3D spin glass in a field",
  journal = "Phys. Rev. Lett.",
    year = "2001",
  volume = "87",
  pages = "197204",
  note = "cond-mat/0107366"
}

@article{KrzakalaKurchan07,
    author = "F. Krzakala and J. Kurchan",
    title = "A Landscape Analysis of Constraint Satisfaction Problems",
  journal = "Phys. Rev. E",
    year = 2007,
  volume = "76",
  pages = "021122",}

@article{KrzakalaMartin01,
    author = "F. Krzakala and O. C. Martin",
    title = "Discrete energy landscapes and replica symmetry breaking
           at zero temperature",
  journal = "Europhys. Lett.",
    year = "2001",
  volume = "6",
  pages = "749--755"}

@article{KrzakalaMartin02,
    author = "F. Krzakala and O. C. Martin",
    title = "Chaotic temperature dependence in a model of spin glasses",
  journal = "Eur. Phys. J. B.",
    year = "2002",
  volume = "28",
  pages = "199-208"}

@article{KrzakalaMartin02b,
    author = "F. Krzakala and O. C. Martin",
    title = "Absence of an equilibrium ferromagnetic spin glass phase in
3d",
  journal = "Phys. Rev. Lett.",
    year = "2002",
  volume = "89",
  pages = "267202",
  note = "cond-mat/0208566"}

@article{KrzakalaMezard02,
    author = "F. Krzakala and M. M{\'e}zard and M. M{\"u}ller",
    title = "Nature of the glassy phase in rna secondary structure",
  journal = "Europhys. Lett.",
    year = "2002",
  volume = "5",
  issue = "57",
  pages = "752--758"}


@article{KrzakalaPagnani04,
      author = "F. Krzakala and A. Pagnani and M. Weigt",
      title = "Threshold values, stability analysis and high-$q$ asymptotics for the coloring problem on random graphs",
      journal = "Phys. Rev. E",
      volume = 70,
      pages = "046705",
      year = 2004}

@article{KrzakalaParisi03,
    author = "F. Krzakala and G. Parisi",
    title = "Local excitations in mean field spin glasses",
  journal = "Europhys. Lett.",
    year = "2004",
  volume = "66",
  pages = "847-853",
  note = "cond-mat/0304590"}

@article{KrzakalaTarzia08,
    author = "Florent Krzakala and Marco Tarzia and Lenka Zdeborov\'a",
    title = "Lattice Model for Colloidal Gels and Glasses",
  journal = "Phys. Rev. Lett.",
    year = "2008",
  volume = "101",
  pages = "165702",
 }

@article{KrzakalaZdeborova07b,
    author = "Florent Krzakala and Lenka Zdeborov\'a",
    title = "Phase Transitions and Computational Difficulty in 
Random Constraint Satisfaction Problems",
  journal = "J. Phys.: Conf. Ser.",
    year = "2008",
  volume = "95",
  pages = "012012",
}

@article{KrzakalaZdeborova07,
    author = "Florent Krzakala and Lenka Zdeborov\'a",
    title = "Potts Glass on Random Graphs",
  journal = "Europhys. Lett.",
    year = "2008",
  volume = "81",
  pages = "57005",
 }


@article{KrzakalaZdeborova09,
    author = "Florent Krzakala and Lenka Zdeborov\'a",
    title = "Hiding Quiet Solutions in Random Constraint Satisfaction Problems",
  journal = "Phys. Rev. Lett.",
    year = "2009",
  volume = "102",
  pages = "238701",
 }


@article{KschischangFrey01,
  author ="F. R. Kschischang and B. Frey and H.-A. Loeliger",
  title = "Factor graphs and the sum-product algorithm",
  journal = "IEEE Trans. Inform. Theory",
  year = "2001",
  volume = "47",
  number = "2",
  pages = "498--519"}


@article{Kurchan01,
    author = "J.~Kurchan",
    title = "Recent theories of glasses as out of
           equilibrium systems",
  journal = "Special issue `Physics of Glasses' of the
       Comptes Rendus de Physique de l'Academie des Science",
    year = "2001",
   note="cond-mat/0011110"}

@article{KurchanParisi93,
    author = "J.~Kurchan and G.~Parisi and M.~A. Virasoro",
    title = "Barriers and metastable states as saddle points in the
replica
  approach",
  journal = "J. Phys I France",
    year = "1993",
  volume = "3",
  page = "1819"
}

@article{KwonThouless88,
    author = "C. Kwon and D.~J. Thouless",
    title = "Ising spin glass at zero temperature on the Bethe lattice",
  journal = "Phys. Rev. B",
    year = "1988",
  volume = "37",
  page = "7649-7654"}

@article{LamarcqBouchaud02,
  author ="J. Lamarcq and J.-P. Bouchaud and O. C. Martin and M.
M\'ezard",
  title  ="Non-compact local excitations in spin-glasses",
  journal = "Europhys. Lett.",
  year   = 2002,
  volume = "58",
  pages = "321"}

@article{LamarcqBouchaud02b,
  author ="J. Lamarcq and J.-P. Bouchaud and O. C. Martin",
  title  ="Local excitations of a spin glass in a magnetic field",
  journal = " ",
  year   = " ",
  volume = " ",
  pages = "",
  note= "To appear in Phys. Rev. B. ; xcond-mat/0208100" }

@article{LandryCoppersmith02,
  author ="J.W. Landry and S.N. Coppersmith",
  title  ="Ground states of two-dimensional $\pm{J}$ {E}dwards-Anderson

                  spin glasses",
  journal = "Phys. Rev. B",
  year   = "2002",
  volume = "65",
  pages = "134404",
  note= "cond-mat/0109136" }

@article{LawlorReagan02,
  author ="A. Lawlor and D. Reagan and G. D. McCullagh and P. De
Gregorio and P. Tartaglia and K. A. Dawson",
  title  ="Universality in lattice models of dynamic arrest:
Introduction of an order parameter",
  journal = "Phys. Rev. Lett.",
  year   = 2002,
  volume = 89,
  pages = "245503"}

@article{Lefloch92,
  author ="F. Lefloch and J. Hammann and Ocio and E. Vincent",
  title  ="",
  journal = "Europhys. Lett.",
  year   = 1992,
  volume = 18,
  pages = "647"}
}

@article{LehenyNagel98,
  author ="R. L. Leheny and S.R. Nagel",
  title  ="Frequency-domain study of physical aging in a simple
liquid",
  journal = "Phys. Rev. E.",
  year   = 1998,
  volume = 57,
  pages = "5154"}

@article{LehenyNagel98,
  author ="R. L. Leheny and S.R. Nagel",
  title  ="Frequency-domain study of physical aging in a simple liquid",
  journal = "Phys. Rev. E.",
  year   = 1998,
  volume = 57,
  pages = "5154"}

@article{LeoneRicci01,
  author ="M. Leone and F. Ricci-Tersenghi and R. Zecchina",
  title  ="Phase coexistence and finite-size scaling in random combinatorial problems",
  journal = "J. Phys. A ",
  year   = 2001,
  volume = 34,
  pages = "4615"}

@article{LiersPalassini03,
  author ="F. Liers and M. Palassini and A. K. Hartmann and M. Juenger",
  title  ="Ground state of the {B}ethe-lattice spin glass and running
           time of an exact optimization algorithm",
  journal = "",
  year   = "",
  volume = "",
  pages = "",
  note = "cond-mat/212630"}

@article{Lin65,
         Author = "S. Lin",
         Title = "Computer Solutions of the Traveling Salesman
Problem",
         journal = "Bell System Technical Journal",
         volume = 44,
         year = 1965,
         pages = "2245--2269"}

@article{LinKernighan73,
        author  = "S. Lin and B. Kernighan",
        title   = "An Effective Heuristic Algorithm for the
                   Traveling Salesman Problem",
        journal = "Operations Research",
        year = 1973,
        volume = 21,
        pages = "498--516"}

@inproceedings{Palmer83,
         Author = "R.G. Palmer",
         Title = "",
         booktitle = "Proc. of the Heidelberg Colloquium on spin glasses, Lecture Notes in Physics 192",
         Editors = "J.L. van Hemmen and I. Morgenstern",
         year = "1983",
         publisher = "Springer", 
         address = "Berlin"        
}

@article{LingBowman83,
         Author = "David D.~Ling and David R.~Bowman and K.~Levin ",
         Title = "Free-energy surface of spin-glasses: Thouless-Anderson-Palmer and Bethe-Peierls-Weiss models",
         journal = "Phys, Rev. B",
         volume = 28,
         year = 1983,
         pages = "262--269"}

@ARTICLE{MetropolisRosenbluth53,
   author = {{Metropolis}, N. and {Rosenbluth}, A.~W. and {Rosenbluth}, M.~N. and 
	{Teller}, A.~H. and {Teller}, E.},
    title = "{Equation of State Calculations by Fast Computing Machines}",
  journal = {The Journal of Chemical Physics},
     year = 1953,
    month = jun,
   volume = 21,
    pages = {1087-1092},
   adsurl = {http://adsabs.harvard.edu/abs/1953JChPh..21.1087M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{LinussonWastlund03,
  author = "S. Linusson and J. Wastlund",
  journal = "Probability Theory and Related Fields",
  title = "A proof of {P}arisi's conjecture on the random assignment
problem",
  year = 2004,
  pages = "419-440",
  volume = "128",
}


@Article{LopantinIoffe02,
  title = {Structural glass on a lattice in the limit of infinite dimensions},
  author = {Lopatin, A. V. and Ioffe, L. B.},
  journal = {Phys. Rev. B},
  volume = {66},
  number = {17},
  pages = {174202},
  numpages = {5},
  year = {2002},
  month = {Nov},
  doi = {10.1103/PhysRevB.66.174202},
  publisher = {American Physical Society}
}



@InCollection{LouMarStu02:mh,
 author = "H. R. Louren\c{c}o and O. Martin and T. St{\"u}tzle",
 title = "Iterated Local Search",
 year = "2002",
 pages = "321--353",
 series = "International Series in Operations Research \& Management
Science",
 volume = 57,
 booktitle = "Handbook of Metaheuristics",
 editor = "F.~Glover and G.~Kochenberger",
 publisher ="Kluwer Academic Publishers, Norwell, MA"}

@article{LuzzatiGulik68,
    author = "V. Luzzati and T. Gulik-Krzywicki and A. Tardieu",
    journal = "Nature",
    year = 1968,
    volume = 218,
    pages = 1031}

@book{Ma76,
    author = "S. K. Ma",
    title = "Modern Theory of Critical Phenomena",
    publisher = "Benjamin Cummings Publishing Company",
    year = 1976,
    address = "Reading MA"}

@book{MacKay03,
    author = "D. J. C. MacKay",
    title = "Information theory, inference, and learning algorithms",
    publisher = "Cambridge University Press",
    year = 2003,
    address = "Cambridge"}

@article{MajumdarKrapivsky00,
      author = "S. N. Majumdar and P. L. Krapivsky",
      title = "Extremal paths on a random {C}ayley tree",
      journal = "Phys. Rev. E",
      volume =  62,
      pages = "7735--7742",
      year = 2000}

@article{MariCampbell99,
    author = "P.O. Mari and I.A. Campbell",
    title = "Ising spin glasses: corrections to finite size scaling,
           freezing temperatures, and critical exponents",
    journal = "Phys. Rev. E,",
    volume = 59,
    pages = "2653",
    year = 1999}

@article{MariKrzakala09,
    author = "R. Mari and F. Krzakala and J. Kurchan",
    title = "Jamming versus Glass Transitions",
    journal = "Phys. Rev. Lett.",
    volume = 103,
    pages = "025701",
    year = "2009"}

@inproceedings{Marinari98,
    author = "E. Marinari",
    title = "Optimized {M}onte {C}arlo methods",
    booktitle = "Advances in {C}omputer {S}imulation",
    editor = "J. Kert\'esz and I. Kondor",
    year = 1988,
    pages = "50",
    address = "{B}erlin",
    publisher = "{S}pringer-{V}erlag"}


@article{Marinari99,
    author = "E. Marinari",
    title = "Numerical Evidence for Continuity of Mean-Field and
        Finite-Dimensional Spin Glasses",
    journal = "Phys. Rev. Lett.",
    volume = 82,
    year = 1999,
    pages = "434--437"}


@article{MarinariMartin01,
    author = "E. Marinari and O. C. Martin and F. Zuliani",
    title = "Equilibrium valleys in spin glasses at low temperature",
    journal = "Phys. Rev. B.",
  volume = 64,
  pages = 184413,
  year = 2001,
    note = "cond-mat/0103534 "}

@article{MarinariNaitza98,
    author = "E. Marinari and C. Naitza and F. Zuliani",
    title = "Critical Behavior of the 4{D} Spin Glass in magnetic Field",
    journal = "J. Phys. A",
    volume = 31,
    year = 1998,
    pages = "6355--6366"}

@article{MarinariNaitza98b,
    author = "E. Marinari and C. Naitza and F. Zuliani and G. Parisi and
        M. Picco and F. Ritort",
    title = "General Method to Determine Replica Symmetry Breaking
        Transitions",
    journal = "Phys. Rev. Lett.",
    volume = 81,
    year = 1998,
    pages = "1698--1701"}

@article{MarinariPagnani02,
    author = "E. Marinari and A. Pagnani and F. Ricci-Tersenghi",
    title = "Zero-temperature properties of RNA secondary structures",
    journal = "Phys. Rev. E",
    year = 2002,
    volume = 65,
    pages = "041919"}



@article{MarinariParisi00a,
    author = "E. Marinari and G. Parisi",
    title = "Comment on ``Triviality of the Ground State Structure
                        in {I}sing Spin Glasses''",
    year = 2000,
  journal = "Phys. Rev. Lett.",
  volume = "85",
  pages = "3332",
    note = "cond-mat/0002457"}

@article{MarinariParisi00b,
    author = "E. Marinari and G. Parisi",
    title = "Effects of Changing the Boundary Conditions
           on the Ground State of {I}sing Spin Glasses",
  journal = "Phys. Rev. B",
    year = 2000,
  volume = "62",
  pages = "11677",
    note = "cond-mat/0005047"}

@article{MarinariParisi00c,
    author = "E. Marinari and G. Parisi",
    title = "On the Effects of a Bulk Perturbation on the Ground
           State of 3D {I}sing Spin Glasses",
 year = 2001,
    journal = "Phys. Rev. Lett.",
    volume = 86,
    pages = "3887--3890"}

@article{MarinariParisi92,
    author = "E. Marinari and G. Parisi",
    title = "Simulated Tempering: a New Monte Carlo Scheme",
    journal = "Europhys. Lett.",
    year = 1992,
    volume = 6,
    pages = "451--458"}

@article{MarinariParisi96,
    author = "E. Marinari and G. Parisi and J. {Ruiz-Lorenzo} and F.
Ritort",
    title = "Numerical Evidence for Spontaneously Broken Replica
        Symmetry in 3{D} Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1996,
    volume = 76,
    pages = "843--846"}

@article{MarinariParisi98,
    author = "E. Marinari and G. Parisi and J. {Ruiz-Lorenzo}",
    title = "Phase Structure of the Three-Dimensional
        {E}dwards-{A}nderson Spin Glass",
    journal = "Phys. Rev. B",
    volume = 58,
    year = 1998,
    pages = "14852--14863"}

@article{MarinariParisi98b,
    author = "E. Marinari and G. Parisi and F. Ricci-Tersenghi and J.
        {Ruiz-Lorenzo}",
    title = "Small Window Overlaps are Effective Probes of Replica
    Symmetry Breaking in Three-Dimensional Spin Glasses",
    journal = "J. Phys. A",
    volume = 31,
    year = 1998,
    pages = "L481--L487"}

@incollection{MarinariParisi98c,
      author = "E. Marinari and G. Parisi and J.J. {Ruiz-Lorenzo}",
      title = "Numerical Simulations of Spin Glass Systems",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@article{MarinariParisi98d,
    author = "E. Marinari and G. Parisi and F. Zuliani",
    title = "Four-dimensional Spin Glasses in a Magnetic
                 Field have a Mean-Field-Like Phase",
    journal = "J. Phys. A",
    volume = 31,
    year = 1998,
    pages = "1181--1187"}

@article{MarinariParisi99,
    author = "E. Marinari and G. Parisi and F. Zuliani",
    title = "Comment on ``{I}sing Spin Glasses in a Magnetic Field''",
  journal = "Phys. Rev. Lett.",
  volume = "84",
  pages = "1056",
    year = 1999,
    note = "cond-mat/9812401"}

@article{MarinariParisi99b,
    author = "E. Marinari and G. Parisi and F. Ricci-Tersenghi
                  and J.J. {Ruiz-Lorenzo} and F. Zuliani",
    title = "Replica Symmetry Breaking in Short Range Spin Glasses:
                 A review of the Theoretical Foundations and of the
                 Numerical Evidence",
  journal = "J. Stat. Phys.",
    year = 2000,
  volume = "98",
  pages =  "973",
    note = "cond-mat/9906076"}

@article{MartinMezard04,
      author = "O. C. Martin and M. M{\'e}zard and O. Rivoire",
      title = " Frozen glass phase in the multi-index matching problem",
      journal = "Phys. Rev. Lett.",
      volume = 93,
      pages = "217205",
      year = 2004}

@article{MartinMezard05,
      author = "O. C. Martin and M. M{\'e}zard and O. Rivoire",
      title = "Random multi-index matching problems",
      year = "2005",
      journal = "J. Stat. Mech.",
      page = "P09006"
}

@article{MartinMonasson01,
    author = "O. C. Martin and R. Monasson and R. Zecchina ",
    title = "Statistical mechanics methods and phase transitions in
optimization problems",
  journal="Theoretical Computer Science",
    year = 2001,
    volume = 256,
    pages = "3-67"}

@article{MartinOtto96,
    author = "O. C. Martin and S. W. Otto",
    title = "Combining Simulated Annealing with Local Search Heuristics",
    journal = "Ann. Oper. Res.",
    year = 1996,
    volume = 63,
    pages = "57--75"}


@article{MartinSiggia73,
    author = "P.~C. Martin and E.~D Siggia and H.~A. Rose",
    title = "Statistical dynamics of classical systems",
    journal = "Phys. Rev. A",
    year = 1973,
    volume = 8,
    pages = "423"}
    note = "cond-mat/"}

@article{MasuiJacobs93,
  author = "S. Masui and A. E. Jacobs and C. Wicentowich and B. W.
Southern",
  title = "Metastable States of the Random-Field Ising Chain",
  journal = "J. Phys. A: Math. Gen.",
  year = 1993,
  volume = 26,
  pages = "25--37"}

@article{MattssonJonsson95,
    author = "J. Mattsson and T. Jonsson and P. Nordblad and H. A.
    Katori and A. Ito",
    title = "No Phase Transition in a Magnetic Field in the Ising Spin
    Glass {Fe$_0.5$Mn$_0.5$TiO$_3$}",
    journal = "Phys. Rev. Lett.",
    year = 1995,
    volume = 74,
    pages = "4305--4308"}

@article{McKayWormald84,
      author = "B. D. Mc{K}ay and N. C. Wormald",
      title = "Automorphisms of random graphs with specified degrees",
      journal = "Combinatorica",
      volume = 4,
      pages = "325--338",
      year = 1984}

@article{McMillan83,
    author = "W. L. McMillan",
  title = "Monte Carlo simulation of the two-dimensional
           random $\pm {J}$ Ising model",
    journal = "Phys. Rev. B",
    year = 1983,
    volume = 28,
    pages = "5216--5219"}

@article{McMillan84,
    author = "W. L. McMillan",
   title="Domain-wall renormalization-group study of the
          two-dimensional random {I}sing Model",
    journal = "Phys. Rev. B",
    year = 1984,
    volume = 29,
    pages = "4026--4029"}

@article{McMillan84b,
    author = "W. L. McMillan",
   title="Domain-wall renormalization-group study of the
          three-dimensional random {I}sing Model",
    journal = "Phys. Rev. B",
    year = 1984,
    volume = 30,
    pages = "476--477"}

@article{McMillan85,
    author = "W. L. McMillan",
    title = "Domain-Wall Renormalization Group Study of the
        Three dimensional Random {I}sing Model at Finite Temperature",
    journal = "Phys. Rev. B",
    year = 1985,
    volume = 31,
    pages = "340--341"}

@article{Mertens01,
   title = "A physicist's approach to number partitioning",
   author = "Stephan Mertens",
   volume = "265",
   journal = "Theoretical Computer Science",
   number = "1-2",
   year = "2001",
   pages = "79-108"
}


@Article{Mertens98,
  title = {Phase Transition in the Number Partitioning Problem},
  author = {Mertens, Stephan },
  journal = {Phys. Rev. Lett.},
  volume = {81},
  number = {20},
  pages = {4281--4284},
  numpages = {3},
  year = {1998},
  month = {Nov},
  doi = {10.1103/PhysRevLett.81.4281},
  publisher = {American Physical Society}
}

@Article{Mertens00,
  title = {Random Costs in Combinatorial Optimization},
  author = {Mertens, Stephan },
  journal = {Phys. Rev. Lett.},
  volume = {84},
  number = {6},
  pages = {1347--1350},
  numpages = {3},
  year = {2000},
  month = {Feb},
  doi = {10.1103/PhysRevLett.84.1347},
  publisher = {American Physical Society}
}

@article{Mertens02,
author = {Stephan Mertens},
title = {Computational Complexity for Physicists},
journal = {Computing in Science and Engineering},
volume = {04},
number = {3},
year = {2002},
issn = {1521-9615},
pages = {31-47},
doi = {http://doi.ieeecomputersociety.org/10.1109/5992.998639},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}


@article{MertensMezard06,
 author = {Stephan Mertens and Marc M\'ezard and Riccardo Zecchina},
 title = {Threshold values of random K-SAT from the cavity method},
 journal = {Random Struct. Algorithms},
 volume = {28},
 number = {3},
 year = {2006},
 issn = {1042-9832},
 pages = {340--373},
 doi = {http://dx.doi.org/10.1002/rsa.v28:3},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
 }

@InProceedings{Mezard00,
    author =             {M. M{\'e}zard},
    title =              {First Steps in Glass Theory},
    booktitle =      {Proceedings of the 2000 Aspen workshop "50 years of
Condensed Matter Physics"},
  year = 2000,
  note = "cond-mat/0005173"}

@incollection{Mezard02,
      author = "M. M{\'e}zard",
      title = "First steps in glass theory",
      editor = "Ong and Bhatt",
      booktitle = "More is different",
      publisher = "Princeton University Press",
      year = 2002}


@article{Mezard04,
  author = "M. M\'ezard",
  title = "Message passing in random satisfiability problems",
  year = 2004,
  note= "Talk given at NIPS 2003, arXiv:cond-mat/0401237"}

@Article{Mezard90,
        author = "M. M{\'e}zard",
        title =  "On the glassy nature of random directed polymers in two dimensions",
        journal = "J. Physique",
        year = 1990,
        volume = 51,
        pages = 1831}

@article{MezardPalassini05,
      author = "M. M{\'e}zard and M. Palassini and O. Rivoire",
      title = "Landscape of solutions in constraint satisfaction problems",
 journal = "Phys. Rev. Lett.",
        year = 2005,
        volume = 95,
        pages = 200202}

@article{MezardParisi00,
      author = "M. M{\'e}zard and G. Parisi",
      title = "Statistical physics of structural glasses",
      journal = "J. Phys.: Condens. Matter",
      volume = 12,
      pages = "6655--6673",
      year = 2000}

@article{MezardParisi01,
   author = "M. M{\'e}zard and G. Parisi",
   title = "The Bethe lattice spin glass revisited",
   journal = "Eur. Phys. J. B",
   year = 2001,
   volume = "20",
   pages = "217"}

@article{MezardParisi02,
   author = "M. M{\'e}zard and G. Parisi and R. Zecchina",
   title = "Analytic and Algorithmic Solution of Random Satisfiability
Problems",
   journal = "Science",
   year = 2002 ,
   volume = "297",
   pages = "812-815"}

@article{MezardParisi03,
   author = "M. M{\'e}zard and G. Parisi",
   title = "The cavity method at zero temperature",
   journal = "J. Stat. Phys. ",
   year = 2003,
   volume = "111",
   pages = "1--34"}

@article{MezardParisi84,
    author = "M. M{\'e}zard and G. Parisi and N. Sourlas and
            G. Toulouse and M. A. Virasoro",
    title = "Replica Symmetry Breaking and the Nature of the Spin-Glass
        Phase",
    journal = "J. Physique",
    year = 1984,
    volume = 45,
    pages = "843--854"}

@article{MezardParisi85,
    author = "M. M{\'e}zard and G. Parisi",
    title = "Replicas and Optimization",
    journal = "J. Physique",
    year = 1985,
    volume = 46,
    pages = "L771--L778"}

@article{MezardParisi85b,
    author = "M. M{\'e}zard and G. Parisi and M. A. Virasoro",
    title = "Random Free Energies in Spin-Glasses",
    journal = "J. Physique Lett.",
    year = 1985,
    volume = 46,
    pages = "L217--L222"}

@article{MezardParisi85c,
    author = "M. M{\'e}zard and G. Parisi and M. A. Virasoro",
    title = "{SK} Model: The Replica Solution without Replicas",
    journal = "Europhys. Lett.",
    year = 1986,
    volume = 1,
    pages = "77--82"}

@article{MezardParisi86,
    author = "M. M{\'e}zard and G. Parisi",
    title = "Mean-Field Equations for the Matching and the Travelling
        Salesman Problem",
    journal = "Europhys. Lett.",
    year = 1986,
    volume = 2,
    pages = "913--918"}

@article{MezardParisi86b,
    author = "M. M{\'e}zard and G. Parisi",
    title = "A Replica Analysis of the Travelling Salesman Problem",
    journal = "J. Physique",
    year = 1986,
    volume = 47,
    pages = "1285--1296"}

@ARTICLE{MezardParisi86c,
   author = {{M{\'e}zard}, M. and {Parisi}, G. and {Virasoro}, M.~A.},
    title = "{SK model: the replica solution without replicas}",
  journal = {Europhysics Letters},
     year = 1986,
    month = jan,
   volume = 1,
    pages = {77},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986EL......1...77M&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{MezardParisi87,
    author = "M. M{\'e}zard and G. Parisi",
    title = "On the Solution of the Random Link Matching Problems",
    journal = "J. Physique",
    year = 1987,
    volume = 48,
    pages = "1451--1459"}

@book{MezardParisi87b,
    author = "M. M{\'e}zard and G. Parisi and M. A. Virasoro",
    title = "Spin-Glass Theory and Beyond",
    publisher = "World Scientific",
    year = 1987,
    volume = 9,
    series = "Lecture Notes in Physics",
    address = "Singapore"}

@article{MezardParisi87c,
    author = "M. M{\'e}zard and G. Parisi",
    title = "Mean-field theory of randomly frustrated systems with finite
connectivity",
    journal = "Europhys. Lett.",
    year = 1987,
    volume = 3,
    pages = "1067--1074"}

@article{MezardParisi88,
    author = "M. M{\'e}zard and G. Parisi",
    title = "The {E}uclidean Matching Problem",
    journal = "J. Physique France",
    year = 1988,
    volume = 49,
    pages = "2019--2025"}

@article{ParisiZamponi09,
    author = "G. Parisi and F. Zamponi",
    title = "Mean field theory of hard sphere glasses and jamming",
    journal = "Rev. Mod. Phys.",
    year = 2009,
    note = "to appear, arXiv:0802.2180"}

@article{MezardParisi90,
    author = "M. M{\'e}zard and G. Parisi",
    title = "Replica field theory for random manifolds",
    journal = "J. Phys.",
    year = 1991,
    volume = "I1",
    pages = "809"}

@article{MezardParisi99,
  author = "M. M{\'e}zard and G. Parisi",
    title = "Thermodynamics of glasses: a first principle computation",
  journal = "Phys. Rev. Lett.",
  year = 1999,
  volume = 82,
  pages = "747--750"}

@article{MezardRicci03,
   author = "M. M{\'e}zard and  F. Ricci-Tersenghi and R. Zecchina",
   title = "Alternative solutions to diluted $p$-spin models and {XORSAT}
problems",
   journal="J. Stat. Phys.",
   volume="111",
   pages="505",
   year = 2003}

@inproceedings{MezardSourlas86,
    author = "M. M{\'e}zard and N. Sourlas and G. Toulouse",
    title = "Some Remarks on Ultrametricity",
    booktitle = "Heidelberg Colloquium on Glassy Dynamics",
    editor = "J. L. van Hemmen and I. Morgenstern",
    year = 1986,
    volume = 275,
    series = "Lecture Notes in Physics",
    pages = "238--248",
    address = "{B}erlin",
    publisher = "{S}pringer"}

@article{MezardVirasoro85,
    author = "M. M{\'e}zard and M. A. Virasoro",
    title = "The Microstructure of Ultrametricity",
    journal = "J. Physique",
    year = 1985,
    volume = 46,
    pages = "1293--1307"}

@article{MezardZecchina02,
   author = "M. M{\'e}zard and R. Zecchina",
   title = "Random $K$-satisfiability problem: {F}rom an analytic
solution to an efficient algorithm",
   journal = "Phys. Rev. E",
   year = 2002,
   volume = "66",
   pages = "056126"}

@article{Middleton01,
        author = "A.A. Middleton",
        title = "Energetics and geometry of excitations in random
systems",
        journal = "Phys. Rev. B.",
        year = 2001,
        volume = 63,
        pages = "060202(R)"}

@article{Middleton99,
        author = "A.A. Middleton",
        title = "Numerical investigation of the thermodynamic
                 limit for ground states in models with quenched
disorder",
        journal = "Phys. Rev. Lett.",
        year = 1999,
        volume = 83,
        pages = "1672--1675"}

@article{Migdal75,
        author = "A.A. Migdal",
        journal = "Sov. Phys. JETP",
        year = 1975,
        volume = 42,
        pages = "423"}

@article{MiglioriniBerker98,
        author = "G. Migliorini and A. N. Berker",
        title = "Global random-field spin-glass phase diagrams in two
and three dimensions",
        journal = "Phys. Rev. B.",
        year = 1998,
        volume = 57,
        pages = "426"}

@article{MiyashitaVincent01,
        author = "S. Miyashita and E. Vincent",
        title = "Microscopic mechanism for rejuvenation and memory
effects in spin glasses",
        note = "cond-mat/0102077"}

@article{MobiusNeklioudov97,
    author = "A. M{\"o}bius and A. Neklioudov and A.
    D{\'\i}az-S{\'a}nchez and K. H. Hoffmann and A. Fachat and M.
Schreiber",
    title = "Optimization by Thermal Cycling",
    journal = "Phys. Rev. Lett.",
    year = 1997,
    volume = 79,
    pages = "4297--4301"}

@article{Monasson95,
    author = "R. Monasson",
    title = "Structural glass transition and the Entropy of the Metastable
States",
  journal = "Phys. Rev. Lett.",
   year = 1995,
   volume = "75",
   pages = "2847"}

@article{Monasson98,
    author = "R. Monasson",
    title = "Optimization problems and replica symmetry breaking in finite
connectivity spin-glasses",
  journal = "J. Phys. A",
   year = 1998,
   volume = "31",
   pages = "515"}

@article{MonassonZecchina96,
    author = "R. Monasson and R. Zecchina",
    title = "Entropy of the {K}-Satisfiability Problem",
    journal = "Phys. Rev. Lett.",
    year = 1996,
    volume = 76,
    pages = "3881--3885"}

@Article{MonassonZecchina97,
  title = {Statistical mechanics of the random $K$-satisfiability model},
  author = {Monasson, R\'emi  and Zecchina, Riccardo },
  journal = {Phys. Rev. E},
  volume = {56},
  number = {2},
  pages = {1357--1370},
  numpages = {13},
  year = {1997},
  month = {Aug},
  doi = {10.1103/PhysRevE.56.1357},
  publisher = {American Physical Society}
}

@article{MonassonZecchina98,
    author = "R. Monasson and R. Zecchina",
    title = "Tricritical Points in Random Combinatorics: the
        $(2+p)$-{SAT} case",
    journal = "J. Phys. A",
    year = 1998,
    volume = 31,
    pages = "9209--9217"}

@article{MonassonZecchina99,
      author = "R. Monasson and R. Zecchina and S. Kirkpatrick and B. Selman and L. Troyansky",
      title = "Determining computational complexity from characteristic phase transitions",
      journal = "Nature",
      volume = 400,
      pages = "133--137",
      year = 1999}

@article{MonassonZecchina99b,
      author = "R. Monasson and R. Zecchina and S. Kirkpatrick and B. Selman and L. Troyansky",
      title = "2+p-SAT: Relation of typical-case complexity to the nature of the phase transition",
      journal = "Random Structures and Algorithms",
      volume = 15,
      pages = "414",
      year = 1999}

@article{AchlioptasKirousis01,
      author = "Dimitris Achlioptas and Lefteris M. Kirousis and Evangelos Kranakis and Danny Krizanc",
      title = "Rigorous results for random (2+p)-SAT",
      journal = "Theoretical Computer Science",
      volume = 256,
      number = "1-2",
      pages = "109-129",
      year = 2001}


@article{Montanari01,
  author = "A. Montanari",
  title = "The glassy phase of {G}allager codes",
  journal = "Eur. Phys. J. B.",
    year = 2001,
    volume = 23,
    pages = "121--136"
}

@unpublished{DemboMontanari08,
  author = "A. Dembo and A. Montanari",
  title = "Ising models on locally tree-like graphs",
  year = "2008",
  note = "arXiv:0804.4726v2 [math.PR]"
}

@unpublished{IoffeMezard09,
  author = "L. Ioffe and M. M\'ezard",
  title = "Energy transport in strongly disordered superconductors and magnets",
  year = "2009",
  note = "arXiv:0909.2263"
}

@article{KestenStigum66,
  author = "H. Kesten and B. P. Stigum",
  title = "Additional Limit Theorems for Indecomposable Multidimensional Galton-Watson Processes",
  journal = "The Annals of Mathematical Statistics",
    year = 1966,
    volume = 37,
    pages = "1463"
}

@article{KestenStigum66b,
  author = "H. Kesten and B. P. Stigum",
  title = "Limit Theorems for Decomposable Multi-Dimensional Galton-Watson Processes",
  journal = "J. Math. Anal. Appl.",
    year = 1966,
    volume = 17,
    pages = "309"
}



@inproceedings{MontanariShah06,
  author = "A. Montanari and D. Shah",
  title = "Counting good truth assignments of random k-SAT formulae",
  booktitle = "Proc. of the 18th ACM-SIAM Symposium on Discrete Algorithms",
   year = {2007},
   pages = "1255-1264",
   publisher = {ACM Press},
   address = {New York, USA},
}

@inproceedings{BandyopadhyayGamarnik06,
  author = "Antar Bandyopadhyay and David Gamarnik",
  title = "Counting without sampling: new algorithms for enumeration problems using statistical physics",
  booktitle = "Proc. of the 17th ACM-SIAM Symposium on Discrete Algorithms",
   year = {2006},
   pages = "890 - 899",
   publisher = {ACM Press},
   address = {New York, USA},
}

@inproceedings{Connamacher04,
  author = "H. Connamacher",
  title = "A Random Constraint Satisfaction Problem That Seems Hard for DPLL",
  year = {2004},
  booktitle     = {SAT 2004 - The Seventh International Conference on Theory
               and Applications of Satisfiability Testing, 10-13 May 2004,
               Vancouver, BC, Canada, Online Proceedings},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{ConnamacherMolloy04,
  author = "H. Connamacher and M. Molloy",
  title = "The Exact Satisfiability Threshold for a Potentially Intractable Random Constraint Satisfaction Problem",
  booktitle     = {45th Symposium on Foundations of Computer Science (FOCS
               2004), 17-19 October 2004, Rome, Italy, Proceedings},
  publisher = {IEEE Computer Society},
  year      = {2004},
  isbn      = {0-7695-2228-9},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@incollection{ManevaMeltzer06,
  author ="E. Maneva and T. Meltzer and J. Raymond and A. Sportiello and L. Zdeborov\'a",
  title ="A Hike in the Phases of the 1-in-3 Satisfiability",
  booktitle = "Les Houches Summer School, Session LXXXV 2006 on Complex Systems",
  year = 2006,
  
}

@inproceedings{GerschenfeldMontanari07,
  author = "A. Gerschenfeld and A. Montanari",
  title = "Reconstruction for models on random graphs",
  year = {2007},
  pages = "194--204",
  booktitle     = {Proc. of 48th FOCS},
  publisher = {IEEE Computer Society},
}

@Article{MontanariRicci04,
  title = {Cooling-schedule dependence of the dynamics of mean-field glasses},
  author = {Andrea Montanari and Federico Ricci-Tersenghi},
  journal = {Phys. Rev. B},
  volume = {70},
  number = {13},
  pages = {134406},
  year = {2004},
  publisher = {American Physical Society}
}


@article{BarthelHartmann02,
  title = {Hiding Solutions in Random Satisfiability Problems: A Statistical Mechanics Approach},
  author= {W. Barthel and A. K. Hartmann and M. Leone and F. Ricci-Tersenghi and M. Weigt and R. Zecchina},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  pages = {188701}, 
  year = {2002} 
}

@inproceedings{KrocSabharwal07,
  author = "Lukas Kroc and Ashish Sabharwal and Bart Selman ",
  title = "Survey Propagation Revisited ",
  booktitle = "Proc. of 23rd AUAI",
   year = {2007},
   pages = "217--226",
   publisher = {AUAI Press},
   address = {Arlington, Virginia, USA},
}

@unpublished{KrocSabharwal08,
  author = "Lukas Kroc and Ashish Sabharwal and Bart Selman ",
  title = "Decimation Strategies: Surveys, Beliefs, and Local Information",
  year = {2007},
  note = "in preparation"
}


@article{MontanariMezard00,
    author = "A. Montanari and M. M\'ezard",
    title = "Pulling Hairpinned Polymers",
  year = 2000,
  note = "cond-mat/0006166"}

@Article{MuellerLeuzzi06,
  title = {Marginal states in mean-field glasses},
  author = {M\"uller, Markus  and Leuzzi, Luca  and Crisanti, Andrea },
  journal = {Phys. Rev. B},
  volume = {74},
  number = {13},
  pages = {134431},
  numpages = {26},
  year = {2006},
  month = {Oct},
  doi = {10.1103/PhysRevB.74.134431},
  publisher = {American Physical Society}
}


@article{MontanariMueller04,
      author = "A. Montanari and M. M{\"u}ller and M. M{\'e}zard",
      title = "The Phase Diagram of Random Heteropolymers",
      journal = "Phys. Rev. Lett.",
      volume = 92,
      pages = "185509",
      year = 2004}

@article{MontanariMuller03,
   author = "A. Montanari and M. M{\"u}ller and M. M{\'e}zard",
   title = "The phase diagram of random heteropolymers",
   journal = "",
   year = 2003,
   volume = "",
   pages = "",
   note="cond-mat/0307040"}

@article{MontanariParisi04,
      author = "A. Montanari and G. Parisi and F. Ricci-Tersenghi",
      title = "Instability of one-step replica-symmetry-broken phase in satisfiability problems",
      journal = "J. Phys. A",
      volume = 37,
      pages = "2073",
      year = 2004}

@article{RicciSemerjian09,
      author = "F. Ricci-Tersenghi and G. Semerjian",
      title = "On the cavity method for decimated random constraint satisfaction problems and the analysis of belief propagation guided decimation algorithms",
      journal = "J. Stat. Mech.",
      pages = "P09001",
      year = 2009}


@article{MontanariRicci03,
    author = "A. Montanari and F. Ricci-Tersenghi",
    title = "On the nature of the low-temperature phase
        in discontinuous mean-field spin glasses",
journal = "Eur. Phys. J. B",
   year = 2003,
   volume = "33",
   pages = "339"}


@unpublished{MontanariRicci07,
    author = "A. Montanari and F. Ricci-Tersenghi and G. Semerjian",
    title = "Solving Constraint Satisfaction Problems through Belief Propagation-guided decimation",
    year = 2007,
    note = "in Proceedings of Allerton 2007. Preprint: arXiv:0709.1667v1 [cs.AI]"}

@article{Sly08,
    author = "Allan Sly",
    title = "Reconstruction of Random Colourings",
    journal = "	Communications in Mathematical Physics",
    volume = "288",
    number = "3",
    year = 2009,
    pages = "943-961"
}

@article{MontanariRicci08,
    author = "A. Montanari and F. Ricci-Tersenghi and G. Semerjian",
    title = "Clusters of solutions and replica symmetry breaking in random k-satisfiability",
    journal = "J. Stat. Mech.",
    year = 2008,
    pages = "P04004"
}

@article{MontanariSemerjian05,
author = "A. Montanari and G. Semerjian",
title = "From Large Scale Rearrangements to Mode Coupling Phenomenology",
journal = "Phys. Rev. Lett.",
year = "2005",
volume = "94",
pages = "247201"}


@article{MontanariSemerjian06,
author = "A. Montanari and G. Semerjian",
title = "On the dynamics of the glass transition on Bethe lattices",
journal="J. Stat. Phys.",
volume=124,
pages="103--189",
year=2006
}

@article{MontanariSemerjian06b,
author = "A. Montanari and G. Semerjian",
title = "Rigorous Inequalities between Length and Time Scales in Glassy Systems",
journal="J. Stat. Phys.",
volume=125,
pages="23",
year=2006,
eprint = "cond-mat/0603018"}

@article{MontanariZecchina02,
      author = "A. Montanari and R. Zecchina",
      title = " Optimizing Searches via Rare Events",
      journal = "Phys. Rev. Lett.",
      volume = 88,
      pages = "178701",
      year = 2002}

@article{Moore02,
    author = "M. A. Moore",
    title = "Corrections to scaling in the droplet picture of spin
glasses",
    year = 2002,
  note = "cond-mat/0203469"}

@article{MooreBokil98,
    author = "M. A. Moore and H. Bokil and B. Drossel",
    title = "Evidence for the Droplet Picture of Spin Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1998,
    volume = 81,
    pages = "4252--4255"}

@article{MooreDrossel02,
    author = "M. A. Moore and B. Drossel",
    title = "p-spin model in finite dimensions and its relation to
structural glasses",
    year = 2002,
  note = "cond-mat/0201107"}

@article{JansonMossel04,
    author = "Svante Janson and Elchanan Mossel",
    title = "Robust reconstruction on trees is determined by the second eigenvalue",
    journal = "Ann. Probab.",
    year = 2004,
    volume = 32,
    pages = "2630-2649"
  }

@article{Mossel01,
    author = "Elchanan Mossel",
    title = "Reconstruction on Trees: Beating the Second Eigenvalue",
    journal = "Ann. Appl. Probab.",
    year = 2001,
    volume = 11,
    number = "1",
    pages = "285-300",
  }
 

@InProceedings{Mossel04,
    author = "E. Mossel",
    title ="Survey: Information flow on trees",
    booktitle ="Graphs, Morphisms and Statistical Physics",
  editor="J. Nestril and P. Winkler",
  series="DIMACS series in discrete mathematics and theoretical computer science",
  pages = "155--170",
  year = 2004}

@article{Moukarzel03,
      author = "C. F. Moukarzel",
      title = "Rigidity percolation in a field",
     journal = "Phys. Rev. E",
      volume =  68,
      pages = "056104",
      year = 2003}

@article{MourikSaad02,
      author = "J. van Mourik and D. Saad",
      title = "Random graph coloring: Statistical physics approach",
     journal = "Phys. Rev. E",
      volume =  66,
      pages = "056120",
      year = 2002}

@article{MuellerMezard04,
      author = "M. M{\"u}ller and M. M{\'e}zard and A. Montanari",
      title = "Glassy phases in Random Heteropolymers with correlated sequences",
     journal = "J. Chem. Phys.",
      volume =  120,
      pages = "11233",
      year = 2004}

@article{MuhlenbeinGeorgesSchleuter88,
        author  = "H. M{\"u}hlenbein and M. Georges-Schleuter and O.
Kramer",
        title   = "Evolution Algorithms in Combinatorial
Optimization",
        journal = "Parallel Computing",
        year = 1988,
        volume = 7,
        pages = 65}

@article{MuletPagnani01,
    author = "R. Mulet and A. Pagnani and G. Parisi",
    title = "Against temperature chaos in naive
            Thouless-Anderson-Palmer equations",
    journal = "Phys. Rev. B",
    year = 2001,
    volume = 63,
    pages = "184438"}

@article{MuletPagnani02,
    author = "R. Mulet and A. Pagnani and M. Weigt and R. Zecchina",
    title = "Coloring random graphs",
  journal = "Phys. Rev. Lett.",
   year = 2002,
   volume = "89",
   pages = "268701"}

@article{Muller02,
    author = "M. M{\"u}ller",
    title = " ",
    journal = " ",
    year = 2002,
    volume = " ",
    pages = " ",
 note = "In preparation"
}

@article{MullerKrzakala02,
    author = "M. M{\"u}ller and F. Krzakala and M. M{\'e}zard",
    title = "The secondary structure of RNA under tension",
    journal = " ",
    year = 2002,
    volume = " ",
    pages = " ",
 note = "cond-mat/0206348"
}

@book{Mydosh93,
    author = "J.A. Mydosh",
  title = "      Spin Glasses: An experimental introduction",
  year = 1993,
  publisher = "Taylor and Francis, London"}

@article{Nagata79,
      author = "S. Nagata and P.H. Keson and H.R. Harrison",
      year = 1979,
       journal = "Phys. Rev. B",
       volume = 19,
    pages = "1633"}

@article{NairPrabhakar03,
  author = "C. Nair, B. Prabhakar and M. Sharma",
  title = "A proof of the conjecture due to {P}arisi for the finite
random assignment problem",
  year = 2003,
  note = "available at http://www.stanford.edu/$\sim$balaji/rap.html"
}

@incollection{Nattermann98,
      author = "T. Nattermann",
      title = "Theory of the Random Field Ising Model",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@article{Nemoto87,
    author = "K. Nemoto",
    title = "A numrical study of the pure states of the SK spin glass
model",
    journal = "J. Phys. C.",
    year = 1987,
    volume = 20,
    pages = "1325--1336"}

@article{NemotoTakayama85,
    author = "K. Nemoto and H. Takayama",
    title = "TAP free energy structure of spin glasses",
    journal = "J. Phys. C.",
    year = 1985,
    volume = 18,
    pages = "529--535"}

@Article{NewmanStein92,
  title = {Multiple states and thermodynamic limits in short-ranged Ising spin-glass models},
  author = {Newman, C. M. and Stein, D. L.},
  journal = {Phys. Rev. B},
  volume = {46},
  number = {2},
  pages = {973--982},
  numpages = {9},
  year = {1992},
  month = {Jul},
  doi = {10.1103/PhysRevB.46.973},
  publisher = {American Physical Society}
}


@article{NewmanStein01,
    author = "C. M. Newman and D. L. Stein",
    title = "Interfaces and the Question of Regional Congruence in Spin
Glasses",
    journal = "Phys. Rev. Lett",
    year = 2001,
    volume = 87,
    pages = "077201"}

@article{NewmanStein02,
    author = "C. M. Newman and D. L. Stein",
    title = "The State(s) of Replica Symmetry Breaking: Mean Field
Theories vs. Short-Range Spin Glasses",
    journal = "J. Stat. Phys.",
  year= 2002,
    volume = 106,
    pages = "213--244"}

@article{NewmanStein96,
    author = "C. M. Newman and D. L. Stein",
    title = "Non-Mean-Field Behavior of Realistic Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1996,
    volume = 76,
    pages = "515--518"}

@article{NewmanStein96b,
    author = "C. M. Newman and D. L. Stein",
    title = "Spatial Inhomogeneity and Thermodynamic Chaos",
    journal = "Phys. Rev. Lett.",
    year = 1996,
    volume = 76,
    pages = "4821--4824"}

@article{NewmanStein96c,
    author = "C. M. Newman and D. L. Stein",
    title = "Ground-State Structure in a Highly Disordered Spin-Glass
Model",
    journal = "J. Stat. Phys.",
    year = 1996,
    volume = 82,
    pages = "1113--1132"}

@article{NewmanStein97,
    author = "C. M. Newman and D. L. Stein",
    title = "Metastate Approach to Thermodynamic Chaos",
    journal = "Phys. Rev. E",
    year = 1997,
    volume = 55,
    pages = "5194--5211"}
    note = " cond-mat/0007493"}

@article{NewmanStein98,
    author = "C. M. Newman and D. L. Stein",
    title = "Simplicity of State and Overlap Structure in Finite-Volume
    Realistic Spin Glasses",
    journal = "Phys. Rev. E",
    year = 1998,
    volume = 57,
    pages = "1356--1366"}

@article{NewmanStrogatz01,
      author = "M. E. J. Newman and S. H. Strogatz and D. J. Watts",
      title = "Random graphs with arbitrary degree distribution and
their applications",
      journal = "Phys. Rev. E",
      volume = 64,
      pages = "026118",
      year = 2001}

@article{NifleHilhorst92,
    author = "M.~Ney-Nifle and H.~Hilhorst",
    title = "A new critical point exponent and new scaling laws for short
range Ising spin glasses",
    journal = "Phys. Rev. Lett",
    year = 1992,
    volume = 68,
    pages = "2992--2995"}

@article{NifleHilhorst93,
   author = "M. Nifle and H. J. Hilhorst",
   title = "",
   journal = "Physica A",
   year = 1993,
   volume = 193,
   pages = "48--"}

@Article{NishimoriStephen83,
  title = {Gauge-invariant frustrated Potts spin-glass},
  author = {Nishimori, Hidetoshi  and Stephen, Michael J.},
  journal = {Phys. Rev. B},
  volume = {27},
  number = {9},
  pages = {5644--5652},
  numpages = {8},
  year = {1983},
  month = {May},
  doi = {10.1103/PhysRevB.27.5644},
  publisher = {American Physical Society}
}



@article{NishimoriWong99,
   author = "H. Nishimori and K. Y. Michael Wong",
   title = "Statistical mechanics of image restoration and error-correcting codes",
   journal = "Phys. Rev. E",
   year = 1999,
   volume = 60,
   pages = "132–144"}

@article{Nishimori81,
   author = "H. Nishimori",
   title = "Internal Energy, Specific Heat and Correlation Function of the Bond-Random Ising Model",
   journal = "Progress of Theoretical Physics",
   year = 1981,
   volume = 66,
   number = 4,
   pages = "1169-1181"}


@book{NishimoriBook01,
    author = "H. Nishimori",
    title = "Statistical Physics of Spin Glasses and Information
Processing:
           An Introduction",
    publisher = "Oxford University Press",
    year = 2001,
    address = "Oxford, UK"}

@unpublished{KrzakalaZdeborova10,
    author = "F. Krzakala and L. Zdeborov\'a",
    note = "in preparation",
    year = "2010"
}

@incollection{NordbladSvedlindh98,
      author = "P. Nordblad and P. Svedlindh",
      title = "Experiments on Spin Glasses",
      editor = "A. P. Young",
      booktitle = "Spin Glasses and Random Fields",
      year = 1998,
      address = "Singapore",
      publisher = "World Scientific"}

@article{ONeil69,
      author = "P. E. O'Neil",
      title = "Asymptotics and random matrices with row-sum and column-sum restrictions",
      journal = "Bull. Am. Math. Soc.",
      volume = 75,
      pages = "1276-1282",
      year = 1969}

@article{OcioHammann90,
    author = "M. Ocio and J. Hammann and E. Vincent",
    journal = "J. Physique Lett.",
    year = 1990,
    volume = "90-91",
    pages = "329"}

@article{Onsager44,
    author = "L. Onsager",
  title = "A two dimensional model with an order-disorder transition",
    journal = "Phys. Rev",
    year = 1965,
    volume = "65"}

@article{Orland85,
    author = "H. Orland",
    title = "Mean-Field Theory for Optimization Problems",
    journal = "J. Physique Lett.",
    year = 1985,
    volume = 46,
    pages = "L763--L770"}

@article{OrlandZee01,
        author = "H. Orland and A. Zee",
        title = "RNA Folding and Large N Matrix Theory",
        year = 2001,
  journal = "Nucl. Phys. B",
        note = "cond-mat/0106359"}

@article{OrlyanchikVaknin02,
        author = "V. Orlyanchik and A. Vaknin and Z. Ovadyahu and M.
Pollak",
        title = "Impairing the memory of an electron-glass by IR
excitation",
        year = 2002,
  journal = "Physica Status Solidi",
         pages= "61-66",
         volume =230}

@article{OzekiNishimori87a,
        author = "Y. Ozeki and N. Nishimori",
        title = "Phase diagram of the {+/-J} {I}sing model in two
dimensions",
        year = 1987,
        journal = "J. Phys. Soc. Jpn.",
        pages= "3265",
        volume =56}

@article{OzekiNishimori87b,
        author = "Y. Ozeki and N. Nishimori",
        title = "Phase diagram and critical exponents of the {+/- J}
                 {I}sing model in finite dimensions by
                 Monte Carlo renormalization group",
        year = 1987,
        journal = "J. Phys. Soc. Jpn.",
        pages= "1568",
        volume =56,
        note="Addendum : 56 (1987) 2992"}

@article{OzekiNishimori87c,
        author = "Y. Ozeki and N. Nishimori",
        title = "",
        year = 1987,
        journal = "J. Phys. Soc. Jpn.",
        pages= "2992",
        volume =56}

@article{PagnaniParisi00,
    author = "A. Pagnani and G. Parisi and F. Ricci-Tersenghi",
    title = "Glassy transition in a disordered model for the RNA secondary
structure",
    journal = "Phys. Rev. Lett.",
    year = 2000,
    volume = 84,
    pages = "2026--2030"}

@article{PagnaniParisi00reply,
    author = "A. Pagnani and G. Parisi and F. Ricci-Tersenghi",
    title = "Reply to the Comment on 'Glassy transition in a disordered
model for the RNA secondary structure'",
    journal = "Phys. Rev. Lett.",
    year = 2001,
    volume = 86,
    pages = "1383"}

@article{PagnaniParisi03,
      author = "A. Pagnani and G. Parisi and M. Rati{\'e}ville",
      title = "Near optimal configurations in mean field disordered systems",
      journal = "Phys. Rev. E",
      volume = 68,
      pages = "046706",
      year = 2003}

@article{Pal95,
   author = "K. F. P\'al",
   title = "Genetic algorithm with local optimization",
   journal = "Biol. Cybern.",
   year = "1995",
   volume = "73",
   pages = "335--341"}


@article{Pal96a,
   author = "K. F. P\'al",
   title = "The ground state energy of the {E}dwards-{A}nderson
            {I}sing spin glass with a hybrid genetic algorithm",
   journal = "Physica A",
   year = "1996",
   volume = "223",
   pages = "283-292"}

@article{Pal96b,
   author = "K. F. P\'al",
   title = "The ground state of the cubic spin glass with
            short-range interactions of {G}aussian distribution",
   journal = "Physica A",
   year = "1996",
   volume = "233",
   pages = "60-66"}

@article{Palassini03,
      author = " M. Palassini",
      title = "Ground-state energy fluctuations in the {S}herrington-{K}irkpatrick model",
      note = "cond-mat/0307713",
      year = 2003}
%   note = "cond-mat/0009418"


@article{PalassiniCaracciolo99,
    author = "M. Palassini and S. Caracciolo",
    title = "Universal Finite Size Scaling Functions in the {3D} {I}sing
             Spin Glass",
    year = 1999,
  journal = "Phys. Rev. Lett.",
  year = "1999",
  volume = "82",
  pages = " 5128--5131",
    note = "cond-mat/9904246"}

@InProceedings{PalassiniCaracciolo99b,
    author = "M. Palassini and S. Caracciolo",
    title = "Monte Carlo Simulation of the Three-dimensional Ising Spin
Glass",
    booktitle = {Procedings of the Workshop "Computer Simulation
               Studies in Condensed Matter Physics XII"},
  year = 1999,
  editor = "D.P. Landau and S.P. Lewis and
       H.B. Schuettler",
    address = "Heidelberg, Berlin, Germany",
    publisher = "Springer Verlag",
    note = "cond-mat/9911449"
}

@article{PalassiniLiers03,
    author = "M. Palassini and F. Liers and M. Juenger and A. P. Young",
    title = "Low Energy Excitations in Spin Glasses from Exact Ground
States",
  journal = "",
    year = "",
  volume = "",
  pages = "",
    note = "cond-mat/0212551"}

@article{PalassiniYoung00a,
    author = "M. Palassini and A. P. Young",
    title = "Nature of the Spin Glass State",
  journal = "Phys. Rev. Lett.",
    year = 2000,
  volume = 85,
  pages = "3017",
    note = "cond-mat/0002134"}

@article{PalassiniYoung00b,
    author = "M. Palassini and A. P. Young",
    title = "Reply to Comment on ``Triviality of the Ground State
           Structure in Ising Spin Glasses''",
    year = 2000,
    note = "cond-mat/0004485"}

@article{PalassiniYoung01,
    author = "M. Palassini and A. P. Young",
    title = "The +/-{J} Spin Glass: Effects of Ground State Degeneracy",
  journal = "Phys. Rev. B",
    year = 2001,
  volume = 63,
  pages = "140408(R)",
    note = "cond-mat/0012161"}

@article{PalassiniYoung99,
    author = "M. Palassini and A. P. Young",
    title = "Trivial Ground State Structure in the
                 two-dimensional {I}sing spin glass",
  journal = "Phys. Rev. B.",
    year = 1999,
  volume = 60,
  pages = "9919",
    note = "cond-mat/9904206"}

@article{PalassiniYoung99a,
    author = "M. Palassini and A. P. Young",
    title = "Triviality of the Ground State Structure in {I}sing
        Spin Glasses",
  journal = "Phys. Rev. Lett.",
    year = 1999,
  volume = 83,
  pages = "5126--5129",
    note = "cond-mat/9906323"}

@article{PalassiniYoung99b,
    author = "M. Palassini and A. P. Young",
    title = "Ground State Structure of Spin Glasses",
  journal = "Journal of the Physical Society of Japan",
  year = 2000,
  volume = 69,
  pages = "165",
    note = "cond-mat/9910278"}

@book{Papadimitriou94,
  author ="C. H. Papadimitriou",
    title ="Computational complexity",
    publisher ="Addison-Wesley",
    year = 1994
}

@book{PapadimitriouSteiglitz82,
    author = "C. H. Papadimitriou and K. Steiglitz",
    title = "Combinatorial Optimization: Algorithms and Complexity",
    publisher = "Prentice Hall",
    year = 1982,
    address = "Englewood Cliffs, NJ"}

@unpublished{Parisi02,
    author = "G. Parisi",
    title = "The physical meaning of Replica Symmetry Breaking",
    year = 1999,
    note = "Dirac Medail lecture, cond-mat/9801176"}

@article{Parisi79,
    author = "G. Parisi",
    title = "Toward a Mean-Field Theory for Spin-Glasses",
    journal = "Phys. Lett.",
    year = 1979,
    volume = "73A",
    pages = "203--205"}

@article{Parisi79b,
    author = "G. Parisi",
    title = "Infinite Number of Order Parameter for Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1979,
    volume = 43,
    pages = "1754--1756"}

@article{Parisi80,
    author = "G. Parisi",
    title = "A Sequence of Approximated Solutions to the {SK} Model for
        Spin-Glasses",
    journal = "J. Phys. A Lett.",
    year = 1980,
    volume = 13,
    pages = "L115--L121"}

@article{Parisi80b,
    author = "G. Parisi",
    title = "The Order Parameter for Spin-Glasses: A Function on the
    Interval 0--1",
    journal = "J. Phys. A",
    year = 1980,
    volume = 13,
    pages = "1101--1112"}

@article{Parisi80c,
    author = "G. Parisi",
    title = "Magnetic Properties of Spin-Glasses in a New Mean-Field
        Theory",
    journal = "J. Phys. A",
    year = 1980,
    volume = 13,
    pages = "1887--1895"}

@article{Parisi83,
    author = "G. Parisi",
    title = "Order Parameter for Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1983,
    volume = 50,
    pages = "1946--1948"}

@article{Parisi86,
    author = "G. Parisi",
    title = "Asymmetric Neural Networks and the Process of Learning",
    journal = "J. Phys. A Lett.",
    year = 1986,
    volume = 19,
    pages = "L675--L680"}

@article{Parisi98,
  author = "G. Parisi",
  title = "A conjecture on random bipartite matchings",
  year = 1998,
  note = "arXiv:cond-mat/9801176"
}

@unpublished{Parisi98,
    author = "G. Parisi",
    title = "A Conjecture on Random Bipartite Matching",
    year = 1998,
    note = "cond-mat/9801176"}

@unpublished{Parisi03,
    author = "G. Parisi",
    title = "Some remarks on the survey decimation algorithm for K-satisfiability",
    year = 2003,
    note = "arXiv:cs/0301015"}

@unpublished{Parisi02b,
    author = "G. Parisi",
    title = "On local equilibrium equations for clustering states",
    year = 2002,
    note = "arXiv:cs.CC/0212047"}

@unpublished{Parisi02c,
    author = "G. Parisi",
    title = "On the survey-propagation equations for the random K-satisfiability problem",
    year = 2002,
    note = "arXiv:cs.CC/0212009"}

@article{DallAstaRamezanpour08,
    author = "L. Dall'Asta and A. Ramezanpour and R. Zecchina",
    title = "Entropy landscape and non-Gibbs solutions in constraint satisfaction problems",
    journal = "Phys. Rev. E",
    volume = "77",
    pages = "031118",
    year = 2008,
  }

@article{ParisiPetronzio01,
    author = "G. Parisi and R. Petronzio and F. Rosati",
    title = "Renormalization Group Approach to Spin Glass Systems",
    journal = "Eur. Phys. J. B",
    year = 2001,
    volume = 21,
    pages = "605--609"}

@article{ParisiPicco99,
    author = "G. Parisi and M. Picco and F. Ritort",
    title = "Continuous phase transition in a spin-glass model
           without time-reversal symmetry",
    journal = "Phys. Rev. E",
    year = 1999,
    volume = 60,
    pages = "58-68"}

@article{ParisiRatieville01,
  author = "G. Parisi and M. Rati\'eville",
  title = "Neighborhood preferences in random matching problems",
  journal = "Eur. J. Phys. B",
    year = 2001,
    volume = 22,
    pages = "229--237"}

@article{ParisiRatieville02,
  author = "G. Parisi and M. Rati\'eville",
  title = "On the finite size corrections to some random matching
problems",
 journal = "Eur. J. Phys. B",
    year = 2002,
    volume = 29,
    pages = "4--57"}

@article{ParisiRicci98,
    author = "G. Parisi and F. Ricci-Tersenghi and J. {Ruiz-Lorenzo}",
    title = "Dynamics of the Four-Dimensional Spin Glass in a Magnetic
        Field",
    journal = "Phys. Rev. B",
    year = 1998,
    volume = 57,
    pages = "13617--13623"}

@article{ParisiRizzo08,
    author = "G. Parisi and T. Rizzo",
    title = "Large Deviations in the Free Energy of Mean-Field Spin Glasses",
    journal = "Phys. Rev. Lett.",
    year = 2008,
    volume = 101,
    pages = "117205"}

@article{ParisiRizzo09,
    author = "G. Parisi and T. Rizzo",
    title = "Phase diagram and large deviations in the free energy of mean-field spin glasses",
    journal = "Phys. Rev. B",
    year = 2009,
    volume = 79,
    pages = "134205"}

@article{ParisiRizzo10,
    author = "G. Parisi and T. Rizzo",
    title = "Large deviations of the free energy in diluted mean-field spin-glass",
    journal = "J. Phys. A: Math. Theor.",
    year = 2010,
    volume = 43,
    pages = "045001"}

@article{ParisiRitort93a,
    author = "G. Parisi and F. Ritort and F. Slanina",
    title = "Critical finite-size corrections for the
Sherrington-Kirkpatrick spin glass",
    journal = "J. Phys. A",
    year = 1993,
    volume = 26,
    pages = "247-259"}

@article{ParisiRitort93b,
    author = "G. Parisi and F. Ritort and F. Slanina",
    title = "Several results on the finite-size corrections in the
Sherrington-Kirkpatrick spin-glass model",
    journal = "J. Phys. A",
    year = 1993,
    volume = 26,
    pages = "3775-3789"}

@book{Pastur,
  author = "M. Lifshitz and S.~A. Gredeskul and L.~A.~Pastur",
  title = "Introduction to the theory of disordered systems",
  year = 1988,
    publisher = "Wiley, New York"}

@article{PercusMartin96,
    author = "A. G. Percus and O. C. Martin",
    title = "Finite Size and Dimensional Dependence in the {E}uclidean
        Traveling Salesman Problem",
    journal = "Phys. Rev. Lett.",
    year = 1996,
    volume = 76,
    pages = "1188--1191"}

@article{PercusMartin99,
    author = "A. G. Percus and O. C. Martin",
    title = "The Stochastic Traveling Salesman Problem: Finite Size
Scaling
        and the Cavity Prediction",
    year = 1999,
    volume = 94,
    journal = "J. Stat. Phys."}

@article{PetitFruchter02,
  author = "D. Petit and L. Fruchter and I. A. Campbell",
  title =  "Ordering in heisenberg Spin Glass",
  year = "2002",
  journal = "Phys. Rev. Lett.",
  volume = "88",
pages = "207206"}

@article{PetitFruchter99,
  author = "D. Petit and L. Fruchter and I. A. Campbell",
  title =  "Ordering in a spin glass under applied magnetic field",
  year = "1999",
  journal = "Phys. Rev. Lett.",
  volume = "83",
  pages = "5130-5133"}

@article{PicaTarzia02,
    author = "M. Pica Ciamarra and M. Tarzia and A. de Candia and A. Coniglio",
    title = "A lattice glass model with no tendency to crystallize",
  journal = "Phys. Rev. E",
   year = 2003,
   volume = "67",
   pages = "057105"}

@article{PiccoRicci01,
    author = "M. Picco and F. Ricci-Tersenghi and F. Ritort",
    title = "Aging effects and dynamic scaling in the 3d Edwards-Anderson
spin glasses: a comparison with experiments",
    year = 2001,
    journal = "Eur. Phys. J. B",
    volume = 21,
    pages = "211"}

@article{PiccoRicci01b,
      author = "M. Picco and F. Ricci-Tersenghi and F. Ritort",
      title = "Chaotic, memory, and cooling rate effects in spin
glasses:
               Evaluation of the Edwards-Anderson model",
      journal = "Phys. Rev. B",
      volume = 63,
      pages = "174412",
      year = 2001}

@article{PiccoRitort01,
    author = "M. Picco and F. Ritort and M. Sales",
    title = "Statistics of lowest excitations in two dimensional Gaussian
spin glasses",
    year = 2001,
  note = "cond-mat/0106554"}

@article{PiccoRitort94,
    author = "M. Picco and F. Ritort",
    title = "Numerical Study of the Ising Spin Glass in a Magnetic
Field",
    year = 1994,
    journal = "J. Phys. I France",
    volume = 4,
    pages = "1619--1625"}

@article{PiccoRitort98,
    author = "M. Picco and F. Ritort",
    title = "Tempering Simulations in the Four Dimensional {+-J}
                 {I}sing Spin Glass in a Magnetic Field",
    year = 1998,
    journal = "Physica A",
    volume = 250,
    pages = "46--57"}

@article{Pierskalla68,
  author = "W. P. Pierskalla",
  title = "The multidimensional assignment problem",
  journal = "Operations Research",
    year = 1968,
    volume = 16,
    pages = "422--431"}

@article{PimentelTemesvari02,
    author = " I. R. Pimentel and T. Temesvari and C. De Dominicis",
    title = "Spin glass transition in a magnetic field : a renormalization
group study",
    year = 2002,
    journal = "Phys. Rev. B",
    volume = "65",
    pages = "224420"}

@article{PitmanYor97,
      author = "J. Pitman and M. Yor",
      title = "The two-parameter Poisson-Dirichlet distribution derived from a stable subordinator",
      journal = "Ann. Probab.",
      volume = 25,
      pages = "855-900",
      year = 1997}

@article{PittelSpencer96,
      author = "B. Pittel and J. Spencer and N.C. Wormald",
      title = "Sudden emergence of a giant $k$-core in a random graph",
      journal = "J. Comb. Theory Ser. B",
      volume = 67,
      pages = "111-151",
      year = 1996}


@article{Poore94,
  author = "A. B. Poore",
  title = "Multidimensional assignment formulation of data association
problems arising from multitarget and multisensor tracking",
  journal = "Comput. Opt. Appl.",
    year = 1994,
    volume = 3,
    pages = "27--54"}

@article{PusztaszeriRensing95,
  author = "J. Pusztaszeri and P. E. Rensing and T. M. Liebling",
  title = "Tracking elementary particles near their primary vertex: a
combinatorial approach",
  journal = "Journal of Global Optimization",
    year = 1995,
    volume = 16,
    pages = "422--431"}

@article{RammalAngles85,
    author = "R. Rammal and J.-C. {Angles d'Auriac} and B. Doucot",
    title = "On the Degree of Ultrametricity",
    journal = "J. Physique Lett.",
    year = 1985,
    volume = 46,
    pages = "L945--L952"}

@book{Reeves93,
      Author = "C. R. Reeves",
      Title = "Modern Heuristic Techniques for Combinatorial
Problems",
      year = 1993,
      publisher = "Halsted Press",
      address = "New York",
      annotate = "A collection of papers on heuristic techniques,
including
      simulated annealing and tabu search."}

@article{Reinelt91,
         Author = "G. Reinelt",
         Title = "{TSPLIB} --- A Traveling Salesman Problem Library",
         Journal = "ORSA Journal on Computing",
         volume = 3,
         year = 1991,
         pages = "376--384",
     note =

"www.iwr.uni-heidelberg.de/\-iwr/\-comopt/\-soft/\-TSPLIB95/\-TSPLIB.html"}

@article{RekaBarabasi02,
      author = "A. R{\'e}ka and A.-L. Barab{\'a}si",
      title = "Statistical mechanics of complex networks",
      journal = "Rev. Mod. Phys.",
      volume = 74,
      pages = "47",
      year = 2002}

@article{RicciRitort00,
      author = " F. Ricci-Tersenghi and F. Ritort",
      title = "Absence of aging in the remanent magnetization
               in Migdal-Kadanoff spin glasses",
      journal = "J. Phys. A",
      volume = 33,
      pages = "3727",
      year = 2000}

@article{RicciWeigt01,
      author = "F. Ricci-Tersenghi and M. Weigt and R. Zecchina",
      title = "Simplest random $K$-satifiablitity problem",
      journal = "Phys. Rev. E",
      volume = 63,
      pages = "026702",
      year = 2001}

@article{RichardsonShokrollahi01,
      author = "T. J. Richardson and M. A. Shokrollahi and R. L. Urbanke",
      title = "Design of capacity-approaching irregular low-density parity-check codes",
      journal = "IEEE Trans. Inform. Theory",
      volume = 47,
      pages = "619--637",
      year = 2001}

@article{CaponeCastellani06,
author = {Barbara Capone and Tommaso Castellani and Irene Giardina and Federico Ricci-Tersenghi},
collaboration = {},
title = {Off-equilibrium confined dynamics in a glassy system with level-crossing states},
publisher = {APS},
year = {2006},
journal = {Physical Review B (Condensed Matter and Materials Physics)},
volume = {74},
number = {14},
eid = {144301},
numpages = {7},
pages = {144301},
keywords = {spin glasses; thermodynamics; energy level crossing; spin dynamics},
doi = {10.1103/PhysRevB.74.144301}
}


@article{RichardsonUrbanke01,
    author = "T. Richardson and R. Urbanke",
    title = "The Capacity of Low-Density Parity-Check Codes Under Message-Passing Decoding",
    journal = "IEEE Trans. Inform. Theory",
    volume = "47",
    year = "2001",
    url = "citeseer.ist.psu.edu/richardson98capacity.html" }

@article{RichertAngell99,
    author = "R. Richert and C.A. Angell",
    journal = "J.Chem.Phys.",
    year = 1999,
    volume = 108,
    pages = "9016"}

@article{Rieger92,
 author = "H. Rieger",
 title =  "The number of solutions of the Thouless-Anderson-Palmer
  equations for p-spin-interaction spin glasses",
 Journal = "Phys. Rev. B",
 volume = 46,
 year = 1992,
 pages = "14655",
}

@article{Rieger93,
    author = "H. Rieger",
    title = "Non-equilibrium Dynamics and Aging in the Three-Dimensional
        {I}sing Spin-Glass Model",
    journal = "J. Phys. A Lett.",
    year = 1993,
    volume = 26,
    pages = "L615--L621"}

@incollection{Rieger95,
    author = "H. Rieger",
    title = "Monte {C}arlo Studies of {I}sing Spin Glasses and Random
        Field Systems",
    booktitle = "Annual Reviews of Computational Physics {II}",
    publisher = "World Scientific",
    year = 1995,
    editor = "D Stauffer",
    address = "Singapore"}

@incollection{Rieger98,
    author = "H. Rieger",
    title = "Frustrated Systems: Ground State Properties via
        Combinatorial Optimization",
    booktitle = "Advances in Computer Simulation",
    publisher = "Springer-Verlag",
    year = 1998,
    editor = "J. Kertesz and I. Kondor",
    address = "Heidelberg",
    series = "Lecture Notes in Physics",
    volume = 501}

@article{RiegerSanten96,
    author = "H. Rieger and L. Santen and U. Blasum and M. Diehl and
             M. J{\"u}nger and G. Rinaldi",
    title = "The critical exponents of the two-dimensional Ising spin
glass revisited: exact ground-state calculations and Monte Carlo
simulations",
    journal = "J. Phys. A",
    year = 1996,
    volume = 29,
    pages = "3939--3950"}

@article{RitortSollich02,
    author = "F. Ritort and P. Sollich",
    title = "Glassy dynamics of kinetically constrained models",
   journal = "Adv. Phys.",
   year = 2003,
   volume = "52",
   pages = "219--342"}

@article{Rivoire04,
      author = "O. Rivoire",
      title = "Properties of atypical graphs from negative complexities",
     journal = "J. Stat. Phys.",
      volume =  117,
      pages = "453",
      year = 2004,
      }

@article{Rivoire05,
      author = "O. Rivoire",
      title = "The cavity method for large deviations",
      journal = "J. Stat. Mech.",
      pages = "P07004",
      year = 2005}

@article{RivoireBiroli04,
      author = "O. Rivoire and G. Biroli and O. C. Martin and M. M{\'e}zard",
      title = "Glass models on Bethe lattices",
     journal = "Eur. Phys. J. B",
      volume =  37,
      pages = "55--78",
      year = 2004,
      }




@article{Rizzo01,
         author = "T. Rizzo",
         title = "Against Chaos in Temperature in Mean-Field
                  Spin-Glass Models",
         journal = "J. Phys. A",
         year = 2001,
         volume = "34",
         pages = "5531-5549"}

@article{Rizzo04,
      author = "T. Rizzo",
      title = "On the complexity of the {B}ethe spin glass",
      note = "cond-mat/0404729",
      journal = "",
      volume = "" ,
      pages = "",
      year = 2004}

@article{RizzoCrisanti02,
         author = "T. Rizzo and A. Crisanti",
         title = "Chaos in temperature in the Sherrington-Kirkpatrick
model",
         year = 2003,
         journal = "Physical Review Letters",
         volume = "90",
         pages = "137201",
}

@article{RouxCates90,
        author = "D. Roux and M. E. Cates and U. Ollson and R. C. Ball
                  and F. Nallet and A. M. Bellocq",
        title = "",
        journal = "Europhys. Lett.",
        year = 1990,
        volume = "11(3)",
        pages = "229--234"}

@article{RouxCates90,
        author = "D. Roux and M. E. Cates and U. Ollson and R. C. Ball
                  and F. Nallet and A. M. Bellocq",
        title = "",
        journal = "Europhys. Lett",
        year = 1990,
        volume = "11(3)",
        pages = "229--234"}

@article{Runnels67,
        author = "L. K. Runnels",
        title = "Phase transition of a {B}ethe lattice gas of hard
molecules",
        journal = "J. Math. Phys.",
        year = 1967,
        volume = "8",
        pages = "2081--2087"}

@article{SalesYoshino02a,
        author = "M. Sales and H. Yoshino",
        title = "Fragility of the glassy state of a directed polymer
                 in random media: a replica approach",
        journal = "",
        year = 2002,
        volume = "",
        pages = "",
        note = "cond-mat/0112384"}

@article{SalesYoshino02b,
  author = "M. Sales and H. Yoshino",
  title  ="Fragility of the Free-Energy Landscape of a Directed
           Polymer in Random Media",
  year   = "2002",
  journal = "Phys. Rev. E",
  volume = "65",
  pages = "066131"}

@article{SasakiDupuis02,
        author = "M. Sasaki and V. Dupuis and J.-P. Bouchaud and E.
Vincent",
        title = "Deviations from Perfect Memory in Spin Glass
                 Temperature Cycling Experiments",
        journal = "Eur. Phys. J. B",
        year = "2002",
        volume = "29",
        pages = "469"}

@article{SasakiMartin02a,
        author = "M. Sasaki and O. C. Martin",
        title = "Discreteness and entropic fluctuations in GREM-like
systems",
        journal = "Phys. Rev. B.",
        year = 2002,
        volume = "66",
        pages = "174411",
}

@article{SasakiMartin02b,
        author = "M. Sasaki and O. C. Martin",
        title = "Temperature chaos in a replica symmetry broken spin
glass
                 model - A hierarchical model with temperature chaos
-",
        journal = "Europhys. Lett.",
        year = 2002,
        volume = "60 (2)",
        pages = "316",
        note = "cond-mat/0206316"}

@article{SasakiNemoto00,
    author = "M. Sasaki and K. Nemoto",
    title = "Memory Effect, Rejuvenation and Chaos Effect
                 in the Multi-Layer Random Energy Model",
    journal = "J. Phys. Soc. Jpn",
    year = 2000,
    volume = 69,
    pages = "2283"}

@article{SaulKardar93,
    author = "L. Saul and M. Kardar",
    title = "Exact integer algorithm for the two-dimensional $\pm {J}$
{I}sing
           spin glass",
    journal = "Phys. Rev. E",
    year = 1993,
    volume = 48,
    pages = "3221--3224"}

@article{SaulKardar94,
    author = "L. Saul and M. Kardar",
    title = "The 2{D} $\pm {J}$ {I}sing spin glass: exact partition
           functions in polynomial time",
    journal = "Nucl. Phys. B [FS]",
    year = 1994,
    volume = 432,
    pages = "641--667"}

@article{Schlijper83,
      author = "A. G. Schlijper",
      title = "Convergence of the cluster-variation method in the thermodynamic limit",
     journal = "Phys. Rev. B",
      volume =  27,
      pages = "6841--6848",
      year = 1983}

@article{SchneiderFroschhammer96,
    author = "J. Schneider and C. Froschhammer and I. Morgenstern and T.
        Husslein and J. Singer",
    title = "Searching for Backbones -- an Efficient Parallel Algorithm
        for the Traveling Salesman Problem",
    journal = "Computer Physics Communications",
    year = 1996,
    volume = 96,
    pages = "173--188"}

@article{SchreiberMartin99,
   author = "G.~R. Schreiber and O.~C. Martin",
   title = "Cut Size Statistics of Graph Bisection Heuristics",
   journal = "SIAM Journal on Optimization",
  volume = "10(1)",
  year = "1999",
   pages = "231--251"}

@article{SellittoBiroli05,
      author = "M. Sellitto and G. Biroli and C. Toninelli",
      title = "Facilitated spin models on {B}ethe lattice: bootstrap percolation, mode-coupling transition and glassy dynamics",
     journal = "Eurphys. Lett.",
      volume =  69,
      pages = "496",
      year = 2005}

@article{Shannon48,
      author = "C. E. Shannon",
      title = "A mathematical theory of communication",
     journal = "Bell System Tech. Journal",
      volume =  27,
      pages = "379--423, 623--655",
      year = 1948}

@article{SherringtonKirkpatrick75,
    author = "D. Sherrington and S. Kirkpatrick",
    title = "Solvable Model of a Spin-Glass",
    journal = "Phys. Rev. Lett.",
    year = 1975,
    volume = 35,
    pages = "1792--1796"}

@article{SimoneDiehl96,
        author = "C. de Simone and M. Diehl and M. Junger and P. Mutzel and G. Reinelt and G. Rinaldi",
        title = "Exact Ground States of Two-Dimensional {+/-J} {I}sing Spin Glasses",
        journal = "J. Stat. Phys.",
        volume = 84,
        year = 1996,
        pages = "1363-1371"}

@article{SkantzosvanMourik03,
        author = "N. S. Skantzos and J. van Mourik and D. Saad and Y. Kabashima",
        title = "Average and reliability error exponents in low-density parity-check codes",
        journal = "J. Phys. A",
        volume = 36,
        year = 2003,
        pages = "11131--11141"}

@phdthesis{Smith89,
    author = "W. D. Smith",
    title = "Studies in Computational Geometry Motivated by Mesh
        Generation",
    school = "Princeton University",
    year = 1989,
    address = "Princeton, NJ"}


@article{SompolinskyZippelius81,
    author = "H. Sompolinski and A. Zippelius",
    title = "Dynamic Theory of the {I}sing Spin-Glass Phase",
    journal = "Phys. Rev. Lett.",
    year = 1981,
    volume = 47,
    pages = "359--362"}

@article{SompolinskyZippelius82,
    author = "H. Sompolinski and A. Zippelius",
    title = "Relaxational Dynamics of the {E}dwards-{A}nderson Model and
        the Mean-Field Theory of Spin-Glasses",
    journal = "Phys. Rev. B",
    year = 1982,
    volume = 25,
    pages = "6860--6875"}

@article{SompolinskyZippelius83,
    author = "H. Sompolinski and A. Zippelius",
    title = "Fluctuations in Short-Range Spin-Glasses",
    journal = "Phys. Rev. Lett.",
    year = 1983,
    volume = 50,
    pages = "1297--1300"}

@article{Sourlas84,
    author = "N. Sourlas",
    title = "Three-Dimensional {I}sing Spin-Glasses and Mean-Field
Theory",
    journal = "J. Physique Lett.",
    year = 1984,
    volume = 45,
    pages = "L969--L975"}

@article{Sourlas86,
    author = "N. Sourlas",
    title = "Statistical Mechanics and the Travelling Salesman Problem",
    journal = "Europhys. Lett.",
    year = 1986,
    volume = 2,
    pages = "919--923"}

@article{Sourlas88,
    author = "N. Sourlas",
    title = "Three-Dimensional {I}sing Spin-Glasses and Ergodicity
        Breaking",
    journal = "Europhys. Lett.",
    year = 1988,
    volume = 6,
    pages = "561--566"}

@article{SouthernChui80,
  title = "Nonuniversality for Two-Dimensional Frustrated Lattices?",
  author = "B. W. Southern and S.T. Chui and G. Forgacs",
  journal = "J.Phys.C",
  volume = 13,
  pages = "L827-30",
  year = 1980}

@article{SouthernYoung77,
  title = "Real space rescaling study of spin glass behaviour
           in three dimensions",
  author = "B. W. Southern and A. P. Young",
    journal = "J.Phys.C",
  volume = 10,
    pages = "2179--2195",
    year = 1977}

@article{SouthernYoung79,
  title = "Effects of Percolation on Spin Glass Order",
  author = "B. W. Southern and A. P. Young and P. Pfeuty ",
  journal = "J.Phys.C",
  volume = 12,
  pages = "683--694",
  year = 1979}

@article{SouthernYoung93,
  title = "Spin Stiffness in Frustrated Antiferromagnets",
  author = "A. P. Young and B. W. Southern",
  journal = "Phys. Rev. B",
  volume = 48,
  pages = "13170--1317",
  year = 1993}

@incollection{Spieksma00,
       author = "F. C. R. Spieksma",
       title = "Multi index assignment problems: complexity,
approximation, applications",
       editor = "L. Pitsoulis and P. Pardalos",
       booktitle = "Nonlinear Assignment Problems, Algorithms and
Applications",
       pages = "1--12",
       year = 2000,
       publisher = "Kluwer, Dordrecht"}

@book{StaufferAharony92,
    author = "D. Staufler and A. Aharony",
    title = "Introduction to Percolation Theory",
  publisher = "Taylor and Francis",
  address = "London",
    year = 1992}

@article{Steele81,
    author = "J. M. Steele",
    title = "Subadditive {E}uclidean Functionals and Nonlinear Growth
        in Geometric Probability",
    journal = "Ann. Probab.",
    year = 1981,
    volume = 9,
    pages = "365--376"}

@book{Steele97,
    author = "J. M. Steele",
    title = "Probability Theory and Combinatorial Optimization",
    publisher = "SIAM",
    year = 1997,
    address = "Philadelphia"}

@book{Struik78,
    author = "L. C. E. Struik",
    title = "Physical aging in amorphous polymers and other materials.",
  publisher = "Elsevier",
    year = 1978,
    address = "Houston"}

@unpublished{KrzakalaRicci09,
    author = "F. Krzakala and F. Ricci-Tersenghi and L. Zdeborov\'a",
    title = "Elusive Glassy Phase in the Random Field Ising Model",
    year = 2009,
    note = "arXiv:0911.1551v1 [cond-mat.dis-nn]",    
}

@unpublished{KrzakalaZdeborova09b,
    author = "F. Krzakala and L. Zdeborov\'a",
    title = "Following Gibbs States adiabatically -- The Energy Landscape of Mean Field Glassy Systems",
    year = "2009",
    note = "arXiv:0909.3820v1 [cond-mat.dis-nn]"
 }

@unpublished{SulcZdeborova09,
    author = "P. \v{S}ulc and L. Zdeborov\'a",
    title = "Belief propagation for graph partitioning",
    year = 2009,
    note = "0912.3563v1 [cond-mat.dis-nn]",    
}

@article{SwendsenWang86,
        author = "R. H. Swendsen and J.-S. Wang",
        title = "Replica Monte Carlo Simulation of Spin-Glasses",
        journal = "Phys. Rev. Lett.",
        year = 1986,
        volume = 57,
        pages = "2607--2609"}

@article{Szipiro03,
        author = "G. Szipiro",
        title = "Does the proof stack up ?",
        journal = "Nature",
        year = 2003,
        volume = "424",
        pages = "12--13"}

@article{Talagrand00,
         author = "M. Talagrand",
        title = "Rigorous low temperature results for the p-spin
                  mean field spin glass model",
         journal = "Probability Theory and Related Fields",
         year = "2000",
         volume = "117",
         pages = "303--360"}

@article{Talagrand06,
		title={The parisi formula},
		author={M. Talagrand},
		journal={Ann. Math.},
		volume=163,
		pages={221--263},
		year=2006
}

@article{PanchenkoTalagrand04,
		title={ Bounds for diluted mean-fields spin glass models},
		author={Dmitry Panchenko and Michel Talagrand},
		journal={Probability Theory and Related Fields},
		volume=130,
                number = 3,
		pages={319-336},
		year=2004
}

@book{Talagrand03,
    author = "M. Talagrand",
    title = "Spin glasses : a challenge for mathematicians. Cavity and mean field models",
  publisher = "Springer-Verlag",
  address = "New-York",
    year = 2003}

@book{Bovier06,
    author = "Anton Bovier",
    title = "Statistical Mechanics of Disordered Systems: A Mathematical Perspective",
  publisher = "Cambridge University Press",
  address = "",
    year = 2006}


@article{Talagrand92,
        author = "M. Talagrand",
        title = "Matching Random Samples in Many Dimensions",
        journal = "Ann. Appl. Probab.",
        year = 1992,
        volume = 2,
        pages = "846--856"}

@article{Tholence74,
    author = "J.L. Tholence and R. Tournier",
    journal = "J. Phys. (Paris)",
    year = 1974,
    volume = 35,
    pages = "C4-229"}

@article{ThorpeJacobs00,
      author = " M. F. Thorpe and D. J. Jacobs and M. V. Chubinsky and J. C. Phillips",
      title = "Self Organization in Network Glasses",
      journal = "J. Non-Cryst. Solids",
      volume = 859,
      pages = "266--269",
      year = 2000}

@article{ThorpeRader01,
      author = "M. F. Thorpe and A. Rader and M. Lei and D. J. Jacobs and L. A. Kuhn",
      title = "Predicting Flexibility in Proteins using Constraint Theory",
      journal = "Journal of Molecular Graphics and Modeling",
      volume = 19,
      pages = "60--69",
      year = 2001}

@article{Thouless86,
    author = "D. J. Thouless",
    title = "Spin-Glass on a {B}ethe Lattice",
    journal = "Phys. Rev. Lett.",
    year = 1986,
    volume = 56,
    pages = "1082--1085"}

@article{ThoulessAnderson77,
    author = "D. J. Thouless and P. W. Anderson and R. G. Palmer",
    title = "Solution of `Solvable Model of a Spin-Glass'",
    journal = "Phil. Mag.",
    year = 1977,
    volume = 35,
    pages = "593--601"}

@article{ToninelliBiroli04,
        author = "C. Toninelli and G. Biroli and D. S. Fisher",
        title = "Spatial structures and dynamics of kinetically constrained models of glasses",
  journal = "Phys. Rev. Lett.",
   year = 2004,
   volume = "92",
   pages = "185504"}

@article{Toulouse77,
    author = "G. Toulouse",
    title = "Theory of Frustration Effect in Spin-Glasses: {I}",
    journal = "Comm. Phys.",
    year = 1977,
    volume = 2,
    pages = "115--119"}

@book{UCIGL99,
  author =   {S. Franz and S.~C Glotzer and S. Sastry},
  editor =   {S. Franz and S.~C Glotzer and S. Sastry},
    title =              {Unifying concepts in glass physics},
    publisher =      {IOP},
    year =               {2000},
    OPTvolume =      {12},
    OPTseries =      {J. Phys C},
  note = "J. Phys C, Vol 12"
}

@article{VaillsQu04,
      author = "Y. Vaills and T. Qu and M. Micoulaut and F. Chaimbault and P. Boolchand",
      title = "Direct evidence of rigidity loss and self-organisation in silicate glasses",
      note = "cond-mat/0406509",
      year = 2004}

@article{VanEnter90,
    author = "A.C.D. van Enter",
    title = "Stiffness Exponent, Number of Pure States, and
                 Almeida-Thouless Line in Spin-Glasses",
    journal = "J. Stat. Phys.",
    year = 1990,
    volume = 60,
    pages = "275--279"}

@article{VannimenusMezard84,
    author = "J. Vannimenus and M. M{\'e}zard",
    title = "On the Statistical Mechanics of Optimization Problems of
        the Travelling Salesman Type",
    journal = "J. Physique Lett.",
    year = 1984,
    volume = 45,
    pages = "L1145--L1153"}

@article{VazquezWeigt03,
    author = "A. Vasquez and M. Weigt",
    title = "Computational complexity arising from degree correlations in
networks",
    journal = "Phys. Rev. E",
  volume ="67",
  pages = "027101",
    year = 2003}

@article{VianaBray85,
    author = "L. Viana and A. J. Bray",
    title = "Phase Diagrams for Dilute Spin-Glasses",
    journal = "J. Phys. C",
    year = 1985,
    volume = 18,
    pages = "3037--3051"}

@article{ViasnoffLequeux02,
    author = "V. Viasnoff and F. Lequeux",
    title = "Rejuvenation and overaging in a colloidal glass under
shear",
    journal = "Phys. Rev. Lett.",
    year = 2002}

@article{Villain86,
    author = "J. Villain",
    journal = "Europhys. Lett.",
    year = 1986,
    volume = 2,
    pages = 871}

@article{Vincent97,
  author = "E. Vincent and J. Hammann and M. Ocio and J.~P. Bouchaud
and L.~F. Cugliandolo",
  title = "Slow dynamics and aging in spin-glasses",
 year=1997,
 note = "cond-mat/9607224 "}

@article{VincentDupuis00,
  author = "E. Vincent and V. Dupuis and M. Alba and J. Hammann and
J.P. Bouchaud",
  titre = "Aging phenomena in spin-glass and ferromagnetic phases:
Domain growth and wall dynamics",
  journal = "Europhys. Lett.",
  year = 2000,
  volume = "50",
  pages = "674-680"}

@InProceedings{VincentHammann00,
    author =    "E. Vincent and J. Hammann and M. Ocio and J.P. Bouchaud
             and L.F. Cugliandolo",
    title =     "Complex behaviour of glassy systems",
    pages =          {184},
    year =       {1997},
    volume =     {476},
    address =    {Germany},
    publisher = "Springer",
    note = "cond-mat/9607224",
}

@article{WangSwendsen88,
   author = "J.-S. Wang and R. H. Swendsen",
   title = "Low-temperature properties of the $\pm {J}$ {I}sing
            spin glass in two dimensions",
   journal = "Phys. Rev. B",
   year = 1988,
   volume = "38",
   pages = "4840--4844"}

@article{WehrAizenman90,
   author = "J. Wehr and M. Aizenman",
   title = "Fluctuations of extensive functions of quenched random
couplings",
   journal = "J. Stat. Phys.",
   year = 1990,
   volume = "60",
   pages = "287--306"}

@article{WeigtHartmann00,
   author = "M. Weigt and A. K. Hartmann",
   title = "The number of guards needed by a museum: A phase transition
in vertex covering of random graphs",
   journal = "Phys. Rev. Lett.",
   year = 2000,
   volume = "84",
   pages = "6118"}

@article{WeigtHartmann01,
   author = "M. Weigt and A. K. Hartmann",
   title = "Minimal vertex covers on finite-connectivity random graphs:
A hard-sphere lattice-gas picture",
   journal = "Phys. Rev. E",
   year = 2001,
   volume = "63",
   pages = "056127"}

@article{WeigtHartmann03,
   author = "M. Weigt and A. K. Hartmann",
   title = "Glassy behavior induced by geometrical frustration in a
hard-core lattice gas model", journal = "Europhys. Lett.",
   year = 2003,
   volume = "62",
   pages = "533--539"}

@article{WeigtHartmann03b,
   author = "M. Weigt and A. K. Hartmann",
   title = "Statistical mechanics of the vertex-cover problem",
   journal = "J. Phys. A",
   volume = "36",
   pages = "11069--11093",
   year = 2003}

@article{Weiss00,
      author = "Y. Weiss",
      title = "Correctness of Local Probability Propagation in Graphical Models with Loops",
      journal = "Neural Comp.",
      volume = 12,
      pages = "1--41",
      year = 2000}

@article{Wilson02,
      author = "David B. Wilson",
      title = "On the critical exponents of random k-SAT",
      journal = "Random Structures and Algorithms",
      volume = 21,
      pages = "182--195",
      year = 2002}


@InProceedings{YedidiaFreeman00, 
    author = "J.S. Yedidia and W.T. Freeman and Y. Weiss",
    title ="Generalized Belief Propagation",
    booktitle ="Advances in Neural Information Processing Systems (NIPS)",
  volume=13,
  pages = "689-695",
  year = 2000}

@InProceedings{AurellGordon04, 
    author = "Erik Aurell and Uri Gordon and Scott Kirkpatrick",
    title ="Comparing Beliefs, Surveys and Random Walks",
    booktitle ="Proc. of 17th NIPS",
    pages = "804",
    year = 2004}


@InProceedings{Wormald99,
    author = "N. C. Wormald",
    title ="Models of random regular graphs",
    booktitle ="Survey in Combinatorics",
  editor="J. D. Lamb and D. A. Preece",
  series="Mathematical Society Lecture Note Series",
  volume=276,
  pages = "239--298",
  publisher = "Cambridge University Press",
  year = 1999}

@article{Wu82,
      author = "F. Y. Wu",
      title = "The {P}otts model",
     journal = "Rev. Mod. Phys.",
      volume =  54,
      pages = "235--268",
      year = 1982}

@inproceedings{Yedidia01,
	author = {Jonathan Yedidia},
	title = {An Idiosyncratic Journey Beyond Mean Field Theory},
	booktitle={Advanced Mean Field Methods, Theory and Practice},
	editor={Manfred Opper and David Saad},
	publisher={The MIT Press},
	year={2001},
	pages={21--36},
	url = {http://www.merl.com/publications/TR2000-027/}
}

@incollection{YedidiaFreeman03,
	author = {Yedidia, J.S. and Freeman, W.T. and Weiss, Y.},
	title = {Understanding Belief Propagation and Its Generalizations},
	booktitle={Exploring Artificial Intelligence in the New Millennium},
	publisher={Science \& Technology Books},
	year={2003},
	pages={239--236},
}


@article{YedidiaFreeman02,
   author = "J. S. Yedidia and W. F. Freeman and Y. Weiss",
   title = "Constructing free energy approximations and generalized
belief propagation algorithms",
   journal = "technical report TR-2002-35, Mitsubishi Electrical
Research Laboratories",
   year = 2002,
   note="available at http://www.merl.com"}

@article{Yoshino97,
   author = "H. Yoshino",
   title = "Hierarchical diffusion, aging and multifractality",
   journal = "J. Phys. A.",
   year = 1997,
   volume = "30",
   pages = "1143--1160"}

@article{YoshinoHukushima02a,
  author = "H. Yoshino and  K. Hukushima and H. Takayama",
 title="Anomalously Soft Droplets and Aging in Short-ranged Spin
Glasses",
  year = 2002,
  note ="cond-mat/0202110"}

@article{YoshinoHukushima02b,
  author = "H. Yoshino and  K. Hukushima and H. Takayama",
 title="Extended droplet theory for aging in short-ranged spin glasses
and a numerical examination",
  year = 2002,
  note ="cond-mat/0203267"}

@article{YoshinoLemaitre00,
  author = "H. Yoshino and A. Lema\^{\i}tre and J.-P. Bouchaud",
 title=" Multiple Domain Growth and Memory in the Droplet Model for
Spin-Glasses",
  journal = "Eur. Phys. J. B.",
  year = 2000,
  volume = "20",
  pages = "367--395",
  note ="cond-mat/0009152"}


@Article{RizzoYoshino06,
  title = {Chaos in glassy systems from a Thouless-Anderson-Palmer perspective},
  author = {Rizzo, Tommaso  and Yoshino, Hajime },
  journal = {Phys. Rev. B},
  volume = {73},
  number = {6},
  pages = {064416},
  numpages = {9},
  year = {2006},
  month = {Feb},
  doi = {10.1103/PhysRevB.73.064416},
  publisher = {American Physical Society}
}



@article{YoshiyukiYoshiki95,
    author = "U. Yoshiyuki and K. Yoshiki",
    title = "New Method of Solving the Traveling Salesman Problem Based
        on Real Space Renormalization Theory",
    journal = "Phys. Rev. Lett.",
    year = 1995,
    volume = 75,
    pages = "1683--1686"}



@article{Young83,
    author = "A. P. Young",
    title = "Direct Determination of the Probability Distribution for
        the Spin-Glass Order Parameter",
    journal = "Phys. Rev. Lett.",
    year = 1983,
    volume = 51,
    pages = "1206--1209"}

@article{Young83b,
  author = "A. P. Young",
  title = "Statics and Dynamics of a Two-Dimensional {I}sing Spin-Glass
Model",
  journal = "Phys. Rev. Lett.",
  year = 1983,
  volume = 50,
  pages = "917--921"}

@book{Young98,
      Editor = "A. P. Young",
      Title = "Spin Glasses and Random Fields",
      Year = 1998,
      address = "Singapore",
      Publisher = "World Scientific"}

@article{YoungPrivate,
      author = "M. Palassini and A. P. Young",
      note = "private communication"}

@article{Zanotto98,
      author = "E.~D. Zanotto",
      title = "Do cathedral glasses flow ?",
      journal = "Am. J. Phys.",
      volume = 66,
      page = 392,
      year = 1998}

@article{Zanotto98,
      author = "E.~D. Zanotto",
      title = "Do cathedral glasses flow ?",
      journal = "Am. J. Phys.",
      volume = 66,
      page = 392,
      year = 1998}


@unpublished{ZhouYang03,
  AUTHOR = {H. Zhou and Z. Ou-Yang},
  TITLE = {Maximum matching on random graphs},
  NOTE = {Preprint arXiv:cond-mat/0309348v1 [cond-mat.dis-nn]},
  YEAR = {2003},
}

@article{Zhou03,
      author = "H. Zhou",
      title = "Vertex cover problem studied by cavity method: Analytics and population dynamics",
     journal = "Eur. Phys. J. B",
      volume =  32,
      pages = "265--20",
      year = 2003}

@article{ZhouZhang01,
  author = "H. Zhou and Y. Zhang",
  title = "Pulling hairpinned polynucleotide chains: Does base-pair
stacking interaction matter?",
  journal = "J. Chem. Phys.",
  volume = 114,
  year = 2001,
  pages = "8694--8700",
}

@article{ZukerSankoff84,
    author =             {M. Zuker and D. Sankoff},
    title =              {},
    journal =        {Bull. Math. Biol. },
    year =               {1984},
    volume =     {46},
  pages = "591"
}


@article{ZukerStiegler81,
    author =             {M. Zuker and P. Stiegler},
    title =              {Optimal computer folding of large RNA sequences using
thermodynamics and auxiliary information},
    journal =        {Nucl. Acid. Res. },
    year =               {1981},
    volume =     {9},
  pages = "133--148"
}

@article{Zukermfold,
    author =             {D. H. Mathews and J. Sabina and M. Zuker and D. H.
Turner },
    title =              {Expanded Sequence Dependence of Thermodynamic Parameters
Improves Prediction of RNA Secondary Structure},
    journal =        {J. Mol. Biol.},
    year =               {1999},
    volume =     {288},
  pages = "911--940"
}

@book{denHollander00,
author = "F. den Hollander",
title = "Large deviations",
series = "Fields Institute Monographs 14",
publisher = "American Mathematical Society",
address = "Providence RI",
year = "2000"}

@InProceedings{BerrouGlavieux93,
author = "C. Berrou and A. Glavieux and P. Thitimajshima",
title = "Near Shannon limit error-correcting coding: Turbo codes",
booktitle = "Proc. IEEE International Conference on Communications",
year = 1993,
pages = "1064-1070"}

@article{Sourlas89,
author= "N. Sourlas",
title = "Spin-glass models as error-correcting codes",
journal = "Nature",
year = 1989,
volume = 339,
pages = "693--694"
}

@article{Sourlas94,
author = "N. Sourlas",
title = "Spin-glasses, error-correcting codes and finite-temperature decoding",
journal = "Europhys. Lett.",
volume = 25,
year = 1994,
pages = "159--164"
}

@incollection{Sourlas94-2,
       author = "N. Sourlas",
       title = "Statistical mechanics and error-correcting codes",
       editor = "P. Grassberger and J.-P. Nadal",
       booktitle = "From Statistical Physics to Statistical Inference and Back",
       pages = "",
       year = 1994,
       publisher = "Kluwer",
adress = "Dordrecht"}

@article{DiProietti02,
author = "C. Di and D. Proietti and I. E. Telatar and T. J. Richardson, R. L. Urbanke",
title = "Finite length analysis of low-density parity-check codes on the binary erasure channel",
journal = "IEEE Trans. Inform. Theory",
volume = 48,
pages = "1570--1579",
year = 2002}

@InProceedings{DiMontanari04,
author = "C. Di and A. Montanari and R. Urbanke",
title = "Weight Distributions of {LDPC} Code Ensembles: Combinatorics Meets Statistical Physics",
booktitle = "International Symposium on Information Theory",
publisher = "IEEE",
adress = "Chicago",
year=2004}

@article{DiRichardson06,
	author={Di, C. and Richardson, T. J. and Urbanke, R.L.},
	title={Weight Distribution of Low-Density Parity-Check Codes},
	journal={IEEE Trans. Inform. Theory},
	volume=52,
	year=2006,
	pages={4839--4855}
}

@article{HaanpaaJarvisalo06,
	author={Harri Haanp\"{a}\"{a} and Matti J\"{a}rvisalo and Petteri Kaski and Ilkka Niemel\"{a}},
	title={Hard Satisfiable Clause Sets for Benchmarking Equivalnce Reasoning Techniques},
	journal={Journal on Satisfiability, Boolean Modeling and Computations},
	volume=2,
	year=2006,
	pages={27--46}
}

@book{ViterbiOmura79,
author = "A. J. Viterbi and J. K. Omura",
title = "Principles of Digital Communication and Coding",
publisher = "McGraw-Hill Int. Ed.",
year=1979,
adress = "Singapore"}

@unpublished{AmraouiMontanari04,
  AUTHOR = {A.~Amraoui and A.~Montanari and T.~Richardson and R.~Urbanke},
  TITLE = {Finite-Length Scaling for Iteratively Decoded LDPC Ensembles},
  NOTE = {Submitted IEEE Trans. on Information Theory. Preprint cs.IT/0406050},
  YEAR = {2004},
  TYPE = {submitted}
}

@article{MoraZdeborova07,
  AUTHOR = {T. Mora and L. Zdeborov\'a},
  TITLE = {Random subcubes as a toy model for constraint satisfaction problems},
  journal = "J. Stat. Phys",
  volume = "131",
  number = "6",
  pages = "1121-1138", 
  YEAR = {2008},
}


@article{SaadKabashima98,
author = "Y. Kabashima and D. Saad",
title = "Belief propagation vs. TAP for decoding corrupted messages",
journal = "Europhys. Lett.",
volume = 44,
pages = "668--674",
year = 1998}

@book{NielsenChuang00,
author = "M. A. Nielsen and I. L. Chuang",
title = "Quantum Computing and Quantum Information",
publisher = "Cambridge University Press",
year=2000}

@article{Condamin02,
author = "S. Condamin",
title = " Study of the weight enumerator function for a Gallager code",
note="http://www.inference.phy.cam.ac.uk/condamin/report.ps",
year=2002}

@article{Verdu98,
author = "S. Verd{\'u}",
title = "Fifty Years of Shannon Theory",
journal = "IEEE Transactions on Information Theory",
volume="44(6)",
year=1998,
pages = "2057--2078"}

@article{Berlekamp02,
author="E. R. Berlekamp",
title = "The Performance of Block Codes",
journal = "Notices of the AMS",
year="January 2002",
pages="17--22"}

@inproceedings{MoraRivoire06,
author="T. Mora and O. Rivoire",
title="Error Exponents of Low-Density Parity-Check Codes on the Binary Erasure Channel",
year="2006",
booktitle={Proc. ITW},
month={october},
pages={81--85},
address={Chengdu, China},
eprint="cs.IT/0605130"}

@INPROCEEDINGS{MeassonMontanari04,
  AUTHOR = {C.~Measson and A.~Montanari and T.~Richardson and R.~Urbanke},
  TITLE = {Life above threshold: from list decoding to area thereom and {MSE}},
  BOOKTITLE = {Proc. ITW},
  YEAR = {2004},
  ADDRESS = {San Antonio, USA},
  MONTH = {October},
  TYPE = {conference}
}

@ARTICLE{MeassonMontanari05,
   author = {{Measson}, C. and {Montanari}, A. and {Urbanke}, R.},
    title = "{Maxwell Construction: The Hidden Bridge between Iterative and Maximum a Posteriori Decoding}",
  journal = {ArXiv Computer Science e-prints},
   eprint = {cs/0506083},
     year = 2005,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2005cs........6083M},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}


@article{MezardMora05,
  author = {M. M\'ezard and T. Mora and R. Zecchina},
  title = {Clustering of solutions in the random satisfiability problem},
  journal = {Physical Review Letters},
  volume = {94},
  pages = {197205},
  year = {2005}
}

@article{MoraMezard05,
  author = {H. Daud\'e and T. Mora and M. M\'ezard and R. Zecchina},
  title = {Pairs of SAT Assignments and Clustering in Random Boolean Formulae},
  journal = "Theoretical Computer Science",
  volume = "393",
  pages = "260-279",
  year = {2008}
}

@article{Friedgut99,
author = "E. Friedgut",
title = "Sharp Thresholds of Graph Proprties, and the $k$-sat Problem", 
journal = "J. Amer. Math. Soc.",
volume = "12",
page = "no. 4, 1017--1054",
year = 1999
}

@article{DuboisMandler02,
author = {O. Dubois and J. Mandler},
title = {The 3-XORSAT Threshold},
journal = {FOCS},
volume = {00},
year = {2002},
issn = {0272-5428},
pages = {769},
doi = {http://doi.ieeecomputersociety.org/10.1109/SFCS.2002.1182002},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@inproceedings{DuboisBoufkhad00,
 author = {Olivier Dubois and Yacine Boufkhad and Jacques Mandler},
 title = {Typical random 3-SAT formulae and the satisfiability threshold},
 booktitle = {SODA '00: Proceedings of the eleventh annual ACM-SIAM symposium on Discrete algorithms},
 year = {2000},
 isbn = {0-89871-453-2},
 pages = {126--127},
 location = {San Francisco, California, United States},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 }

@unpublished{HajiaghayiSorkin03,
   author = {{Hajiaghayi}, M. and {Sorkin}, G.~B.},
    title = "{The Satisfiability Threshold of Random 3-SAT Is at Least 3.52}",
     note = {arXiv: math/0310193},
     year = 2003,
}

@inproceedings{KaporisKirousis03,
  author = "A. Kaporis and L. Kirousis and E. Lalas",
  title = "Selecting complementary pairs of literals",
  booktitle = "Proc. LICS`03 Workshop on Typical Case Complexity and Phase
    Transitions",
  year = "2003",
  url = "citeseer.ist.psu.edu/kaporis03selecting.html" }

@article{AchlioptasNaor05,
author={D. Achlioptas and A. Naor and Y. Peres},
title = {Rigorous location of phase transitions in hard optimization problems},
journal = {Nature},
volume = 435,
year = 2005,
pages={759--764}
}

@article{AchlioptasMoore02,
author = {Dimitris Achlioptas and Cristopher Moore},
title = {The Asymptotic Order of the Random k -SAT Threshold},
journal = {focs},
volume = {00},
year = {2002},
issn = {0272-5428},
pages = {779},
doi = {http://doi.ieeecomputersociety.org/10.1109/SFCS.2002.1182003},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@article{AchlioptasMoore06,
author = {Dimitris Achlioptas and Cristopher Moore},
title = {Two moments suffice to cross a sharp threshold},
journal = {SIAM Journal on Computing},
volume = {36},
year = {2006},
pages = {740--762},
}


@article{AchlioptasPeres04,
author={D. Achlioptas and Y. Peres},
title={The threshold for random $k$-SAT is $2^k  \log 2 - {O}(k)$},
journal={Journal of the AMS},
volume=17,
year=2004,
pages = {947--973}
}

@article{AchlioptasMoore03,
author={D. Achlioptas and C. Moore},
title={Almost all graphs with average degree 4 are 3-colorable},
journal={J. Comput. Syst. Sci.},
volume=67,
year=2003,
pages = {441}
}

@article{Vardy97,
author={A. Vardy},
title = {The intractability of computing the minimum distance of a code},
journal ={IEEE Trans. Inf. Theory},
volume = 43,
year =1997,
pages={1757--1766}
}

@book{RichardsonUrbanke07,
author={T. Richardson and R. Urbanke},
title = {Modern Coding Theory},
year=2007,
publisher = {Cambridge University Press},
note="In preparation, disponible at lthcwww.epfl.ch/mct"
}

@inproceedings{SemerjianMonasson04,
author={G. Semerjian and R. Monasson},
title = {A Study of Pure Random Walk on Random Satisfiability Problems with ``Physical'' Methods},
booktitle = {Proceedings of the {SAT} 2003 conference},
editor={E. Giunchiglia and A. Tachella},
year=2004,
volume=120,
series = {Lecture Notes in Computer Science},
publisher = {Springer},
pages=2919
}

@inproceedings{AchlioptasRicci06,
 author = {Dimitris Achlioptas and Federico Ricci-Tersenghi},
 title = {On the solution-space geometry of random constraint satisfaction problems},
 booktitle = {Proc. of 38th STOC},
 year = {2006},
 pages = {130--139},
 location = {Seattle, WA, USA},
 doi = {http://doi.acm.org/10.1145/1132516.1132537},
 publisher = {ACM},
 address = {New York, NY, USA},
 }


@incollection{CookMitchell97,
    author = "Stephen A. Cook and David G Mitchell",
    title = "Finding Hard Instances of the Satisfiability Problem: {A} Survey",
    booktitle = "Satisfiability Problem: Theory and Applications",
    volume = "35",
    publisher = "American Mathematical Society",
    editor = "Du and Gu and Pardalos",
    pages = "1--17",
    year = "1997",
    url = "citeseer.ist.psu.edu/cook97finding.html" 
}

@inproceedings{AchlioptasBeame01,
    author = "Dimitris Achlioptas and Paul Beame and Michael S. O. Molloy",
    title = "A sharp threshold in proof complexity",
    booktitle = "{ACM} Symposium on Theory of Computing",
    pages = "337--346",
    year = "2001",
    url = "citeseer.ist.psu.edu/achlioptas01sharp.html" }

@article{ChvatalSzemer88,
 author = {Va\v{s}ek ChvÃ¡tal and Endre SzemerÃ©di},
 title = {Many hard examples for resolution},
 journal = {J. ACM},
 volume = {35},
 number = {4},
 year = {1988},
 issn = {0004-5411},
 pages = {759--768},
 doi = {http://doi.acm.org/10.1145/48014.48016},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@article{KirousisKranakis98,
    author = "Lefteris M. Kirousis and Evangelos Kranakis and Danny Krizanc and Yannis C. Stamatiou",
    title = "Approximating the unsatisfiability threshold of random formulas",
    journal = "Random Structures and Algorithms",
    volume = "12",
    number = "3",
    pages = "253-269",
    year = "1998",
    url = "citeseer.ist.psu.edu/kirousis95approximating.html" }

@article{DuboisBoufkhad97,
 author = {O. Dubois and Y. Boufkhad},
 title = {A general upper bound for the satisfiability threshold of random r-SAT formulae},
 journal = {J. Algorithms},
 volume = {24},
 number = {2},
 year = {1997},
 issn = {0196-6774},
 pages = {395--420},
 doi = {http://dx.doi.org/10.1006/jagm.1997.0867},
 publisher = {Academic Press, Inc.},
 address = {Duluth, MN, USA},
 }

@article{ChaoFranco90,
 author = {Ming-Te Chao and John Franco},
 title = {Probabilistic analysis of a generalization of the unit-clause literal selection heuristics for the k satisfiability problem},
 journal = {Inf. Sci.},
 volume = {51},
 number = {3},
 year = {1990},
 issn = {0020-0255},
 pages = {289--314},
 doi = {http://dx.doi.org/10.1016/0020-0255(90)90030-E},
 publisher = {Elsevier Science Inc.},
 address = {New York, NY, USA},
 }

@article{ChaoFranco86,
 author = {Ming-Te Chao and John Franco},
 title = {Probabilistic analysis of two heuristics for the 3-satisfiability problem},
 journal = {SIAM J. Comput.},
 volume = {15},
 number = {4},
 year = {1986},
 issn = {0097-5397},
 pages = {1106--1118},
 doi = {http://dx.doi.org/10.1137/0215080},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 }

@article{DavisLogemann62,
 author = {Martin Davis and George Logemann and Donald Loveland},
 title = {A machine program for theorem-proving},
 journal = {Commun. ACM},
 volume = {5},
 number = {7},
 year = {1962},
 issn = {0001-0782},
 pages = {394--397},
 doi = {http://doi.acm.org/10.1145/368273.368557},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@article{DavisPutnam60,
 author = {Martin Davis and Hillary Putnam},
 title = {A Computing Procedure for Quantification Theory},
 journal = {Journal of the ACM},
 volume = {7},
 number = {3},
 year = {1960},
 pages = {201--215},
 }


@inproceedings{Papadimitriou91,
 author = {Christos H. Papadimitriou},
 title = {On selecting a satisfying truth assignment (extended abstract)},
 booktitle = {Proceedings of the 32nd annual symposium on Foundations of computer science},
 year = {1991},
 isbn = {0-8186-2445-0},
 pages = {163--169},
 location = {San Juan, Puerto Rico},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA},
 }

@article{Ladner75,
 author = {Richard E. Ladner},
 title = {On the Structure of Polynomial Time Reducibility},
 journal = {J. ACM},
 volume = {22},
 number = {1},
 year = {1975},
 issn = {0004-5411},
 pages = {155--171},
 doi = {http://doi.acm.org/10.1145/321864.321877},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@inproceedings{Cook71,
 author = {Stephen A. Cook},
 title = {The complexity of theorem-proving procedures},
 booktitle = {Proc. 3rd STOC},
 year = {1971},
 pages = {151--158},
 location = {Shaker Heights, Ohio, United States},
 doi = {http://doi.acm.org/10.1145/800157.805047},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Goldberg79,
 author = {A. Goldberg},
 title = {On the complexity of the satisfiability problem},
 booktitle = {Courant Computer Science Report},
 volume = {16},
 year = {1979},
 address = {New York, NY, USA},
 }

@article{GoldbergPurdom82,
 author = {A. Goldberg and Jr. P.W. Purdom and C.A. Brown},
 title = {Average time analysis of simplified Davis-Putnam procedure},
 journal = {Information Process. Lett.},
 volume = 15,
 number = 2,
 year = 1982,
 pages = {72--75},
 note = "see also Errata, vol. 16, 1983, p. 213"
 }



@article{FriezeSuen96,
 author = {Alan Frieze and Stephen Suen},
 title = {Analysis of two simple heuristics on a random instance of k-SAT},
 journal = {J. Algorithms},
 volume = {20},
 number = {2},
 year = {1996},
 issn = {0196-6774},
 pages = {312--355},
 doi = {http://dx.doi.org/10.1006/jagm.1996.0016},
 publisher = {Academic Press, Inc.},
 address = {Duluth, MN, USA},
 }

@inproceedings{CheesemanKanefsky91,
    author = "Peter Cheeseman and Bob Kanefsky and William M. Taylor",
    title = "{Where the Really Hard Problems Are}",
    booktitle = "Proc. 12th IJCAI",
    year = "1991",
    pages = "331--337",
    publisher = {Morgan Kaufmann},
    address = {San Mateo, CA, USA},
 }

@article{SelmanMitchell96,
 author = {Bart Selman and David G. Mitchell and Hector J. Levesque},
 title = {Generating hard satisfiability problems},
 journal = {Artif. Intell.},
 volume = {81},
 number = {1-2},
 year = {1996},
 issn = {0004-3702},
 pages = {17--29},
 doi = {http://dx.doi.org/10.1016/0004-3702(95)00045-3},
 publisher = {Elsevier Science Publishers Ltd.},
 address = {Essex, UK},
 }

@inproceedings{MitchellSelman92,
    author = "David G. Mitchell and Bart Selman and Hector J. Levesque",
    title = "Hard and Easy Distributions for {SAT} Problems",
    booktitle = "Proc. 10th AAAI",
    publisher = "AAAI Press",
    address = "Menlo Park, California",
    pages = "459--465",
    year = "1992",
   }

@inproceedings{BayardoPehousek00,
    author = "R. J. Bayardo Jr. and J. D. Pehousek",
    title = "Counting models using connected components",
    booktitle = "Proc. 17th AAAI",
    publisher = "AAAI Press",
    address = "Menlo Park, California",
    pages = "157--162",
    year = "2000",
   }

@unpublished{BayatiNair06,
    author = "Mohsen Bayati and Chandra Nair",
    title = "A rigorous proof of the cavity method for counting matchings",
    booktitle = "Allerton conference on communication, control and computing,",
    note = "arXiv:cond-mat/0607290v2 [cond-mat.dis-nn]",
    year = "2006",
   }

@inproceedings{BayatiShah05,
    author = "M. Bayati and D. Shah and M. Sharma",
    title = "Maximum Weight Matching via Max-Product Belief Propagation",
    booktitle = "Proc. IEEE Int. Symp. Information Theory",
    year = "2005",
   }

@inproceedings{BayatiShah06,
    author = "M. Bayati and D. Shah and M. Sharma",
    title = "A simpler max-product maximum weight matching algorithm and the auction algorithm",
    booktitle = "Proc. IEEE Int. Symp. Information Theory",
    year = "2006",
   }


@inproceedings{SelmanKautz96,
    author = "Bart Selman and Henry A. Kautz and Bram Cohen",
    title = "Local Search Strategies for Satisfiability Testing",
    booktitle = "Proceedings of the Second {DIMACS} Challange on Cliques, Coloring, and Satisfiability",
    address = "Providence RI",
    editor = "Michael Trick and David Stifler Johnson",
    year = "1996",
    url = "citeseer.ist.psu.edu/article/selman96local.html" }

@inproceedings{SelmanKautz94,
    author = "Bart Selman and Henry A. Kautz and Bram Cohen",
    title = "Noise strategies for improving local search",
    booktitle = "Proc. 12th AAAI",
    publisher = "AAAI Press",
    address = "Menlo Park, CA, USA",
    pages = "337--343 ",
    year = "1994"
 }




@ARTICLE{KrzakalaMontanari06,
  author = {Florent Krzakala and Andrea Montanari and Federico Ricci-Tersenghi and Guilhem Semerjian and Lenka Zdeborov{\'a}},
  title = {Gibbs States and the Set of Solutions of Random Constraint Satisfaction   Problems},
  journal = {Proc. Natl. Acad. Sci. U.S.A},
  volume = {104},
  pages = {10318},
  year = {2007}
}




@ARTICLE{MoraRivoire06b,
   author = {{Mora}, T. and {Rivoire}, O.},
    title = "{Statistical mechanics of error exponents for error-correcting codes}",
  journal = {Phys. Rev. E},
   eprint = {cond-mat/0606696},
     year = 2006,
    month = nov,
   volume = 74,
   number = 5,
    pages = {056110},
      doi = {10.1103/PhysRevE.74.056110},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006PhRvE..74e6110M&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MoraMezard06,
   author = {{Mora}, T. and {M{\'e}zard}, M.},
    title = "{Geometrical organization of solutions to random linear Boolean equations}",
  journal = {J. Stat. Mech.},
     year = 2006,
    month = oct,
   volume = 10,
    pages = {P10007},
      doi = {10.1088/1742-5468/2006/10/P10007},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006JSMTE..10..007M&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@book{MillerThatcher72
,title={{Complexity of computer computations}}
,booktitle={{Complexity of computer computations}}
,editor={Raymond E. Miller and James W. Thatcher}
,ISBN={0306307073}
,MR={51:9575}
,publisher={Plenum Press}
,address={New York}
,year={1972}
}

@article{AchlioptasFriedgut99,
 author = {Dimitris Achlioptas and Ehud Friedgut},
 title = {A sharp threshold for k-colorability},
 journal = {Random Struct. Algorithms},
 volume = {14},
 number = {1},
 year = {1999},
 issn = {1042-9832},
 pages = {63--70},
 doi = {http://dx.doi.org/10.1002/(SICI)1098-2418(1999010)14:1<63::AID-RSA3>3.0.CO;2-7},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
 }

@article{CreignouDaude03,
 author = {Nadia Creignou and HervÃ© DaudÃ© and Olivier Dubois},
 title = {Approximating the Satisfiability Threshold for Random k-XOR-formulas},
 journal = {Comb. Probab. Comput.},
 volume = {12},
 number = {2},
 year = {2003},
 issn = {0963-5483},
 pages = {113--126},
 doi = {http://dx.doi.org/10.1017/S0963548302005552},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
 }

@inproceedings{Schaefer78,
	author="T. J. Schaefer",
	title="The complexity of satisfiability problems",
	booktitle="Proc. 10th STOC",
	publisher="ACM",
	pages="216--226",
	year="1978",
	address="New York, NY, USA"}

@ARTICLE{Murayama04,
   author = {{Murayama}, T.},
    title = "{Thouless-Anderson-Palmer approach for lossy compression}",
  journal = {Phys. Rev. E},
   eprint = {cond-mat/0310440},
     year = 2004,
    month = mar,
   volume = 69,
   number = 3,
    pages = {035105},
      doi = {10.1103/PhysRevE.69.035105},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004PhRvE..69c5105M&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MurayamaOkada03,
   author = {{Murayama}, T. and {Okada}, M.},
    title = "{One step RSB scheme for the rate distortion function}",
  journal = {Journal of Physics A Mathematical General},
   eprint = {cond-mat/0207637},
     year = 2003,
    month = oct,
   volume = 36,
    pages = {11123-11130},
      doi = {10.1088/0305-4470/36/43/031},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003JPhA...3611123M&db_key=PHY},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MartinianWrainwright06b,
   author = {{Martinian}, E. and {Wainwright}, M.~J.},
    title = "{Analysis of LDGM and compound codes for lossy compression and binning}",
  journal = {ArXiv Computer Science e-prints},
   eprint = {cs/0602046},
     year = 2006,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006cs........2046M&db_key=PRE},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@inproceedings{MartinianWrainwright06,
 author = {Emin Martinian and Martin Wainwright},
 title = {Low Density Codes Achieve theRate-Distortion Bound},
 booktitle = {DCC '06: Proceedings of the Data  Compression Conference (DCC'06)},
 year = {2006},
 isbn = {0-7695-2545-8},
 pages = {153--162},
 doi = {http://dx.doi.org/10.1109/DCC.2006.44},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 }

@inproceedings{KolmogorovWainwright05,
 author = {Vladimir Kolmogorov and Martin Wainwright},
 title = {On the Optimality of Tree-reweighted Max-product Message Passing},
 booktitle = {In 21st Conference on Uncertainty in Artificial Intelligence (UAI)},
 year = {2005},
 }

@unpublished{Chertkov08,
   author = "M. Chertkov",
   title = "Exactness of Belief Propagation for some Graphical Models with Loops",
   year = 2008,
   note = "arXiv:0801.0341v1 [cond-mat.stat-mech]",
}

@article{Newman03,
author = {M. E. J. Newman},
collaboration = {},
title = {The Structure and Function of Complex Networks},
publisher = {SIAM},
year = {2003},
journal = {SIAM Review},
volume = {45},
number = {2},
pages = {167-256},
keywords = {networks; graph theory; complex systems; computer networks; social networks; random graphs; percolation theory},
url = {http://link.aip.org/link/?SIR/45/167/1},
doi = {10.1137/S003614450342480}
}

@article{Tanner81,
  author    = {Robert Michael Tanner},
  title     = {A recursive approach to low complexity codes.},
  journal   = {IEEE Transactions on Information Theory},
  volume    = {27},
  number    = {5},
  year      = {1981},
  pages     = {533-547},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{LubyMitzenmacher97,
 author = {Michael G. Luby and Michael Mitzenmacher and M. Amin Shokrollahi and Daniel A. Spielman and Volker Stemann},
 title = {Practical loss-resilient codes},
 booktitle = {STOC '97: Proceedings of the twenty-ninth annual ACM symposium on Theory of computing},
 year = {1997},
 isbn = {0-89791-888-6},
 pages = {150--159},
 location = {El Paso, Texas, United States},
 doi = {http://doi.acm.org/10.1145/258533.258573},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@ARTICLE{MarinariMonasson06,
   author = {{Marinari}, E. and {Monasson}, R. and {Semerjian}, G.},
    title = "{An algorithm for counting circuits: Application to real-world and random graphs}",
  journal = {Europhysics Letters},
   eprint = {arXiv:cond-mat/0507525},
     year = 2006,
    month = jan,
   volume = 73,
    pages = {8--14},
      doi = {10.1209/epl/i2005-10355-0},
   adsurl = {http://adsabs.harvard.edu/abs/2006EL.....73....8M},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MarinariSemerjian06,
   author = {{Marinari}, E. and {Semerjian}, G.},
    title = "{On the number of circuits in random graphs}",
  journal = {J. Stat. Mech.},
     year = 2006,
    month = jun,
   volume = 6,
    pages = {P06019},
      doi = {10.1088/1742-5468/2006/06/P06019},
   adsurl = {http://adsabs.harvard.edu/abs/2006JSMTE..06..019M},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MarinariSemerjian07,
   author = {{Marinari}, E. and {Semerjian}, G. and {Van Kerrebroeck}, V.
	},
    title = "{Finding long cycles in graphs}",
  journal = {ArXiv Condensed Matter e-prints},
   eprint = {cond-mat/0702613},
     year = 2007,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2007cond.mat..2613M},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@book{LovaszPlummer86,
	author={Lovasz, L. and Plummer, M. D.},
	title={Matching Theory},
	publisher={North-Holland},
	address={Amsterdam, New York},
	year={1986}
}

@ARTICLE{ZdeborovaMezard06,
   author = {{Zdeborov{\'a}}, L. and {M{\'e}zard}, M.},
    title = "{The number of matchings in random graphs}",
  journal = {J. Stat. Mech.},
     year = 2006,
    month = may,
   volume = 5,
    pages = {P05003},
      doi = {10.1088/1742-5468/2006/05/P05003},
   adsurl = {http://adsabs.harvard.edu/abs/2006JSMTE..05..003Z},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{ZdeborovaMezard08,
   author = {{Zdeborov{\'a}}, L. and {M{\'e}zard}, M.},
   title = "{Locked constraint satisfaction problems}",
   journal = {Phys. Rev. Lett.},
   volume = 101,
   pages = {078702},
   year = 2008,
}


@article{ZdeborovaMezard08b,
   author = {{Zdeborov{\'a}}, L. and {M{\'e}zard}, M.},
   title = "{Constraint satisfaction problems with isolated solutions are hard}",
   journal = {	J. Stat. Mech.},
   pages = {P12004},
   year = 2008,
}


@article{OrlitskyViswanathan05,
	author={ Orlitsky, A. and Viswanathan, K. and  Zhang, J.},
	title={Stopping set distribution of LDPC code ensembles},
	journal={IEEE Trans. Inform. Theory},
	volume=51,
	pages={929--953},
	year=2005
}

@inproceedings{KashyapVardy03,
	author={Kashyap, N. and Vardy, A.},
	title={Stopping sets in codes from designs},
	booktitle={Proc. Intern. Symp. on Inform. Theory (ISIT'03)},
	pages=122,
	year=2003
}

@inproceedings{MacKayPostol02,
 author={MacKay, David J. C. and Postol,  M. J. },
 title={Weaknesses of  {M}argulis  and  {R}amanujan--{M}argulis Low-Density Parity-Check  Codes},
 booktitle={Proceedings of MFCSIT2002, Galway},
 volume={74},
 series={Electronic Notes in Theoretical Computer Science},
 publisher={Elsevier},
 year={2003}, annote={Volume 74 of ENTCS}
}

@article{AckleyHinton85,
 author = {David H. Ackley and Geoffrey E. Hinton and Terrence J. Sejnowski},
 title = {A learning algorithm for Boltzmann machines},
 book = {Readings in computer vision: issues, problems, principles, and paradigms},
 year = {1987},
 isbn = {0-934613-33-8},
 pages = {522--533},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
 }

@ARTICLE{Tanaka98,
   author = {{Tanaka}, T.},
    title = "{Mean-field theory of Boltzmann machine learning}",
  journal = {Phys. Rev. E},
     year = 1998,
    month = aug,
   volume = 58,
    pages = {2302-2310},
      doi = {10.1103/PhysRevE.58.2302},
   adsurl = {http://adsabs.harvard.edu/abs/1998PhRvE..58.2302T},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{KappenRodriguez98,
 author = {H. J. Kappen and F. B. RodrÃ­guez},
 title = {Efficient learning in Boltzmann machines using linear response theory},
 journal = {Neural Comput.},
 volume = {10},
 number = {5},
 year = {1998},
 issn = {0899-7667},
 pages = {1137--1156},
 doi = {http://dx.doi.org/10.1162/089976698300017386},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
 }

@article{PetersonAnderson97,
	author={C. Peterson and R. Anderson},
	title={A Mean Field Theory Learning Algorithm for Neural Networks},
	journal={Complex Systems},
	volume=1,
	pages={995--1019},
	year=1987
}

@ARTICLE{SchneidmanBerry06,
   author = {{Schneidman}, E. and {Berry}, M.~J. and {Segev}, R. and {Bialek}, W.
	},
    title = "{Weak pairwise correlations imply strongly correlated network states in a neural population}",
  journal = {Nature},
   eprint = {arXiv:q-bio/0512013},
     year = 2006,
    month = apr,
   volume = 440,
    pages = {1007-1012},
      doi = {10.1038/nature04701},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.440.1007S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@inproceedings{MacKayNeal95,
 author = {David J. C. MacKay and R. M. Neal},
 title = {Good Codes Based on Very Sparse Matrices},
 booktitle = {Proceedings of the 5th IMA Conference on Cryptography and Coding},
 year = {1995},
 isbn = {3-540-60693-9},
 pages = {100--111},
 publisher = {Springer-Verlag},
 address = {London, UK},
 }

@Article{MacKayNeal96,
  author = 	 "D. J. C. MacKay and R. M. Neal",
  title = 	 "Near {S}hannon Limit Performance of Low Density Parity
		  Check Codes",
  key =		 "MacKay and Neal",
  journal =	 "Electronics Letters",
  year =	 1996,
  volume =	 32,
  number =	 18,
  pages =	 "1645-1646",
  month =	 "August",
 note = {Reprinted {\em Electronics Letters}, vol 33, no
                 6, 13th March 1997, p.457--458},
  annote =	 "Date submitted: Jul 12 1996; Date accepted: Aug 12
		  1996; printed 29 Aug. Collaborating institutes:
		  University of Toronto"
}

@article{MacKay99,
    author = "D. J. C. MacKay",
    title = "Good Error-Correcting Codes Based on Very Sparse Matrices",
    journal = "IEEE Trans. Inform. Theory",
    volume = "45",number={2},
 PAGES ="399--431",
    year = "1999",
  }

@book{MezardMontanari07,
	title={Physics, Information, Computation},
	author={M. M\'ezard and A. Montanari},
	year={2009},
        publisher = {Oxford Press},
        address = {Oxford} 
}

@article{FrancoPaull83,
	author={J. Franco, and M. Paull},
	title={Probabilistic analysis of the Davis-Putnam procedure for solving satisfiability},
	journal={Discrete Applied Mathematics},
	volume=5,
	pages={77--87},
	year=1983
}

@ARTICLE{Istrate07,
   author = {{Istrate}, G.},
    title = "{Satisfying assignments of Random Boolean CSP: Clusters and Overlaps}",
  journal = {ArXiv Computer Science e-prints},
   eprint = {cs/0703065},
     year = 2007,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2007cs........3065I},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{KrishnanShankar05,
   author = {{Krishnan}, K.~M. and {Shankar}, P.},
    title = "{On the Complexity of finding Stopping Distance in Tanner Graphs}",
  journal = {ArXiv Computer Science e-prints},
   eprint = {cs/0512101},
     year = 2005,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2005cs.......12101K},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{PrettiWeigt06,
  author = {Marco Pretti and Martin Weigt},
  title = {Sudden emergence of q-regular subgraphs in random graphs},
  journal = {Europhysics Letters},
  volume = {75},
  pages = {8},
  url = {doi:10.1209/epl/i2006-10070-4},
  year = {2006}
}

@ARTICLE{KalapalaMoore05,
   author = {{Kalapala}, V. and {Moore}, C.},
    title = "{The Phase Transition in Exact Cover}",
  journal = {ArXiv Computer Science e-prints},
   eprint = {cs/0508037},
     year = 2005,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2005cs........8037K},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{RaymondSportiello07,
   author = {{Raymond}, J. and {Sportiello}, A. and {Zdeborov{\'a}}, L.},
    title = "{The Phase Diagram of 1-in-3 Satisfiability Problem}",
  journal = {Phys. Rev. E},
   volume = {76},
    pages = {011101},
     year = 2007,
    month = feb,
}

@ARTICLE{CastellaniKrzakala05,
  author = {Tommaso Castellani and Florent Krzakala and Federico Ricci-Tersenghi},
  title = {Spin glass models with ferromagnetically biased couplings on the Bethe lattice: analytic solution and numerical simulations},
  journal = {Eur. Phys. J. B},
  volume = {47},
  pages = {99},
  year = {2005}
}

@ARTICLE{CastellaniNapolano03,
  author = {Tommaso Castellani and Vincenzo Napolano and Federico Ricci-Tersenghi and Riccardo Zecchina},
  title = {Bicoloring Random Hypergraphs},
  journal = {J. Phys. A},
  volume = {36},
  pages = {11037},
  year = {2003}
}

@ARTICLE{SemerjianWeigt04,
   author = {{Semerjian}, G. and {Weigt}, M.},
    title = "{Approximation schemes for the dynamics of diluted spin models: the Ising ferromagnet on a Bethe lattice}",
  journal = {Journal of Physics A Mathematical General},
   eprint = {arXiv:cond-mat/0402451},
     year = 2004,
    month = may,
   volume = 37,
    pages = {5525-5546},
      doi = {10.1088/0305-4470/37/21/003},
   adsurl = {http://adsabs.harvard.edu/abs/2004JPhA...37.5525S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{SemerjianMonasson03,
  title = {Relaxation and metastability in a local search procedure for the random satisfiability problem},
  author = {Semerjian, Guilhem  and Monasson, R\'emi },
  journal = {Phys. Rev. E},
  volume = {67},
  number = {6},
  pages = {066103},
  numpages = {18},
  year = {2003},
  month = {Jun},
  doi = {10.1103/PhysRevE.67.066103},
  publisher = {American Physical Society}
}

@article{BurshteinMiller04,
  author    = {David Burshtein and
               Gadi Miller},
  title     = {Asymptotic Enumeration Methods for Analyzing LDPC Codes.},
  journal   = {IEEE Transactions on Information Theory},
  volume    = {50},
  number    = {6},
  year      = {2004},
  pages     = {1115-1131},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{LubyMitzenmacher01,
  author =       {M. G. Luby  and M. Mitzenmacher and M. Amin Shokrollahi and
D. A. Spielman},
  title =        {Efficient Erasure Correcting Codes},
journal={IEEE Transactions on Information Theory},
volume={47},
number={2},
pages={569-584},
  year =         {2001}
}

@article{BraunsteinMezard05,
 author = {A. Braunstein and M. M\'ezard and R. Zecchina},
 title = {Survey propagation: An algorithm for satisfiability},
 journal = {Random Struct. Algorithms},
 volume = {27},
 number = {2},
 year = {2005},
 issn = {1042-9832},
 pages = {201--226},
 doi = {http://dx.doi.org/10.1002/rsa.v27:2},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
 }

@article{ManevaMossel05,
     author    = {Elitza N. Maneva and
                  Elchanan Mossel and
                  Martin J. Wainwright},
     title     = {A new look at survey propagation and its generalizations},
     journal   = {J. ACM},
     volume    = {54},
     number    = {4},
     year      = {2007},
}

@unpublished{ManevaSinclair07,
     author    = {Elitza Maneva and Alistair Sinclair},
     title     = {On the Satisfiability Threshold and Clustering of Solutions of Random 3-SAT Formulas},
     note = "arXiv:0710.0805v1 [cs.CC]",
     year      = {2007},
}


@inproceedings{Pearl82,
 author = {J. Pearl},
 title = {Reverend Bayes on inference engines: A distributed hierarchical approach},
 booktitle = {Proceedings American Association of Artificial Intelligence National Conference on AI},
 year = {1982},
 pages = {133--136},
 address = {Pittsburgh, PA, USA},
 }



@ARTICLE{RivoireBarre06,
   author = {{Rivoire}, O. and {Barr{\'e}}, J.},
    title = "{Exactly Solvable Models of Adaptive Networks}",
  journal = {Physical Review Letters},
   eprint = {arXiv:cond-mat/0606754},
     year = 2006,
    month = oct,
   volume = 97,
   number = 14,
    pages = {148701},
      doi = {10.1103/PhysRevLett.97.148701},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvL..97n8701R},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@MISC{MeassonMontanari05,
  author = {Cyril Measson and Andrea Montanari and Ruediger Urbanke},
  title = {Maxwell Construction: The Hidden Bridge between Iterative and Maximum a  Posteriori Decoding},
  url = {http://www.citebase.org/abstract?id=oai:arXiv.org:cs/0506083},
  year = {2005}
}

@MISC{MontanariTse06,
  author = {Andrea Montanari and David Tse},
  title = {Analysis of Belief Propagation for Non-Linear Problems: The Example of  CDMA (or: How to Prove Tanaka's Formula)},
  url = {http://www.citebase.org/abstract?id=oai:arXiv.org:cs/0602028},
  year = {2006}
}

@ARTICLE{LebowitzSpohn98,
   author = {{Lebowitz}, J.~L. and {Spohn}, H.},
    title = "{A Gallavotti-Cohen Type Symmetry in the Large Deviation Functional for Stochastic Dynamics}",
  journal = {ArXiv Condensed Matter e-prints},
   eprint = {cond-mat/9811220},
     year = 1998,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/1998cond.mat.11220L},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{EvansKenyon00,
   author = {William Evans and Claire Kenyon and Yuval Peres and Leonard J. Schulman},
    title = "{Broadcasting on trees and the Ising model}",
  journal = {Ann. Appl. Probab.},
     year = 2000,
   volume = 10,
    pages = {410--433},
}

@ARTICLE{EvansSearles02,
   author = {{Evans}, D.~J. and {Searles}, D.~J.},
    title = "{The Fluctuation Theorem}",
  journal = {Advances in Physics},
     year = 2002,
    month = nov,
   volume = 51,
    pages = {1529--1585},
   adsurl = {http://adsabs.harvard.edu/abs/2002AdPhy..51.1529E},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{Montanari05,
	author={A. Montanari},
	title={Tight Bounds for LDPC and LDGM Codes Under MAP Decoding},
	journal={IEEE Trans. Inform. Theory},
	volume=51,
	pages={3221--3246},
	year=2005
}


@incollection{BraunsteinMezard02,
       author = "{Braunstein}, A. and {M\'ezard}, M. and {Weigt}, M. and {Zecchina}, R.",
       title = "Constraint Satisfaction by Survey Propagation",
       editor = "Allon Percus and Gabriel Istrate and Cristopher Moore",
       booktitle = "Computational Complexity and Statistical Physics",
       pages = "107",
       year = 2003,
       publisher = "Oxford University Press"}


@ARTICLE{Zhou05,
   author = {{Zhou}, H.},
    title = "{Long-Range Frustration in a Spin-Glass Model of the Vertex-Cover Problem}",
  journal = {Physical Review Letters},
   eprint = {arXiv:cond-mat/0411077},
     year = 2005,
    month = jun,
   volume = 94,
   number = 21,
    pages = {217203},
      doi = {10.1103/PhysRevLett.94.217203},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvL..94u7203Z},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{ChertkovChernyak06,
   author = {{Chertkov}, M. and {Chernyak}, V.~Y.},
    title = "{Loop series for discrete statistical models on graphs}",
  journal = {Journal of Statistical Mechanics: Theory and Experiment},
   eprint = {arXiv:cond-mat/0603189},
     year = 2006,
    month = june,
   volume = 6,
    pages = {P06009},
      doi = {10.1088/1742-5468/2006/06/P06009},
   adsurl = {http://adsabs.harvard.edu/abs/2006JSMTE..06..009C},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{StepanovChernyak05,
   author = {{Stepanov}, M.~G. and {Chernyak}, V. and {Chertkov}, M. and 
	{Vasic}, B.},
    title = "{Diagnosis of Weaknesses in Modern Error Correction Codes: A Physics Approach}",
  journal = {Physical Review Letters},
   eprint = {arXiv:cond-mat/0506037},
     year = 2005,
    month = nov,
   volume = 95,
   number = 22,
    pages = {228701},
      doi = {10.1103/PhysRevLett.95.228701},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvL..95v8701S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{MontanariRizzo05,
   author = {{Montanari}, A. and {Rizzo}, T.},
    title = "{How to compute loop corrections to the Bethe approximation}",
  journal = {Journal of Statistical Mechanics: Theory and Experiment},
   eprint = {arXiv:cond-mat/0506769},
     year = 2005,
    month = oct,
   volume = 10,
    pages = {P10011},
      doi = {10.1088/1742-5468/2005/10/P10011},
   adsurl = {http://adsabs.harvard.edu/abs/2005JSMTE..10..011M},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@article{MezardMontanari06,
	author={Marc M\'ezard and Andrea Montanari},
	title={Reconstruction on Trees and Spin Glass Transition},
	journal={J. Stat. Phys.},
	volume={124},
	pages={1317--1350},
	year=2006,
	month={september}
}

@ARTICLE{FreyDueck07,
   author = {{Frey}, B.~J. and {Dueck}, D.},
    title = "{Clustering by Passing Messages Between Data Points}",
  journal = {Science},
     year = 2007,
    month = february,
   volume = 315,
    pages = {972},
      doi = {10.1126/science.1136800},
   adsurl = {http://adsabs.harvard.edu/abs/2007Sci...315..972F},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{BraunsteinZecchina06,
   author = {{Braunstein}, A. and {Zecchina}, R.},
    title = "{Learning by Message Passing in Networks of Discrete Synapses}",
  journal = {Physical Review Letters},
     year = 2006,
   volume = 96,
   number = 3,
    pages = {030201},
      doi = {10.1103/PhysRevLett.96.030201},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvL..96c0201B},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{CorrealeLeone06b,
   author = {{Correale}, L. and {Leone}, M. and {Pagnani}, A. and {Weigt}, M. and 
	{Zecchina}, R.},
    title = "{The computational core and fixed point organization in Boolean networks}",
  journal = {Journal of Statistical Mechanics: Theory and Experiment},
   eprint = {arXiv:cond-mat/0512089},
     year = 2006,
    month = mar,
   volume = 3,
    pages = {P03002},
      doi = {10.1088/1742-5468/2006/03/P03002},
   adsurl = {http://adsabs.harvard.edu/abs/2006JSMTE..03..002C},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@MISC{MahmoudiPagnani07,
  author = {Hamed Mahmoudi and Andrea Pagnani and Martin Weigt and Riccardo Zecchina},
  title = {Propagation of external regulation and asynchronous dynamics in random  Boolean networks},
  url = {http://www.citebase.org/abstract?id=oai:arXiv.org:0704.3406},
  year = {2007}
}

@ARTICLE{TkacikScheidman06,
   author = {{Tkacik}, G. and {Schneidman}, E. and {Berry}, M.~J.~I. and 
	{Bialek}, W.},
    title = "{Ising models for networks of real neurons}",
  journal = {eprint arXiv:q-bio/0611072},
   eprint = {q-bio/0611072},
     year = 2006,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2006q.bio....11072T},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{BarreBouchet05,
  author = {Julien Barr\'e and Freddy Bouchet and Thierry Dauxois and Stefano Ruffo},
  title = {Large deviation techniques applied to systems with long-range  interactions},
  journal = {J. Stat. Phys.},
  volume = {119},
  pages = {677},
  year = {2005}
}

@article{ZdeborovaKrzakala07,
      author = "L. Zdeborov{\'a} and F. Krzakala",
      title = "Phase Transitions in the Coloring of Random Graphs",
      journal = "Phys. Rev. E",
      volume = {76},
      pages = {031131},
      year = 2007}

@inproceedings{WainwrightManeva05,
	author={Wainwright, M.J. and Maneva, E.},
	title={Lossy source encoding via message-passing and decimation over generalized codewords of LDGM codes},
	booktitle={Proc. Intern. Symp. on Inform. Theory (ISIT'03)},
	pages={1493--1497},
	year=2003
}

@article{Semerjian07,
  author = {Guilhem Semerjian},
  title = {On the freezing of variables in random constraint satisfaction problems},
  journal = "J. Stat. Phys.",
  volume = {130},
  pages = {251},
  year = {2008}
}



@inproceedings{AchlioptasChtcherba01,
 author = {Dimitris Achlioptas and Arthur Chtcherba and Gabriel Istrate and Cristopher Moore},
 title = {The phase transition in 1-in-k SAT and NAE 3-SAT},
 booktitle = {SODA '01: Proceedings of the twelfth annual ACM-SIAM symposium on Discrete algorithms},
 year = {2001},
 pages = {721--722},
 location = {Washington, D.C., United States},
 publisher = {SIAM},
 address = {Philadelphia, PA, USA},
 }

@inproceedings{Ben-ShimonVilenchik07,
author={S. Ben-Shimon and D. Vilenchik},
title={Message passing for the coloring problem: Gallager meets Alon and Kahale},
booktitle={Proceedings of the 13th International Conference on Analysis of Algorithms, DMTCS proc.}, 
pages={217--226},
year={2007}
}

@inproceedings{Coja-OghlanKrivelevich07,
author={A. Coja-Oghlan and M. Krivelevich and D. Vilenchik},
title={Why almost all k-colorable graphs are easy to color},
booktitle={Proceedings of the 24th International Symposium on Theoretical Aspects of Computer Science (STACS), LNCS  4393}, 
pages={121--132},
year={2007}
}

@article{AchlioptasJia05,
author={D. Achlioptas and H. Jia and C. Moore},
title={Hiding Truth Assignments: Two are Better Than One },
journal={Journal of Artifical Intelligence Research}, 
volume={24}, 
year={2005}, 
pages={623=-639}
}

@inproceedings{MooreJia05,
author={C. Moore and H. Jia and D. Strain},
title={Generating Hard Satisfiable Formulas by Hiding Solutions Deceptively },
booktitle={Proc. AAAI},
year={2005}
}

@inproceedings{AchlioptasGomes00,
author={D. Achlioptas and C. Gomes and H. Kautz and B. Selman},
title={Generating Satisfiable Problem Instances },
booktitle={Proceedings of AAAI-2000, Austin, Texas, USA},
year={2000}
}

@inproceedings{FeigeMossel06,
author={U. Feige and E. Mossel and D. Vilenchik}, 
title={Complete convergence of message passing algorithms for some satisfiability problems},
booktitle={Proc. of Random 2006, LNCS  4410}, 
pages={339–350},
year={2006}
}

@article{AltarelliMonasson07,
title={Can rare SAT formulas be easily recognized? On the efficiency of message passing algorithms for K-SAT at large clause-to-variable ratios},
author={F. Altarelli, R. Monasson and F. Zamponi},
journal={J. Phys. A: Math. Theor.},
volume={40}, 
pages={867--886},
year={2007} 
}

@unpublished{AchlioptasCoja-Oghlan08,
  author = "Dimitris Achlioptas and Amin Coja-Oghlan",
  title = "Algorithmic barriers from phase transitions",
  year = {2008},
  note = "arXiv:0803.2122v2, in Proceedinds of FOCS'08"
}

@unpublished{ZdeborovaKrzakala09,
  author = "Lenka Zdeborov\'a and Florent Krzakala",
  title = "Quiet Planting in the Locked Constraint Satisfaction Problems",
  year = {2009},
  note = "arXiv:0902.4185v1 [cond-mat.stat-mech]"
}

@article{LiMaZhou08,
  author = "Kang Li and Hui Ma and Haijun Zhou",
  title = "From one solution of a 3-satisfiability formula to a solution cluster: Frozen variables and entropy",
  journal = "Physical Review E",
  year = {2009},
  volume = "79",
  pages = "031102",
}

@unpublished{Zhou09,
author = "H. Zhou", 
title = "Criticality and Heterogeneity in the Solution Space of Random Constraint Satisfaction Problems",
note = "arXiv:0911.4328v1 [cond-mat.dis-nn]",
}
